LEAF: Latent Exploration Along the Frontier

Self-supervised goal proposal and reaching is a key component for exploration and efficient policy learning algorithms. Such a self-supervised approach without access to any oracle goal sampling distribution requires deep exploration and commitment so that long horizon plans can be efficiently discovered. In this paper, we propose an exploration framework, which learns a dynamics-aware manifold of reachable states. For a goal, our proposed method deterministically visits a state at the current frontier of reachable states (commitment/reaching) and then stochastically explores to reach the goal (exploration). This allocates exploration budget near the frontier of the reachable region instead of its interior. We target the challenging problem of policy learning from initial and goal states specified as images, and do not assume any access to the underlying ground-truth states of the robot and the environment. To keep track of reachable latent states, we propose a distance-conditioned reachability network that is trained to infer whether one state is reachable from another within the specified latent space distance. Given an initial state, we obtain a frontier of reachable states from that state. By incorporating a curriculum for sampling easier goals (closer to the start state) before more difficult goals, we demonstrate that the proposed self-supervised exploration algorithm, superior performance compared to existing baselines on a set of challenging robotic environments.https://sites.google.com/view/leaf-exploration

==> 1-introduction.tex <==
\section{Introduction}
\label{sec:intro}  

%Reinforcement Learning (RL) enables agents to learn complex skills by interacting with the environment, alleviating the need for manual engineering of behavioral skills.
Efficient exploration is one of the central open challenges in Reinforcement Learning (RL), and a key requirement for learning optimal policies, particularly in sparse-reward and long-horizon settings, where the optimization problem is difficult to solve, but easy to specify. We show that discovering policies for  these settings benefits significantly from autonomous goal-setting and exploration, which requires keeping track of what regions of the state-space have been sufficiently explored and can be reached via planning, and what regions remain unknown. In this paper we present an exploration method that keeps track of reachable regions of state space and naturally handles the exploration-exploitation dilemma in sequential decision-making for unknown environments~\cite{varibad,goexplore}, while being practical in real robotics settings. \HB{General introduction}


%One of the central challenges in Reinforcement Learning (RL) is to learn large general purpose repertoires of behaviors that can be used for solving  complex tasks, without undertaking the time-consuming and potentially intractable job of learning each behavior separately. Such self-supervised discovery of composable behaviors for solving temporally extended tasks requires agents to autonomously explore the environment, keep track of what regions of the state-space have been sufficiently explored and can be reached, and hence naturally relates to the exploration-exploitation dilemma in sequential decision-making in unknown environments~\cite{varibad,goexplore}. \HB{General introduction}



For learning to plan in \textit{unknown} environments, appropriately trading off exploration i.e. learning about the environment, and exploitation i.e. executing promising actions is the key to successful policy learning. The necessity for this trade-off is more pertinent when we want to train agents to learn autonomously in a self-supervised manner such that it is able to solve goals sampled from an unknown distribution during evaluation. In this setting, during training, the agent must practice reaching self-specified random goals~\cite{rig}. However, trying to specify goals through exact states of objects in the environment will require a combinatorially large representation, for explicitly randomizing different variables of the states~\cite{avi,rig}. On the contrary, raw sensory signals, such as images can be used to specify goals, as has been done in recent goal-conditioned policy learning algorithms~\cite{rig,upn,skew}\HB{In the previous two lines I am trying to motivate the need for learning from images even in simulation. In the real environment it is clear why we want to use images as input - we cannot describe the environment state exactly.}. This paper tackles the question of how should an autonomous agent balance exploration and exploitation for goal-directed robotic tasks while learning directly from images, with no access to the ground-truth parameters of the environment during training. 
%Specifically, we focus our attention to the problem of keeping track of the frontier of reachable states, and using latent space reachability measures to devise efficient exploration algorithms in the above setting. \HB{The problem being considered. It is slightly vague because I intended this to be a description of the problem, not the solution. I would appreciate help to make it more crisp though.}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{illustrative_figs/reachexplore_idea_final.png}
    \caption{ReachExplore encourages reaching the current frontier of reachable states with a deterministic policy, and performing goal-directed exploration beyond it with a stochastic policy. In this illustration, the yellow volume corresponds to end-effector positions for the currently reachable frontier corresponding to the shown initial state.}
    \label{fig:firstfig}
    \vspace*{-0.7cm}
\end{figure}
% In this paper, we attempt to mitigate the exploration-exploitation tradeoff in self-supervised learning of goal-conditioned policies directly from images by keeping track of the frontier of reachable states, and performing committed exploration. 


\begin{figure*}[h!]
\centering
   \hspace*{-0.9cm}
        \begin{subfigure}[b]{0.7\textwidth}
               \centering
    \includegraphics[width=0.9\textwidth]{arxiv_version/figures/ReachExploreMainfig_updated.png}
    \caption{Forward pass of the ReachExplore approach}
    \label{fig:reachidea}
        \end{subfigure}% \\
        \hspace*{-0.8cm}
         \begin{subfigure}[b]{0.37\textwidth}
               \centering
    \includegraphics[width=\textwidth]{reachnet.png}
    \caption{Reachability Network}
    \label{fig:reachnet}
        \end{subfigure}                 %\quad
     \caption{(a) An overview of our method ReachExplore on the Sawyer Pick and Place task. The initial and goal images are encoded by the encoder of the VAE into latents $z_0$ and $z_g$ respectively. Random states are sampled from the currently learned manifold of the VAE latent states, and are used to infer the current frontier $p_{k^*}$ as described in Section~\ref{sec:reachidea}. The currently learned deterministic policy is used to reach a state in the frontier $z^*$ from the initial latent state $z_0$. After that, the currently learned stochastic policy is used to reach the latent goal state $z_g$. A reconstruction of what the latent state in the frontier $z^*$ decodes to is shown. For clarity, a rendered view of the actual state $z^*$ reached by the agent is shown alongside the reconstruction. (b) A schematic of the reachability network used to determine whether the latent state $z_i$ ($state_i$) is reachable from the latent state $z_j$ ($state_j$) in $k$ time-steps. The reachability vector $\mathbf{k}$ consists of a vector of the same size as $z_i$ and $z_j$ with all its elements being $k$. The output $0$ indicates that state $z_i$ is not reachable from state $z_j$.} 
 \label{fig:mainfig}
 \vspace*{-0.7cm}
\end{figure*}
The main idea of our approach is to maintain and gradually expand the frontier of reachable states by trying to reach the current frontier directly without exploring i.e. by executing a deterministic goal-conditioned policy, and exploring from beyond the current frontier in order to reach the goal by executing a stochastic goal-conditioned policy (Fig.~\ref{fig:firstfig}). In order to achieve this, we encourage the agent to sample goals closer to the start state(s) before sampling goals that are farther away, by appropriately querying the reachability network. Planning directly in the pixel-space is not meaningful. For example, computing rewards as the pixel-wise distance between two images does not necessarily correspond to a semantically meaningful correlation with respect to how close the two ground-truth states actually are~\cite{upn,rig}. Hence, we learn a latent abstraction from images, and plan in the latent space. We train a reachability network that learns whether a latent state is currently reachable from another latent state in $k$ time-steps ($k$ varies from $1$ to the maximum length of the horizon), and use this network to compute the current frontier of reachable states given a random initial start state during training. While training the goal-conditioned policy to reach a goal latent state (corresponding to a goal image), we first execute the deterministic policy trained so far to reach a latent state at the frontier (\textit{commitment}), and then execute the stochastic policy from beyond the frontier to reach the goal (\textit{exploration}). We refer to this procedure of commitment to reach the frontier and exploring beyond it as \textit{committed exploration} required for solving temporally abstracted tasks. \HB{The proposed approach. Every episode in training hasa two phases - execute deterministic policy to reach frontier. Explore beyond frontier while trying to reach goal. I don't mean to say the 2nd phase here is "deep exploration". The overall scheme of having this two stage approach is enforcing deep exploration - to discover temporally abstracted winning sequences of actions that solve the task - this process happens completely at the end of training, when the reachable frontier = real frontier.}

%In order to impose this curriculum over the self-supervised sampling of goals during training, we gradually increase the max. horizon length of episodes during successive epochs of training. 

In summary, this paper makes the following contributions:
\begin{enumerate}
%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]
 \item We propose a dynamics-aware latent space reachability network.
 \item We devise a policy learning scheme using the reachability network that combines deterministic and stochastic policies for committed exploration. 
 \item We empirically evaluate the proposed approach  in a range of both image-based, and state-based simulation environments, and in a real robot environment. We demonstrate an improvement of $30\%$ on average compared to state-of-the-art exploration baselines. 
\end{enumerate}


%Since the proposed approach explicitly keeps track of reachability for committed exploration, we call our approach ReachExplore. 
% Through detailed experimentation across image-based simulation environments, a state-based simulation environment, and a real-world robotic environment, we show that ReachExplore successfully solves difficult temporally-extended tasks by achieving much higher rewards and converging with much less interactions with the environment as compared to state-of-the art image-based exploration methods. \HB{image based methods.} \HB{A brief highlight of the results. To put in specifics if needed later.}

==> 2-preliminaries.tex <==
\section{Problem Setup and Background}
% In this section, we elaborate on the key concepts and paradigms that relate to the proposed approach, and lay out the mathematical notations for the rest of the paper.
\label{sec:prelim}

\subsection{Problem Setup}
In standard model-free RL, the objective is to learn a policy $\pi(\cdot)$ as a function of the current state of the world $s_t$ (this could be a latent abstraction state as well) that outputs an action $a_t=\pi(s_t)$ to be executed in the environment, such that the expected sum of discounted returns from the environment $R_t=\mathbb{E}_{\pi(a|s),p(s'|s,a)} [\sum_{i=t}^T\gamma^{(i-t)}r(s_i,a_i,s_{i+1})]$ is maximized. Here, $a\in\mathcal{A}$, $s\in\mathcal{S}$, $\gamma$, and $r(\cdot)$ respectively denote an action in the set of actions, a state in the set of states, the discount factor, and the reward function.

\noindent \textbf{ Goal-conditioned policies} This formulation is insufficient when we want to optimize expected returns with respect to different goals that can be specified at test-time. Hence, explicitly conditioning the policy on the goal $s_g$ that must be achieved in the current episode, $a_t=\pi(s_t;s_g)$, and optimizing the expected sum of discounted rewards over different goals $s_g$ sampled from the goal distribution $s_g\sim\mathcal{G}$, $R_t=\mathbb{E}_{\pi(a|s;s_g),p(s'|s,a)} [\sum_{i=t}^T\gamma^{(i-t)}r(s_i,a_i,s_{i+1};s_g)]$  is a common method of learning policies that can be adapted to different goals at test time~\cite{her}.

\noindent \textbf{Self-supervised learning to solve goals} We consider the setting of learning directly from images, such that the the goals are specified as images to the policy. Also, the setting is self-supervised in the sense that during training, we do not have access to any oracle goal-sampling distribution from which goals will be sampled at test-time. Hence, the agent must learn to autonomously set goals and solve them during training, in order to learn necessary re-usable skills for solving new goals sampled from an unknown distribution at test-time. 

This is the setting considered in a number of recent approaches for policy learning~\cite{skew,rig}, and is challenging because it assumes very less information about the ground-truth environment and goal-specifications. One of the desiderata as pointed out in Skew-Fit~\cite{skew} is to sample sufficiently diverse goals and learn to solve them, i.e. optimize $\mathcal{H}(\mathcal{G}) - \mathcal{H}(\mathcal{G}|\mathcal{S})$, where $\mathcal{H}(\cdot)$ denotes entropy. Although this guarantees uniform coverage in the infinite limit (assuming a perfectly learned goal-reaching policy), it does not ensure deep exploration in the finite horizon case.  \HB{Agreed that uniform coverage is not guaranteed for SkewFit in the general case. For showing this, SkewFit assumes a perfect oracle goal-reaching policy. But even if the goal-reaching policy is learned (not given by an oracle), then if we assume that it can be perfectly learned, the SkewFit analysis will still hold, and they can claim uniform coverage in the infinite limit. } In this paper, we emphasize the need to keep track of reachable states so to enable deep exploration via commitment, and set goals in a curriculum fashion, so that the agent learns to solve easier goals before trying to solve more difficult goals. 


  
\subsection{Notation}

We denote the set of observations (images) as $\mathcal{S}$ and the set of goals (images) as $\mathcal{G}$. In this paper we assume the underlying sets for $\mathcal{S}$ and $\mathcal{G}$ to be the same (any valid image can be a goal image~\cite{rig,skew}) but maintain separate notations for clarity. $f_\psi(\cdot)$ denotes the encoder of the $\beta-VAE$~\cite{betavae} that encodes observations $s\sim S$ to latent states $z\sim f_\psi(s)$. The goal conditioned policy given the current latent state $z_t$, and the goal $z_g$ is denoted by $\pi_\theta(\cdot | z_t,z_g)$, and $a_t\sim \pi_\theta(\cdot | z_t,z_g)$ denotes the action sampled from the policy at time $t$. The policy $\pi_\theta(\cdot | z_t,z_g)$ consists of a deterministic component $\mu_\theta(\cdot | z_t,z_g)$, and a noise term $\epsilon$, such that $\pi_\theta(\cdot | z_t,z_g) = \mu_\theta(\cdot | z_t,z_g) + \sigma_\theta\epsilon$, where $\epsilon$ is a Gaussian $\mathcal{N}(0,\mathbf{I})$ in this paper. $ReachNet(z_i,z_j;k)$ denotes the reachability network that takes as input two latent states  $z_i$, and $z_j$ and is conditioned on a reachability integer $k\in[1,..,H]$, where $H$ is the maximum time horizon of the episode. The output of $ReachNet(z_i,z_j;k)$ is either a $0$ denoting $z_j$ is currently not reachable from $z_i$  (and vice-versa) or a $1$ denoting $z_j$ is reachable from $z_i$ (and vice-versa). 

We consider the problem setting where a robot is initialized to a particular configuration, and is tasked to reach a goal, specified as an image. The test time goal distribution, from which goal images will be sampled for evaluation is not available during training, and hence the training approach is completely self-supervised. The underlying distribution of observations $\mathcal{S}$ is same as the underlying distribution of goals $\mathcal{G}$ during training, and are distributions over images from a camera.


==> 3-approach.tex <==
\vspace*{-0.2cm}
\section{Our Approach: ReachExplore}
\label{sec:approach}
In this section, we discuss the specifics of the proposed approach, ReachExplore, summarized in Algorithm~\ref{alg:mainbrief} .

%\subsection{Setup}


%either a third person view (in the real robot experiment) or from a camera mounted on the robot arm (in all the simulation experiments). 

%  \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{reachnet.png}
%     \caption{A schematic of the reachability network used to determine whether the latent state $z_i$ is reachable from the latent state $z_j$ in $k$ time-steps. The reachability vector $\mathbf{k}$ consists of a vector of the same size as $z_i$ and $z_j$ with all its elements being $k$. The output $0$ indicates that state $z_i$ is not reachable from state $z_j$.}
%     \label{fig:reachnetwork}
% \end{figure}

% \begin{figure*}[h!]
% \centering
%   \hspace*{-0.9cm}
%         \begin{subfigure}[b]{0.30\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{illustrative_figs/reach_vae1.PNG}
%     \caption{Sampling from the VAE}
%     \label{fig:vaegeneral}
%         \end{subfigure}% \\
%         \hspace*{-0.2cm}
%       %\vspace*{-2cm}
%          \begin{subfigure}[b]{0.30\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{illustrative_figs/vae_one_episode_pushreach1.PNG}
%     \caption{Traversal in the latent space}
%     \label{fig:vaeepisode}
%         \end{subfigure}   
%          \hspace*{-0.1cm}
%         \begin{subfigure}[b]{0.4\textwidth}
%               \centering
%   \includegraphics[width=\textwidth]{illustrative_figs/analysis2.PNG}
%     \caption{Analysis of ReachExplore}
%     \label{fig:analysis1}
%           \end{subfigure}   
%          \hspace*{-0.9cm}%\quad
%     \caption{(a) ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red). (b) This figure shows how sampling goals that lie on the latent VAE manifold and traversing on the latent manifold leads to latent states that decode to realistic dynamically feasible image frames.\
%     (c) The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (3) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it executes the stochastic policy for $T-k^*$ steps. (2) shows the case when the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then executes the stochastic policy for $T-k$ steps. This is similar in principle to the high level idea of Go-Explore~\cite{goexplore} (1) shows the case when the agent executes the stochastic policy for $T$ steps starting at the origin. The simplified Go-Explore and SkewFit~\cite{skew} models are described in Section~\ref{sec:analysis}}
%     \label{fig:vae}
%     \vspace*{-0.5cm}
% \end{figure*}


\subsection{The ReachExplore Insight}
\label{sec:reachidea}
Consider the goal conditioned policy $\pi(\cdot | z_t,z_g)$ with an initial latent state $z_0$, and a goal latent state $z_g$. The key idea of ReachExplore is to do committed exploration, by directly going to the frontier of reachable states for $z_0$ by executing the deterministic policy $\mu_\theta(\cdot | z_t,z_{k^*})$ and then execute the exploration policy $\pi_\theta(\cdot | z_t,z_g)$ from the frontier to perform goal directed exploration for the actual goal $z_g$. The frontier defined by $p_{k^*}$ is the empirical distribution of states that can be reliably reached from the initial state, and are the farthest away from the initial state, in terms of the minimum number of timesteps needed to visit them. The timestep index $k^*$ that defines how far away the current frontier is, can be computed as follows:
$$k^*=\argmax_k(IsReachable(z_0;k)) $$
The binary predicate  $IsReachable(z_0;k)$ keeps track of whether the fraction of states in the empirical distribution of $k-$reachable states $p_k$ is above a threshold $1-\delta$. The value of $IsReachable(z_0;k)$ $\forall k\in[1,..,H]$ before the start of the episode from $z_0$ is computed as:
%IsReachable(k)==True \text{iff}
\begin{equation}
       =\begin{cases}
      True, & \text{if}\ \mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)\geq 1 - \delta \\
      False, & \text{otherwise}
    \end{cases}
  \end{equation}
Here  $p_\phi(z)$ is the current probability distribution of latent states as learned by the $\beta-VAE$~\cite{betavae} with encoder $f_\psi(\cdot)$. For computing $\mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)$ above, we randomly sample states $z\sim p_\phi(z)$ from the latent manifold of the VAE, the intuition of which is illustrated in Fig.~\ref{fig:vae}. After calculating all the predicates $IsReachable(z_0;k)$ $\forall k\in[1,...,H]$ and determining the value of $k^*$, we sample a random state $z_{k^*}$ from the empirical distribution of $k^*-$reachable states, $p_{k^*}$, ensuring that it does not belong to any $p_{k}$ $ \forall k< k^*$. Here, the empirical distribution $p_k$ denotes the set of states $z$ in the computation of $\mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)$ for which $ReachNet(z_0,z;k)$ returns a $1$, and  $ReachNet(z_0,z;k')$ returns a $0$, $\forall k'<k$.

\begin{algorithm}[t!]
	\begin{algorithmic}[1]
		\Procedure{Reach-Explore}{GCP $\mu_\theta$, $\pi_\theta$, Prior $p(z)$, $S$, $f_\psi(\cdot)$, $IsReachable(\cdot)$, $H_0$, $N$, $\epsilon$, $\delta$, ReplayBuffer $\mathcal{B}$}
		\State $p_\phi = p(z)$
		\State Init $ReachNet(\cdot,\cdot; k)$, Def ReachData $\mathcal{D}$, $K=H_0N$
% 			\State Initialize $ReachNet(\cdot,\cdot; k)$ where $k=\{K,...,1\}$ 
% 			\State Def $K=H_0*N$ lists for $p_k$.
% 			\State Def Global ReachDataset = $\{ \}$ //to train $ReachNet$
		\For{episodes = 1 to $N$}
		\State $s_0\sim S_0$, encode $z_0=f_\psi(s_0)$, $z_{g}\sim p_\phi,\hat{z}^*=z_0$
% 		\State Sample initial state $s_0\sim S_0$, encode $z_0=f_\psi(s_0)$
% 		\State Sample latent goal $z_{g}$ from $p_\phi=p_{skewed}$
    %\State $\hat{z}^*=z_0$
    % \State //\texttt{Apply ReachExplore idea after some training}
	\If{episodes $\geq$ $N/4$} 
	 \For{$k=K-1,...,1$}
	\State Set the value of $IsReachable(z_0;k)$
	 \EndFor
% 			 \State Sample $M$ latent states $\{z\}_M\sim p_{\phi}$
% 	 \For{$k=K_{max},...,1$, $\forall z\in\{z\}_M$}
% 	 \State Initialize list $p_k\longleftarrow\{\}$
	
% 	  \If{$\frac{1}{k-1}\sum_{i=1}^{k-1}	 ReachNet(z,z_0;i)\geq 1-\epsilon$} 
% 	  \State Append $z$ to $p_k$
% 	  \EndIf
% 	  \For{counter = 1 to $C$}
% 	  \State Sample a latent state $z\sim p_k$
% 	   \If{$ReachNet(z,z_0;k)$}
% 	  \State c = c+1
% 	  \EndIf
% 	  \EndFor
% 	  \If{$\frac{c}{C}\geq 1-\epsilon$} 
% 	  \State Set $IsReachable(k)==True$
% 	  \EndIf
% 	  \EndFor
	  \State  $k^*=\argmax_k(IsReachable(z_0;k))$ 
	  \State Sample a latent state in the frontier, $z^*\sim p_{k^*}$
	  	% 	\State //Set initial latent state to be $z^*$
	  	\State Exec $\pi_\theta(z_0;z^*)$	to reach $\hat{z}^*$ s.t. $||\hat{z}^*-z^*||<\delta$
	  	\EndIf
		\State Set $H=H_0*episodes$ // \texttt{Curriculum} 
		\For{$t=0,...,H-1$}
		\If{$t==0$}
		\State Select $a_t\sim\mu_\theta(\hat{z}^*;z_{g})$ and execute it
		\EndIf
		\If{$t>0$ and $t<k^*$}
		\State Select $a_t\sim\mu_\theta(f_\psi(s_t);z_{g})$ and execute it
		\EndIf 
			\If{$t>0$ and $t\geq k^*$}
		\State Select $a_t\sim\pi_\theta(f_\psi(s_t);z_{g})$ and execute it
		\EndIf 
		\State // \texttt{Store tuple and Train policy}
		\State \textsc{StoreandTrain()}
		\EndFor 
%\State //Append to the dataset for training the ReachNet
%\State //Append observations and labels to $\mathcal{D}$
\State \textsc{AppendtoDataset($\mathcal{D}$)}
% \For{$t_1 = 0,...,H-1$}
% \For{$t_2 = 0,...,H-1$}
% \If{$t_1\neq t_2$}
% \State ReachDataset.add($(z_{t_1},z_{t_2},|t_1-t_2|)$)
% \EndIf
% \EndFor
% \EndFor

		

% 	\EndFor
%\State // Samples states to add in replay buffer $\mathcal{R}$
% \State //\texttt{Replay with goals as previously seen states}
\State \textsc{SampleFutureStates($\mathcal{B}$)}
% 	\For{$t=0,...,H-1$}
% 	\For{$i=0,...,k-1$}
%     \State Sample future states $s_{h_i}, t\leq h_i-1 \leq H-2$
%     \State Store $(s_t,a_t,s_{t+1},f_\psi(s_{h_i}),h_i+1)$ in $\mathcal{R}$
%     	\EndFor
%     		\EndFor
    \State Construct skewed dist.  $p_{skewed}$ from $\mathcal{B}$ (Skew-Fit) 
    \State Train the encoder using $p_\phi = p_{skewed}$
    \State Train $ReachNet(\cdot,\cdot; k)$ using ReachDataset $\mathcal{D}$
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\caption{Overview of the ReachExplore Algorithm (Subroutines and the complete Algorithm are in the Appendix)}
	\label{alg:mainbrief}
\end{algorithm}
  
%  remove space after algo float  
% \setlength{\textfloatsep}{5pt}% Remove \textfloatsep


ReachExplore encourages \textit{committed} exploration because the set of states until the frontier $p_{k^*}$ have already been sufficiently explored, and hence the major thrust of exploration should be beyond that, so that new states are rapidly discovered. The SkewFit~\cite{skew} approach showed that if the distribution over states is skewed to highly weigh rare states, and goals are sampled from this skewed distribution, the entropy over states $\mathcal{H}(\mathcal{S})$ will eventually approach the entropy of a uniform distribution $U_{\mathcal{S}}$ over the states. However, this is guaranteed in the infinite time limit. Applying ReachExplore with the SkewFit trick for sampling goals will still maintain the guarantee of maximum entropy, but improve sample efficiency of policy learning. Algorithm~\ref{alg:mainbrief} shows an overview algorithm for ReachExplore. In our specific implementation, we use SAC~\cite{sac} as the base off-policy model-free RL algorithm for minimizing the Bellman Error in the overall algorithm that is described in the Appendix.


\begin{figure*}[t!]
\centering
   \hspace*{-1cm}
       \adjustbox{valign=t}{ \begin{subfigure}[t]{0.60\textwidth}
               \centering
    \includegraphics[width=\textwidth]{arxiv_version/figures/vae_manifold_updated.png}
    \caption{\begin{footnotesize}(1) ReachExplore samples latent goals from the the probability density manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold (i.e. sampling $z$ with low probability density under $p_\phi(z)$) is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the sphere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red). (2) The second figure shows how sampling goals that lie on the latent VAE manifold and traversing on the latent manifold leads to latent states that decode to realistic dynamically feasible image frames.\end{footnotesize}}
    \label{fig:vaegeneral}
        \end{subfigure}}% \\
    %     \hspace*{-0.1cm}
    %   %\vspace*{-2cm}
    %      \adjustbox{valign=t}{\begin{subfigure}[t]{0.30\textwidth}
    %           \centering
    % \includegraphics[width=\textwidth]{illustrative_figs/vae_one_episode_pushreach1.PNG}
    % \caption{\textcolor{red}{This figure shows how sampling goals that lie on the latent VAE manifold and traversing on the latent manifold leads to latent states that decode to realistic dynamically feasible image frames.}}
    % \label{fig:vaeepisode}
    %     \end{subfigure}}   
        % \hspace*{-0.1cm}
        \hspace{0.2cm}
        \adjustbox{valign=t}{\begin{subfigure}[t]{0.38\textwidth}
               \centering
   \includegraphics[width=\textwidth]{illustrative_figs/analysis_final.PNG}
    \caption{\begin{footnotesize}\textcolor{black}{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (3) shows the case when  the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it executes the stochastic policy for $T-k^*$ steps. (2) shows the case when the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then executes the stochastic policy for $T-k$ steps. (1) shows the case when the agent executes the stochastic policy for $T$ steps starting at the origin. The simplified Go-Explore~\cite{goexplore} and SkewFit~\cite{skew} models are described in Section~\ref{sec:analysis}}\end{footnotesize}}
    \label{fig:analysis1}
          \end{subfigure}}   
         \hspace*{-0.9cm}%\quad
    \caption{(a) Sampling from the VAE probability density manifold and traversal in the VAE latent space. (b) Simplified analysis of ReachExplore.}
    \label{fig:vae}
    \vspace*{-0.5cm}
\end{figure*}




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{reach_vae.PNG}
%     \caption{ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red).}
%     \label{fig:vae}
% \end{figure}


% \begin{figure}[t]
%     \centering
%      \begin{subfigure}[b]{0.6\columwidth}
%               \centering
%     \includegraphics[width=0.9\columwidth]{illustrative_figs/reach_vae.PNG}
%     \caption{Forward pass of the ReachExplore approach}
%     \label{fig:reachidea}
%         \end{subfigure}% \\
%          \begin{subfigure}[b]{0.4\columwidth}
%               \centering
%      \includegraphics[width=\columnwidth]{illustrative_figs/vae_one_episode.PNG}
%     \caption{Simulation of one episode}
%     \label{fig:reachidea}
%         \end{subfigure}% \\
%     \caption{ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red).}
%     \label{fig:vae}
% \end{figure}



\subsection{Training the Reachability Network}
\label{sec:trainreachnet}
\vspace*{-0.2cm}
The reachability network $ReachNet(z_i,z_j;k)$ is a feedforward neural network with fully connected layers and ReLU non-linearities, the architecture of which is shown in Fig.~\ref{fig:mainfig}, with details in the Appendix. The architecture has three basic components, two encoders ($encoder_{\mathbf{state}}$, $encoder_{\mathbf{reach}}$), one decoder, and one concatenation layer. The latent states $z_i,z_j$ are encoded by the same encoder $encoder_{\mathbf{state}}$ (i.e. two encoders with tied weights, as in a Siamese Network~\cite{siamese}) and the reachability value $k$ is encoded by another encoder $encoder_{\mathbf{reach}}$. In order to ensure effective conditioning of the network $ReachNet$ on the variable $k$, we input a vector of the same dimension as $z_i$ and $z_j$, with all of its values being $k$, $\mathbf{k}=[k,k,...,k]$.

It is important to note that such neural networks conditioned on certain vectors have been previously explored in literature, e.g. for dynamics conditioned policies~\cite{mangapfn}. The three encoder outputs, corresponding to $z_i, z_j,$ and $k$ are concatenated and fed into a series of shared fully connected layers, which we denote as the decoder. The output of  $ReachNet(z_i,z_j;k)$ is a $1$ or a $0$ corresponding to whether $z_j$ is reachable from $z_i$ in $k$ steps or not, respectively.

To obtain training data for $ReachNet$, while executing rollouts in each episode, starting from the start state $z_0$, we keep track of  the number of time-steps needed to visit every latent state $z_i$ during the episode. We store tuples of the form $(z_i,z_j,k_{ij})$ $\forall i<j$ in memory, where $k_{ij} = j-i$, corresponding to the entire episode. Now, to obtain labels $\{0,1\}$ corresponding to the input tuple $(z_i,z_j,k)$, we use the following heuristic:
\begin{equation}
       label(z_i,z_j,k) =\begin{cases}
      1, & \text{if}\ |k_{ij} > \alpha k|\\
      0, & \text{if}  |k_{ij} < k|
    \end{cases}
  \end{equation}
Here $\alpha\in[1.2,1.5)$ is a threshold to ensure sufficient separation between positive and negative examples. 

%may include the bi about symmetric inputs bein fed to ensure the learned notion of symmetry 
\subsection{Implicit Curriculum for Increasing the Frontier}
\label{sec:curricula}
% In Sections~\ref{sec:reachidea} and~\ref{sec:trainreachnet}, we described the ReachExplore approach and demonstrated the computation of the current frontier. 
% Central to ReachExplore is the idea of repeatedly increasing the frontier of reachable states during training. It is crucial to note that for the ReachExplore approach of gradually increasing the frontier of exploration to succeed, it must be ensured that in-distribution nearby goals are sampled before goals far away.
The idea of growing the set of reachable states during training is vital to ReaxhExplore. Hence, we leverage curriculum to ensure that in-distribution nearby goals are sampled before goals further away.
This naturally relates to the idea of a curriculum~\cite{curriculum}, and can be ensured by gradually increasing the maximum horizon $H$ of the episodes. So, we start with a horizon length of $H=H_0$ and gradually increase it to $H=NH_0$ during training, where $N$ is the total number of episodes.

In addition to this, while sampling goals we also ensure that the chosen goal before the start of every episode does not lie in any of the $p_k$ distributions, where $k\leq k^*$ corresponding to the calculated $k^*$. This implies that the chosen goal is beyond the current frontier, and hence would require exploration beyond what has been already visited.

%\subsection{Overall Algorithm}
    
%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{illustrative_figs/reachexplore_analysis_all.PNG}
%     \caption{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (c) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it randomly explores for $T-k^*$ steps. (b) shows the case when ReachExplore is not employed, and the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then randomly explores for $T-k$ steps. This is similar in principle to the high level idea of Go-Explore~\cite{goexplore} (a) shows the case when ReachExplore is not employed, and the agent starts doing random exploration for $T$ steps starting at the origin. This is similar in principle to SkewFit~\cite{skew}.}
%     \label{fig:analysis1}
% \end{figure}





%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{analysis.png}
%     \caption{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (a) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it randomly explores for $T-k^*$ steps. (b) shows the case when with probability $1-\chi$, the goal-reaching policy fails to take the agent to the frontier, and ends up somewhere within the already explored blue region. After that the  agent randomly explores for $T-k^*$ steps. Note that for computing the lower bound $L_1$, we consider the worst case when the circle of radius $\sqrt{T-k^*}$ is contained within the circle of radius $k^*$. (c) shows the case when ReachExplore is not employed, and the agent starts doing random exploration for $T$ steps starting at the origin.}
%     \label{fig:analysis}
% \end{figure}


==> 4-analysis.tex <==

\section{Analysis of ReachExplore: Intuition of deep exploration through average case analysis}
\label{sec:analysis}
In this section, we provide formal analysis of ReachExplore in a simplified, idealized, setting. Consider a 2D world with a single start location $\mathbf{z}_0$ and and let the goal be denoted by $\mathbf{z}_g$. Let $p_{k^*}$ denote the current frontier. Let $T$ denote the total time-steps in the current episode. 

We aim to show that using this time-step budget, the odds of exploring previously unvisited states farther away from the start state are higher when using ReachExplore, as compared to without using it. 
% Let $\chi$ denote the probability of the deterministic goal-conditioned policy reaching a goal state in $p_{k^*}$ in $k^*$. 
For simplicity, we assume the stochastic goal-reaching policy to be the policy of a random walker, and the deterministic goal-reaching policy to be near-optimal in the sense that given a target goal in $p_{k^*}$, and an initial state in the already explored region, it can precisely reach the  target location at the frontier with a high probability($\gg0$). 

For analysis, we define SkewFit~\cite{skew}, GoExplore~\cite{goexplore}, and ReachExplore in the above setting to be the following simplified schemes, and illustrate the same in Fig.~\ref{fig:analysis1}:
\begin{enumerate}

%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]

    \item \textbf{SkewFit:} The model that executes the stochastic policy for the entire length $T$ of the episode to reach goal $z_g$, and sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
    \item \textbf{GoExplore:} The model that first chooses a random previously visited intermediate latent goal state from the archive (not necessarily from the frontier $p_{k^*}$), executes a deterministic goal directed policy for say $k$ steps to reach the intermediate goal, and then executes the stochastic policy exploring for the next $T-k$ steps. For analysis, $0<k<k^*$. This is similar in principle to the idea of Go-Explore~\cite{goexplore}\footnote{Here, we refer to the intuition of Phase 1 of Go-Explore, where the idea is to ``select a state from the archive, go to that state, start exploring from that state, and update the archive." For illustration and analysis, we do not consider the exact approach of Go-Explore. In order to ``go to that state" Go-Explore directly resets the environment to that state, which is not allowed in our problem setting. Hence, in Fig.~\ref{fig:analysis1}, we perform the analysis with a goal-directed policy to reach the state. Also, since Go-Explore does not keep track of reachability, we cannot know whether the intermediate goal chosen can be reached in $k$ timesteps. But for analysis, we assume the intermediate goal is chosen from some $p_k$ distribution as described in Section~\ref{sec:reachidea}}. It also sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
    \item \textbf{ReachExplore:} The model that first chooses a state from the frontier $p_{k^*}$, executes a deterministic goal directed policy for say $k^*$ steps to reach the frontier, and then executes the stochastic policy exploring for the next $T-k^*$ steps.  It also sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
\end{enumerate}

%From the theory of hitting times in 2D random walks, we have the following result.
\begin{lemma}
For a random walk with unit step size in 2D (in a plane), the average distance away from a point (say, the origin) traversed in $t$ time-steps is $\sqrt{t}$.
\label{lemma:main}
\end{lemma}
\begin{proof}
The proof of is provided in the Appendix.
% In a plane, consider the sum of $t$ 2D vectors with random orientations. For convenience, we use the phasor notation, and so assume the phase of each vector to be random. Starting at some point (let's call it the origin $z_0$), we assume $t$ steps are taken in an arbitrary direction, which is equivalent to assuming that the angle $\theta$ of the phasors is uniformly distributed in $[0,2\pi)$. The position $z_t$ in the complex plane after $t$ steps is:
% $$ z_t = \sum_{k=1}^te^{i\theta_k}$$
% The square of the absolute value of $z_t$is:
% $$ |z_t|^2 = \sum_{k=1}^te^{i\theta_k}\sum_{m=1}^te^{-i\theta_m}
% = t + \underset{k=1,m=1,k\neq m}{\sum\sum^t}e^{i(\theta_k-\theta_m)}$$
% Now, we calculate the expected value of the $|z_t|^2$ variable by noting that since $\theta_k$ and $\theta_m$ are randomly sampled in $[0,2\pi)$ with uniform probability, the displacements $e^{i\theta_k}$ and $e^{i\theta_m}$ are random variables, so their difference corresponding to $\theta_k-\theta_m$ is also a random variable and has an expected value (mean) of $0$. Hence,
% $$<|z_t|^2> = t \implies |z_t|_{rms} = \sqrt{t}$$

% So, the average (root-mean-square) distance traversed after $t$ steps starting at some $z_0$ in the 2D plane is $\sqrt{t}$
\end{proof}
\noindent The subsequent results are all based on the above stated lemma and assumptions. 
\begin{lemma}
Starting at $z_0$ and assuming the stochastic goal-reaching policy to be a random walk, on average the SkewFit scheme will reach as far as $R_1 =\sqrt{T}$ at the most in one episode.
\end{lemma}
\begin{proof}
This follows directly from Lemma~\ref{lemma:main} by setting $t=T$, where $T$ is the max. number of timesteps in the episode.
\end{proof}
\vspace{-0.3cm}
% The lemma is illustrated in the first figure (1) of Fig.~\ref{fig:analysis1}, and is similar in principle to the basic SkewFit~\cite{skew} approach because at the start of each episode a stochastic goal-directed policy is rolled out from the initial state.

% In the second figure (2) of Fig.~\ref{fig:analysis1}, we consider a situation where a random previously visited intermediate latent goal state from the archive is chosen (not necessarily from the frontier $p_{k^*}$). Then the agent executes a deterministic goal directed policy for say $k$ steps to reach the intermediate goal, and then executes the stochastic policy exploring for the next $\sqrt{T-k}$ steps. For analysis, $0<k<k^*$. This is similar in principle to the idea of Go-Explore~\cite{goexplore}\footnote{Here, we refer to the intuition of Phase 1 of Go-Explore, where the idea is to ``select a state from the archive, go to that state, start exploring from that state, and update the archive." For illustration and analysis, we do not consider the exact approach of Go-Explore. In order to ``go to that state" Go-Explore directly resets the environment to that state, which is not allowed in our problem setting. Hence, in Fig.~\ref{fig:analysis1}(b), we perform the analysis with a goal-directed policy to reach the state. Also, since Go-Explore does not keep track of reachability, we cannot know whether the intermediate goal chosen can be reached in $k$ timesteps. But for analysis, we assume the intermediate goal is chosen from some $p_k$ distribution as described in Section~\ref{sec:reachidea}}. 

%In this case, the maximum average distance away from the origin traversed by the agent is atmost $r=\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$.
\begin{lemma}
Starting at $z_0$ and assuming the deterministic goal-deterministic policy to be near optimal (succeeds with a very high probability$>>0$), and the stochastic goal-reaching policy to be a random walk, on average GoExplore scheme will be bounded by $R_2 =\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$ in one episode.
\label{lemma:goexplore}
\end{lemma}
\begin{proof}
Since GoExplore first goes to a random previously visited state using the deterministic goal conditioned policy, from Fig~\ref{fig:analysis1} it is evident that the distance of such a state from the start state could be in the range $(0,k^*)$. Let this distance be $k$. Then, from Lemma~\ref{lemma:main}, the max distance on average traversed by the agent from $z_0$, if the intermediate state is at a distance $k$, can be given as:
$$ r_k = k + \sqrt{T-k}$$
Averaging over all the distance of all possible intermediate positions $k\in(0,k^*)$, we obtain the final averaged maximum distance reached by the agent in one episode as:
$$R_2 = \frac{1}{k^*}\sum_{k=0}^{k^*}(k+\sqrt{T-k})$$
%\vspace{-0.2cm}
\end{proof}
\vspace{-0.3cm}

% From the theory of hitting times in 2D random walks where at each timestep, the agent can move by 1 unit in any direction~\cite{hitting}, the average distance away from the origin traversed in $t$ steps is $\sqrt{t}$ \HB{Not a grid graph. This is for moving in free space, starting at a fixed point, where at each timestep the agent moves by 1 unit - so the agent can take discrete steps. We had discussed this on the whiteboard}. Hence, considering the stochastic policy (which for simplicity of analysis we considered to be a random walk), the maximum distance on average from $\mathbf{s}_0$ traversed in $T$ time-steps is $\sqrt{T}$. 



% While, if we employ ReachExplore, the maximum distance on average is atmost $k^* + \sqrt{T-k^*}$, as described in the following lemma:
\begin{lemma}
Starting at $z_0$ and assuming the deterministic  goal-conditioned policy to be near optimal (succeeds with a very high probability $>>0$), and the stochastic goal-reaching policy to be a random walk, on average ReachExplore will be bounded by $R_3 = k^* + \sqrt{T-k^*}$
\end{lemma}
\begin{proof}
In the proof for lemma~\ref{lemma:goexplore}, setting $k=k^*$ in the formula, for $r_k$ gives us the maximum average distance for ReachExplore as:
$$R_3 =  k^* + \sqrt{T-k^*}$$
%\vspace{-0.2cm}
\end{proof}
\vspace{-0.3cm}
\begin{theorem}
$R_3>R_2$ $\forall k^*\in[1,T)$ and $R_3>R_1$ $\forall k^*\in[1,T)$. i.e. After the frontier $k^*$ is sufficiently large, the maximum distance from the origin reached by ReachExplore is more than both GoExplore and SkewFit.
\label{lemma:final}
\end{theorem}
\begin{proof}
We provide the proof of this in the Appendix.
\end{proof}

% In the Appendix we show that for values of $k^*>T/4$, $k^* + \sqrt{T-k^*}$ is always greater than  $r=\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$.
\noindent Theorem~\ref{lemma:final} is the main result of our analysis and it intuitively suggests the effectiveness of deep exploration guaranteed by ReachExplore. This is shown through a visualization in Fig.~\ref{fig:analysis1}. 

In Fig.~\ref{fig:analysis1}\,(2) and (3), we assume the deterministic policy succeeds with high probability($\gg0$), which is usually the case after sufficient training iterations in off-policy Q-learning. It can be easily seen that if $k^*$ increases during training (i.e. the reachable frontier expands), then after a finite number of interactions with the environment, we will have $k^*>\sqrt{T}$. We ensure that this happens because of the implicit curriculum on horizon length, and the sampling of goals beyond the current reachable frontier at the start of every episode.




% \subsection{Fast(er) coverage guarantees through average case analysis (Sec to be commented)}
% In this section, we provide theoretical justifications for why applying the ReachExplore trick ensures faster coverage. Consider a 2D world with a single start location $\mathbf{s}_0$ and and let the goal be denoted by $\mathbf{s}_g$. Let $k^*$ denote the current frontier. Let $T$ denote the total number of time-steps in the current episode. We sim to show that using this time-step budget, the odds of exploring previously unvisited states are higher when using ReachExplore, as compared to without using it. Let $\chi$ denote the probability of the deterministic goal-conditioned policy reaching a goal state in $p_{k^*}$ in $k^*$. For simplicity, we assume the stochastic goal-reaching policy to be the policy of a random walker. 

% From the theory of hitting times in 2D random walks~\cite{hitting}, the average distance away from the origin traversed in $t$ steps is $\sqrt{t}$. We consider two cases:
% \begin{itemize}
%     \item The agent employs ReachExplore to go to the frontier at a radius of $k^*$, using the deterministic goal-conditioned policy and then perform a random walk with the remaining $T-k^*$ steps. During this random walk the agent will go upto a distance of $\sqrt{T-k^*}$ in any direction. Let the total area traversed on average be $A_1$.
%     \item The agent does not employ ReachExplore and executes the default stochastic goal conditioned policy (which we assumed for simplicity to be the policy of a random walk) from the start state $\mathbf{s}_g$ and continues for  $T$ time-steps, thus ending up on an average somewhere in a circle of radius $\sqrt{T}$ centered at $\mathbf{s}_{k^*}\sim p_{k^*}$. Let the total area traversed on average be denoted by $A_2$, and we have $A_2=\pi T$.
% \end{itemize}
% We have the following lower bound on $A_1$ (Fig.~\ref{fig:analysis})
% $$A_1 \geq \chi\left(\pi (k^*)^2 + \frac{1}{2}\pi (T - k^*)\right) + (1-\chi)\pi (k^*)^2 $$
% Let us denote the above lower bound by $L_1$. To show $A_1>A_2$ it is enough to show that $L_1-A_2>0$. Let us consider the difference $L_1-A_2$:
% $$L_1-A_2 = \pi(k^*)^2 -\frac{1}{2}\pi\chi k^* + \frac{1}{2}\pi (\chi-2)T$$
% Treating the above as a quadratic expression in the variable $x=k^*$, we note that the value of $Ax^2+Bx+C>0$ $\forall x$ when $B^2-4AC < 0$. For our problem, $$B^2-4AC = \frac{1}{4}\pi^2\chi^2 - 2\pi^2T(\chi-2)=2\pi^2(\frac{1}{8}\chi^2-T\chi+2T)$$
% Since $\chi\in(0,1)$ and $T>1$, the value of $B^2-4AC$ is always greater than $0$. So, by analyzing the roots of the equation, 
% $$\pi(k^*)^2 -\frac{1}{2}\pi\chi k^* + \frac{1}{2}\pi (\chi-2)T = 0$$
% we have 
% $$\forall k^* >\frac{1}{4}\chi + \frac{1}{2}\sqrt{\frac{1}{4}\chi^2 -2T\chi + 4T}$$
% $L_1-A_2>0$ and so $A_1>A_2$. This result tells us that there is a certain value of frontier $k^*<T$ such that when we have achieved this frontier, it is beneficial to perform committed exploration via the ReachExplore approach. Now, in each iteration of training, since we sample goals beyond the currently reachable frontier $k^*$ (Section~\ref{sec:approach}C), so the value of $k^*$ will always increase during training. Hence, the above value will be reached at some point during training. 


==> 5-experiments.tex <==

\section{Experiments}
Our experiments aim to understand the following questions: (1) How does ReachExplore compare to existing state-of-the-art exploration baselines, in terms of faster convergence and higher cumulative success? 
%(2) How does keeping track of reachability ensure faster convergence and deep exploration required to solve long-horizon robotic tasks directly from images?
(2) How does ReachExplore scale as task complexity increases?
(3) Can ReachExplore scale to tasks on a real robotic arm?

\subsection{Environments}
We consider the image-based and state-based environments illustrated in Fig.~\ref{fig:sim_envs}. In case of image-based environments, the initial state and the goal are both specified as images. In case of state-based environments, the initial state and the goal consists of the coordinates of the object(s), the position and velocity of different components of the robotic arm, and other details as appropriate for the environment (Refer to the Appendix for details). In both these cases, during training, the agent does not have access to any oracle goal-sampling distribution. In Fig.~\ref{fig:sim_envs}, (b), and (c) are configured to be \textit{sparse-reward} settings, where the reward is $1$ only when the agent $solves$ the goal and is $0$ otherwise. To define when a goal is $solved$, for each environment there is a certain threshold distance between the agent's final state and the goal state, the details of which are mentioned in the appendix. All the other environments in Fig.~\ref{fig:sim_envs} use \textit{only} a latent distance based reward during training (reward $r=-||z_t-z_g||_2$; $z_t$ is the agent's current latent state and $z_g$ is the goal latent state), and have no access to ground-truth simulator states. 

% \begin{figure}[t]
% \centering
%         \begin{subfigure}[b]{0.5\columnwidth}
%               \centering             \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/one.png}
%     %\caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%          \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/five.png}
%   % \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%     % \includegraphics[width=0.7\columnwidth]{illustrative_figs/one.png}
%     \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%           \begin{subfigure}[b]{0.5\columnwidth}
%               \centering             \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/fetch_one.png}
%     %\caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%          \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/fetch_final.png}
%   % \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%     % \includegraphics[width=0.7\columnwidth]{illustrative_figs/one.png}
%     \caption{Fetch Slide}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
        
       
%      \caption{Illustrations of all the simulation environments evaluated in this paper, with example initial and goal images.}  
%  \label{fig:sim_results}
% \end{figure}
 \begin{figure}
     \centering
     \includegraphics[width=0.99\columnwidth]{arxiv_version/figures/reachexplore_allenvs.png}
     \caption{Illustrations of all the environments evaluated in this paper, with example initial (left) and goal (right) images.  Each environment we consider is meant to demonstrate scaling of the proposed approach to different settings: image-based goals, state-based goals, continuous action spaces, discrete action spaces, different dynamics (point mass, Fetch robot, Sawyer robot, Franka Panda robot), increasing task complexity (Push to Push and Reach), and applicability to a real robot. Details are in the Appendix. }
     \label{fig:sim_envs}
     \vspace*{-0.4cm}
 \end{figure} 
 
 
\begin{figure*}[h!]
\centering
 \begin{subfigure}[b]{0.60\textwidth}
               \centering
    \includegraphics[width=\textwidth]{illustrative_figs/results_figs/all_results.png}
    \caption{Comparative results on simulation environments}
    \label{fig:quantitative}
        \end{subfigure}\hspace*{-0.1cm}
                 \begin{subfigure}[b]{0.40\textwidth}
               \centering
    \includegraphics[width=\textwidth]{illustrative_figs/results_figs/sim_qualitative.png}
    \caption{Qualitative results showing the goal image on the left, and rendered images of the final states reached by SkewFit and ReachExplore for two evaluation runs in two different environments.}
    \label{fig:qualitative}
        \end{subfigure}

            %\quad
     \caption{Comparison of ReachExplore and SkewFit on an ensemble of vision-based and state-based simulation environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are with respect to three random seeds. It is important to emphasize that the training proceeds in a completely self-supervised manner (for both ReachExplore and SkewFit), without assuming any access to the oracle goal sampling distribution. The results reported are for evaluations on test suites (initial and goal images are sampled from a test distribution unknown to the agent) as training progresses. Although the ground-truth simulator states are not accessed during training (for (a), (c), (d), (e), and (f)), for the evaluation reported in these figures, we measure the ground truth $L_2$ norm of the final distance of the object/end-effector (as appropriate for the environment) from the goal location.  In (f), we evaluate the final distance between the (puck+end-effector)'s location and the goal location. In (c), success is measured as +1 if the agent reaches the final green goal square in the grid, and 0 otherwise. In (b), success is measured as +1 if the puck reaches within 2cm of the goal location. In (a), (d), (e), and (f), lower is better. In (b) and (c), higher is better.}  
 \label{fig:sim_results}
 \vspace*{-0.6cm}
\end{figure*}

 
%  Each environment we consider is meant to demonstrate scaling of the proposed approach to different settings: image-based goals, state-based goals (Fetch slide), continuous action spaces, discrete action spaces (Locked door navigation), different dynamics (point mass, Fetch robot, Sawyer robot, Franka Panda robot), and applicability to a real robot (Franka Panda).
\begin{enumerate}

%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]
  
  \item \textbf{Pointmass Navigation} (\textit{Image-based}): A pointmass object must be navigated from an initial location to a goal location in the presence of obstacles. The agent must plan a temporally extended path that would occassionally involve moving away from the goal. This is a 2D environment with a continuous action space, and the agent has access to images from a top-down view. 
   \item \textbf{Fetch Slide} (\textit{State-based}): A Fetch robot arm must be controlled to push and slide a puck on the table such that it reaches a certain goal location. It is ensured that sliding must happen (and not just pushing) because the goal location is beyond the reach of the arm's end-effector. We make this environment significantly difficult by reducing the default friction coefficient by a factor of 2. The agent has access to state information - the position $(x,y,z)$ and velocity $(v_x,v_y,v_z)$ of its end-effector. 
   \item \textbf{Gridworld Locked Door Navigation} (\textit{Image-based}): A point agent navigates a maze to pick up a key, open a locked door, and navigate to a goal location on the other side of the door. This is a 2D environment, and the agent has access to a top-down view. At each time-step, the agent has the option to choose from six actions (so discrete action space).
   \item \textbf{Sawyer Pick} (\textit{Image-based}): A Sawyer robot arm must be controlled to pick a puck from a certain location and lift it to a target location above the table. The agent has access to images from a camera mounted on the arm.
   \item \textbf{Sawyer Pick and Place} (\textit{Image-based}): A Sawyer robot arm must be controlled to pick a puck from a certain location and place it on a target location on the table. A wall as shown in Fig.~\ref{fig:sim_envs} ensures that simply pushing cannot get the puck to the goal location. The agent has access to images from a camera mounted on the arm.
     \item \textbf{Sawyer Push} (\textit{Image-based}): A Sawyer robot must push a puck to a certain location with the help of its end-effector. The agent has access to images from a camera mounted on the arm.
    \item \textbf{Sawyer Push and Reach} (\textit{Image-based}): A Sawyer robot arm is controlled to push a puck to a target location, and move its end-effector to a (different) target location. The agent has access to images from a camera mounted on the arm.
    \item \textbf{Franka Panda Peg in a Hole} (\textit{State-based; Real robot}); A real Franka Panda arm must be controlled to place a peg in a hole. The agent is velocity controlled and has access to state information - the position $(x,y,z)$ and velocity $(v_x,v_y,v_z)$ of its end-effector. 
\end{enumerate}
\subsection{Setup}
We use the Pytorch library~\cite{pytorch1,pytorch2} in Python for implementing our algorithm, and ADAM~\cite{adam} for optimization. We use SAC (Soft Actor-Critic)~\cite{sac} as the base off-policy RL algorithm for policy learning. We consider two recent state-of-the-art exploration algorithms, namely Skew-Fit~\cite{skew}, and Go-Explore~\cite{goexplore} as our primary baselines for comparison. For both these baselines, for consistency, we use SAC for policy-learning.  Based on the original implementation of Go-Explore~\cite{goexplore}, we create a version using SAC as the base policy and employing the Go-Explore trick which we use as our baseline.

For training, we train ReachExplore and the baselines in a completely unsupervised manner, without access to any oracle goal-sampling distribution. In addition, in the image-based environments, during training the agent does not have access to any prior information about the state-space. In order to 
\textit{evaluate} the performance of the algorithms, we sample goal images from a uniform distribution over valid images and report the final distance of the agent to the corresponding states in simulator. This method of evaluation, although applicable only in simulation, is a reliable metric for RL with vision-based goals, as described in prior works~\cite{rig,skew}. It is important to note that we access the simulator states only for \textit{evaluation} - not for training (except for (b), and (h) in Fig.~\ref{fig:sim_envs}). 

%During training, to measure reward, we compute the $L_1$ norm of the difference between the agent's latent state $z_t$ and the goal latent state $z_g$.
% \begin{figure*}[h!]
% \centering
%  \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pointmassfinal.png}
%     \caption{Pointmass Navigation (Image)}
%     \label{fig:pointmass}
%         \end{subfigure}\hspace*{-0.2cm}
%                  \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pickplacefinal.png}
%     \caption{Sawyer Pick and Place (Image)}
%     \label{fig:pickplace}
%         \end{subfigure}
        
        
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/push_easy_final.png}
%     \caption{Sawyer Push (Image)}
%     \label{fig:pusheasy}
%         \end{subfigure}% \\
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pushreachfinal.png}
%     \caption{Sawyer Push and Reach (Image)}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%         %\hspace*{-0.5cm}
        
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/gridlocked_doorfinal.png}
%     \caption{Gym Locked Door Navigation (Image)}
%     \label{fig:fetchslide}
%         \end{subfigure}\hspace*{-0.2cm}
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/fetchslide_final.png}
%     \caption{Fetch robot - Slide (State)}
%     \label{fig:fetchslide}
%         \end{subfigure}
%             %\quad
%      \caption{Comparison of ReachExplore and SkewFit on an ensemble of vision-based and state-based simulation environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are with respect to three random seeds. It is important to emphasize that the training proceeds in a completely self-supervised manner (for both ReachExplore and SkewFit), without assuming any access to the oracle goal sampling distribution. The results reported are for evaluations on test suites (initial and goal images are sampled from a test distribution unknown to the agent) as training progresses. Although the ground-truth simulator states are not accessed during training (for (a), (b), (c), (d), and (e)), for the evaluation reported in these figures, we measure the ground truth L2 norm of the final distance of the oject/end-effector (as appropriate for the environment) from the goal location. In (e), success is measured as +1 if the agent reaches the final green goal square in the grid, and 0 otherwise. In (f), success is measured as +1 if the puck reaches the goal location with a tolerance threshold of $0.1\%$. In (a), (b), (c), and (d), lower is better. In (e) and (f), higher is better.}  
%  \label{fig:sim_results}
% \end{figure*}




\subsection{Results}
\noindent\textbf{ReachExplore achieves higher success during evaluation in reaching closer to the goals compared to the baselines}
Fig.~\ref{fig:sim_results} shows comparisons of ReachExplore against the baseline algorithms on all the robotic simulation environments. It is evident that ReachExplore performs significantly better than all the baselines. The image based environments Sawyer Pick and Place, and Sawyer Push and Reach are challenging because there are two components to the overall task. The significant performance improvement of ReachExplore over the baselines can be can be clearly seen in Fig.~\ref{fig:sim_results}.

 The pointmass navigation environment is challenging because during evaluation, we choose the initial position to be inside the U-shaped area, and the goal location to be outside it, and the agent does not know this apriori. So, during training the agent must learn to set difficult goals outside the black arena and must try to solve them. This requires deep committed exploration, and as shown in Fig.~\ref{fig:quantitative}, ReachExplore succeeds in achieving this.

In addition to the image based goal environments, we consider a challenging state-based goal environment as proof-of-concept to demonstrate the effectiveness of ReachExplore. In Fig.~\ref{fig:quantitative} we see that for the slide task on a Fetch robot, ReachExplore achieves much higher success rate compared to the baselines in pushing the puck with the right amount of force in the right direction such that it stops exactly at the goal location. In order to succeed in this task, the agent must acquire an implicit estimate of the friction coefficient between the puck and the table top, and hence must learn to set goals close and solve them before setting goals farther away. 


\noindent\textbf{ReachExplore scales to tasks of increasing complexity}
From Fig.~\ref{fig:quantitative}, we see that ReachExplore performs comparably to its baselines. The improvement of ReachExplore over SkewFit is not statistically significant. However, in the task of Push and Reach (Fig.~\ref{fig:quantitative}) we observe significant improvement of ReachExplore over SkewFit. The baselines succeed either in the push part of the task or the reach part of the task but not both, suggesting overly greedy policies without long term consideration (Refer qualitative results in Fig.~\ref{fig:qualitative}).This suggests the effectiveness of ReachExplore in scaling to a difficult task that requires more temporal abstraction. This benefit is probably because ReachExplore performs two staged exploration, which enables it to quickly discover regions that are farther away from the initial state given at the start of the episode. 
%Since the agent receives a +1 reward only when it pushes the puck to the desired location and brings the end-effector to its desired location (i.e. sparse reward), focusing the thrust of exploration on previously unexplored states is crucial to discover trajectories that successfully solve the task. 

We observe similar behaviors of scaling to more complicated tasks by looking at the results of the Pick task (in Appendix) and the Pick and Place task in Fig.~\ref{fig:quantitative}. While the pick task can be solved even by simple strategies like pushing the object to the desired location, to solve the pick and place task, the agent must actually discover trajectories that pick that object and place in at its desired location over the other side of the fence. Discovering such successful trajectories in the face of only latent rewards, and no ground-truth reward signals further demonstrates the need for committed exploration. In the Pick and Place experiment, the baselines are able to either successfully pick the object but not place it correctly or try to push the object unsuccessfully to the goal location (Fig.~\ref{fig:qualitative}). In contrast, ReachExplore succeeds in both parts of the sequential task.
  

% \begin{figure*}[t]
% \centering
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pushreach_eval1.png}
%     \caption{Sawyer Push and Reach (Image)}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pickplace_final.png}
%     \caption{Sawyer Pick and Place (Image)}
%     \label{fig:pickplace}
%         \end{subfigure}
        
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pointmass.png}
%     \caption{Pointmass Navigation (Image)}
%     \label{fig:pointmass}
%         \end{subfigure}
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{anglediff_compare.png}
%     \caption{Sawyer Door opening (I)[rev. legend]}
%     \label{fig:avg_r_lf}
%         \end{subfigure}
        
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{fetchslideresult.png}
%     \caption{Fetch robot - Slide (State)}
%     \label{fig:fetchslide}
%         \end{subfigure}
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{fetchesults.png}
%     \caption{Fetch robot - Reach (State)}
%     \label{fig:results}
%         \end{subfigure}
%     %\quad
%      \caption{Comparison of ReachExplore and SkewFit on an ensemble of vision-based and state-based environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are wrt 3 seeds in (a), (d), and (e), and wrt 2 seeds in (b), (c), and (f). It is important to emphasize that the training proceeds in a completely unsupervised manner (for both ReachExplore and SkewFit), without assuming any access to the oracle goal sampling distribution.}  
%  \label{fig:sim_results}
% \end{figure*}
  

  
\noindent\textbf{ReachExplore scales to tasks on a Real Franka Panda robotic arm} Fig.~\ref{fig:panda} shows results for ReachExplore on a peg-in-a-hole evaluated on the Franka Panda arm. Here the objective is to insert a peg into a hole, an illustration of which is shown in Fig.~\ref{fig:sim_envs}.  The reward function is defined to be the negative of the distance from the center of bottom of the peg to the center of the bottom of the hole. There is an additional heavy reward penalty for `collision' and a mild penalty for `contact.' The home position of the panda arm (to which it is initialized) is such that the distance from the center of the bottom of the peg to the center of the bottom of the hole is 0.35 meters. The heavy penalty for collision is -10 and the mild penalty for contact is -1. We can observe from Fig.~\ref{fig:panda} and the video in supplementary that ReachExplore successfully solves the task while the baseline GoExplore does not converge to the solution. This demonstrates the applicability of ReachExplore on a real robotic arm.

% \begin{figure}
%   \centering
%  \begin{subfigure}[b]{0.7\columnwidth}
%               \centering
%     \includegraphics[width=\columnwidth]{results_figs/franka_real_arm.png}
%     \caption{Reaching task (State-based)}
%     \label{fig:pointmass}
%         \end{subfigure}%\hspace*{-0.2cm}
%                  \begin{subfigure}[b]{0.2\columnwidth}
%               \centering
%     \includegraphics[width=\columnwidth]{illustrative_figs/pandaarm.png}
%     \caption{Panda arm}
%     \label{fig:pickplace}
%         \end{subfigure}
%       \caption{Results of a Reaching task on the real Franka Emika Panda arm. The goal is specified as a tuple of coordinates (x,y,z) to be reached. The state consists of the position and velocities of the end-effector. Higher is better.}
%     \label{fig:panda}
%     \vspace*{-0.2cm}
% \end{figure}


\begin{figure}
   \centering
    \includegraphics[width=0.85\columnwidth]{illustrative_figs/results_figs/panda_peg.png}    
    \caption{Results of a Peg-in-a hole task on the real Franka Emika Panda arm. The evaluation metric on the y-axis is the distance ($L_2$ norm) of the center of the bottom of the hole from the center of the bottom of the peg. The state consists of the position and velocities of the end-effector. Lower is better}
    \label{fig:panda}
     \vspace*{-0.5cm}
  \end{figure}
   

==> 6-related_works.tex <==
\vspace*{-0.35cm}
\section{Related Works}


\noindent \textbf{Vision-based RL for Robotics.} Recent works have investigated vision-based learning of RL policies for specific robotic tasks like grasping~\cite{grasping1,grasping2}, pushing~\cite{pushing2,pushing1}, and navigation~\cite{navigation2,navigation1}, however relatively few prior works have considered the problem of learning policies in a completely self-supervised manner~\cite{rig,skew}. A recent paper~\cite{avi} considers RL directly from images, for general tasks without engineering a reward function, but involves a human in the loop. Some other prior works learn latent representations for RL in an unsupervised manner which can used as input to the policy, but they either require expert demonstration data~\cite{upn,demo2}, or assume access to ground-truth states and reward functions during training~\cite{worldmodels,ground2,ground3}. RIG~\cite{rig} proposes a general approach of first learning a latent abstraction from images, and then planning in the latent space, but requires data collected from a randomly initialized policy to design parametric goal distributions.  In addition, niether approaches do not guarantee any notion of exploration or coverage that is required for solving difficult temporally-extended tasks from minimal supervision - in particular with goals specified as raw images.



\noindent \textbf{Goal-conditioned Policy Learning.}
While traditional model-free RL algorithms are trained to succeed in single tasks~\cite{td3,sac,ppo,trpo}, goal-conditioned policy learning holds the promise of learning general-purpose policies that can be used for different tasks specified as different goals~\cite{kaelbling1993learning,her,rig,arc}. However, most goal-conditioned policy learning algorithms make the stronger assumption of having access to an oracle goal sampling distribution during training~\cite{kaelbling1993learning,her,universal,leap}. A recent paper~\cite{arc} proposes an algorithm to create dynamics-aware embeddings of states, for goal-conditioned RL, but it is not scalable to images as goals (instead of ground-truth states).  

Some other prior works do not assume access to an oracle goal-sampling distribution, but sample goals based on some ad-hoc heuristics like learning progress~\cite{learnprogress1,learnprogress2}, how off-policy the goal is~\cite{offpolicy} or sample goals randomly from the learn latent distribution over image observations~\cite{rig}. Skew-Fit~\cite{skew} adds structure to the goal-sampling process by sampling goals in the latent space such that the entropy over the learned distribution over states is maximized, but provides no guarantee of coverage/exploration in finite time. 





\noindent \textbf{Exploration for RL.} Skew-fit~\cite{skew} proposes a novel entropy maximizing objective that ensures gradual coverage in the infinite time limit. In addition, it does not incorporate any notion of commitment during exploration, which is needed to discover complex skills for solving temporally extended tasks in finite time. Go-Explore~\cite{goexplore} addresses this issue to some extent by keeping track of previously visited states in the replay buffer, and at the start of each episode, re-setting the environment to an arbitrary previously visited state, and continuing exploration from there. However, this approach is fundamentally limited because it assumes the environment is re-settable, which is not always feasible on a real robot. In addition, re-setting to an \textit{arbitrary} previously visited state is not guaranteed to ensure deep exploration.

On the contrary, novelty/surprise based criteria have been used in many RL applications like games, and mazes~\cite{curiosity,count,rupam}. In~\cite{curiosity}, a curiosity based intrinsic reward signal is used in addition to the external reward in order to encourage the RL agent to visit previously unvisited states. In~\cite{count}, the authors explicitly keep track of the state visitation frequencies and reward the agent for visiting states with less visitation frequency. VIME \cite{vime} considers information gathering behaviors to reduce epistemic uncertainty on the dynamics model. 

%Although these methods are general in that novelty bonuses are not %task-specific, there is no mechanism to distill the learned %knowledge from visiting novel states into adaptive policies that can %adapt to diverse goals at test-time. The policies learned are %reactive because the knowledge gained by visiting $novel$ states is %quickly forgotten when other states become more novel.

\noindent \textbf{Reachability and Curriculum Learning.} Our method is related to curriculum learning approaches in reinforcement learning \cite{approximate_hjb, curriculum_held, ELMAN199371, openai2019solving, curriculum_bengio, racaniere2019automated} whereby learning easier tasks is prioritized over hard tasks, as long as measures are taken to avoid forgetting behaviors on old tasks.   

\noindent \textbf{Frontier-based Exploration for Robot Mapping.} Finally, ReachExplore is intuitively similar to a large body of classic work on robot mapping, particularly frontier-based exploration approaches \cite{frontier_based_exploration, frontier_based_exploration_multirobot, frontier_based_exploration_holz}.


==> 7-conclusion.tex <==
 \vspace*{-0.2cm}
\section{Conclusion} 
 \vspace*{-0.2cm}
\label{sec:conclusion}
In this paper we proposed an algorithm for committed exploration, by keeping track of the frontier of reachable states, and during the start of every episode, executing a deterministic goal-conditioned policy to reach the current frontier, followed by executing a stochastic goal-conditioned exploration policy to reach the goal. The proposed approach can work directly over image-based observations and goal specifications, does not require any reward signal from the environment during training, and is completely self-supervised in that it does not assume access to the oracle goal-sampling distribution for evaluation. Through experiments on eight environments with varying characteristics, task complexities, and temporal abstractions, we demonstrate the efficacy of the proposed approach over state of the art exploration baselines.


==> arxiv_version/1-introduction.tex <==
\section{Introduction}
\label{sec:intro}  

%Reinforcement Learning (RL) enables agents to learn complex skills by interacting with the environment, alleviating the need for manual engineering of behavioral skills.
Efficient exploration is one of the central open challenges in Reinforcement Learning (RL), and a key requirement for learning optimal policies, particularly in sparse-reward and long-horizon settings, where the optimization problem is difficult to solve, but easy to specify. We show that discovering policies for  these settings benefits significantly from autonomous goal-setting and exploration, which requires keeping track of what regions of the state-space have been sufficiently explored and can be reached via planning, and what regions remain unknown. In this paper we present an exploration method that keeps track of reachable regions of state space and naturally handles the exploration-exploitation dilemma in sequential decision-making for unknown environments~\cite{varibad,goexplore}, while being practical in real robotics settings. \HB{General introduction}


%One of the central challenges in Reinforcement Learning (RL) is to learn large general purpose repertoires of behaviors that can be used for solving  complex tasks, without undertaking the time-consuming and potentially intractable job of learning each behavior separately. Such self-supervised discovery of composable behaviors for solving temporally extended tasks requires agents to autonomously explore the environment, keep track of what regions of the state-space have been sufficiently explored and can be reached, and hence naturally relates to the exploration-exploitation dilemma in sequential decision-making in unknown environments~\cite{varibad,goexplore}. \HB{General introduction}



For learning to plan in \textit{unknown} environments, appropriately trading off exploration i.e. learning about the environment, and exploitation i.e. executing promising actions is the key to successful policy learning. The necessity for this trade-off is more pertinent when we want to train agents to learn autonomously in a self-supervised manner such that it is able to solve goals sampled from an unknown distribution during evaluation. In this setting, during training, the agent must practice reaching self-specified random goals~\cite{rig}. However, trying to specify goals through exact states of objects in the environment will require a combinatorially large representation, for explicitly randomizing different variables of the states~\cite{avi,rig}. On the contrary, raw sensory signals, such as images can be used to specify goals, as has been done in recent goal-conditioned policy learning algorithms~\cite{rig,upn,skew}\HB{In the previous two lines I am trying to motivate the need for learning from images even in simulation. In the real environment it is clear why we want to use images as input - we cannot describe the environment state exactly.}. This paper tackles the question of how should an autonomous agent balance exploration and exploitation for goal-directed robotic tasks while learning directly from images, with no access to the ground-truth parameters of the environment during training. 
%Specifically, we focus our attention to the problem of keeping track of the frontier of reachable states, and using latent space reachability measures to devise efficient exploration algorithms in the above setting. \HB{The problem being considered. It is slightly vague because I intended this to be a description of the problem, not the solution. I would appreciate help to make it more crisp though.}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{illustrative_figs/reachexplore_idea_final.png}
    \caption{Our method encourages reaching the current frontier of reachable states with a deterministic policy, and performing goal-directed exploration beyond it with a stochastic policy. In this illustration, the yellow volume corresponds to end-effector positions for the currently reachable frontier corresponding to the shown initial state.}
    \label{fig:firstfig}
    \vspace*{-0.7cm}
\end{figure}
% In this paper, we attempt to mitigate the exploration-exploitation tradeoff in self-supervised learning of goal-conditioned policies directly from images by keeping track of the frontier of reachable states, and performing committed exploration. 


\begin{figure*}[h!]
\centering
   \hspace*{-0.9cm}
        \begin{subfigure}[b]{0.7\textwidth}
               \centering
    \includegraphics[width=0.9\textwidth]{arxiv_version/figures/ReachExploreMainfig_updated.png}
    \caption{Forward pass of the proposed approach}
    \label{fig:reachidea}
        \end{subfigure}% \\
        \hspace*{-0.8cm}
         \begin{subfigure}[b]{0.37\textwidth}
               \centering
    \includegraphics[width=\textwidth]{reachnet.png}
    \caption{Reachability Network}
    \label{fig:reachnet}
        \end{subfigure}                 %\quad
     \caption{(a) An overview of our method on the Sawyer Push and Reach task. The initial and goal images are encoded by the encoder of the VAE into latents $z_0$ and $z_g$ respectively. Random states are sampled from the currently learned manifold of the VAE latent states, and are used to infer the current frontier $p_{k^*}$ as described in Section~\ref{sec:reachidea}. The currently learned deterministic policy is used to reach a state in the frontier $z^*$ from the initial latent state $z_0$. After that, the currently learned stochastic policy is used to reach the latent goal state $z_g$. A reconstruction of what the latent state in the frontier $z^*$ decodes to is shown. For clarity, a rendered view of the actual state $z^*$ reached by the agent is shown alongside the reconstruction. (b) A schematic of the reachability network used to determine whether the latent state $z_i$ ($state_i$) is reachable from the latent state $z_j$ ($state_j$) in $k$ time-steps. The reachability vector $\mathbf{k}$ consists of a vector of the same size as $z_i$ and $z_j$ with all its elements being $k$. The output $0$ indicates that state $z_i$ is not reachable from state $z_j$.} 
 \label{fig:mainfig}
 \vspace*{-0.7cm}
\end{figure*}
The main idea of our approach is to maintain and gradually expand the frontier of reachable states by trying to reach the current frontier directly without exploring i.e. by executing a deterministic goal-conditioned policy, and exploring from beyond the current frontier in order to reach the goal by executing a stochastic goal-conditioned policy (Fig.~\ref{fig:firstfig}). In order to achieve this, we encourage the agent to sample goals closer to the start state(s) before sampling goals that are farther away, by appropriately querying the reachability network. Planning directly in the pixel-space is not meaningful. For example, computing rewards as the pixel-wise distance between two images does not necessarily correspond to a semantically meaningful correlation with respect to how close the two ground-truth states actually are~\cite{upn,rig}. Hence, we learn a latent abstraction from images, and plan in the latent space. We train a reachability network that learns whether a latent state is currently reachable from another latent state in $k$ time-steps ($k$ varies from $1$ to the maximum length of the horizon), and use this network to compute the current frontier of reachable states given a random initial start state during training. While training the goal-conditioned policy to reach a goal latent state (corresponding to a goal image), we first execute the deterministic policy trained so far to reach a latent state at the frontier (\textit{commitment}), and then execute the stochastic policy from beyond the frontier to reach the goal (\textit{exploration}). We refer to this procedure of commitment to reach the frontier and exploring beyond it as \textit{committed exploration} required for solving temporally abstracted tasks. \HB{The proposed approach. Every episode in training hasa two phases - execute deterministic policy to reach frontier. Explore beyond frontier while trying to reach goal. I don't mean to say the 2nd phase here is "deep exploration". The overall scheme of having this two stage approach is enforcing deep exploration - to discover temporally abstracted winning sequences of actions that solve the task - this process happens completely at the end of training, when the reachable frontier = real frontier.}

%In order to impose this curriculum over the self-supervised sampling of goals during training, we gradually increase the max. horizon length of episodes during successive epochs of training. 

In summary, this paper makes the following contributions:
\begin{enumerate}
%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]
 \item We propose a dynamics-aware latent space reachability network.
 \item We devise a policy learning scheme using the reachability network that combines deterministic and stochastic policies for committed exploration. 
 \item We empirically evaluate the proposed approach  in a range of both image-based, and state-based simulation environments, and in a real robot environment. We demonstrate an improvement of $20\%$ on average compared to state-of-the-art exploration baselines. 
\end{enumerate}


%Since the proposed approach explicitly keeps track of reachability for committed exploration, we call our approach ReachExplore. 
% Through detailed experimentation across image-based simulation environments, a state-based simulation environment, and a real-world robotic environment, we show that ReachExplore successfully solves difficult temporally-extended tasks by achieving much higher rewards and converging with much less interactions with the environment as compared to state-of-the art image-based exploration methods. \HB{image based methods.} \HB{A brief highlight of the results. To put in specifics if needed later.}

==> arxiv_version/2-preliminaries.tex <==
\section{Problem Setup and Background}
% In this section, we elaborate on the key concepts and paradigms that relate to the proposed approach, and lay out the mathematical notations for the rest of the paper.
\label{sec:prelim}

\subsection{Problem Setup}
In standard model-free RL, the objective is to learn a policy $\pi(\cdot)$ as a function of the current state of the world $s_t$ (this could be a latent abstraction state as well) that outputs an action $a_t=\pi(s_t)$ to be executed in the environment, such that the expected sum of discounted returns from the environment $R_t=\mathbb{E}_{\pi(a|s),p(s'|s,a)} [\sum_{i=t}^T\gamma^{(i-t)}r(s_i,a_i,s_{i+1})]$ is maximized. Here, $a\in\mathcal{A}$, $s\in\mathcal{S}$, $\gamma$, and $r(\cdot)$ respectively denote an action in the set of actions, a state in the set of states, the discount factor, and the reward function.

\noindent \textbf{ Goal-conditioned policies} This formulation is insufficient when we want to optimize expected returns with respect to different goals that can be specified at test-time. Hence, explicitly conditioning the policy on the goal $s_g$ that must be achieved in the current episode, $a_t=\pi(s_t;s_g)$, and optimizing the expected sum of discounted rewards over different goals $s_g$ sampled from the set of goals $s_g\sim\mathcal{G}$, $R_t=\mathbb{E}_{\pi(a|s;s_g),p(s'|s,a)} [\sum_{i=t}^T\gamma^{(i-t)}r(s_i,a_i,s_{i+1};s_g)]$  is a common method of learning policies that can be adapted to different goals at test time~\cite{her}.

\noindent \textbf{Self-supervised learning to solve goals} We consider the setting of learning directly from images, such that the the goals are specified as images to the policy. Also, the setting is self-supervised in the sense that during training, we do not have access to any oracle goal-sampling distribution from which goals will be sampled at test-time. Hence, the agent must learn to autonomously set goals and solve them during training, in order to learn necessary re-usable skills for solving new goals sampled from an unknown distribution at test-time. 

This is the setting considered in a number of recent approaches for policy learning~\cite{skew,rig}, and is challenging because it assumes very less information about the ground-truth environment and goal-specifications. One of the desiderata as pointed out in Skew-Fit~\cite{skew} is to sample sufficiently diverse goals and learn to solve them, i.e. optimize $\mathcal{H}(\mathcal{G}) - \mathcal{H}(\mathcal{G}|\mathcal{S})$, where $\mathcal{H}(\cdot)$ denotes entropy. Although this guarantees uniform coverage in the infinite limit (assuming a perfectly learned goal-reaching policy), it does not ensure deep exploration in the finite horizon case.  \HB{Agreed that uniform coverage is not guaranteed for SkewFit in the general case. For showing this, SkewFit assumes a perfect oracle goal-reaching policy. But even if the goal-reaching policy is learned (not given by an oracle), then if we assume that it can be perfectly learned, the SkewFit analysis will still hold, and they can claim uniform coverage in the infinite limit. } In this paper, we emphasize the need to keep track of reachable states so to enable deep exploration via commitment, and set goals in a curriculum fashion, so that the agent learns to solve easier goals before trying to solve more difficult goals. 


  
\subsection{Notation}

We denote the set of observations (images) as $\mathcal{S}$ and the set of goals (images) as $\mathcal{G}$. In this paper we assume the underlying sets for $\mathcal{S}$ and $\mathcal{G}$ to be the same (any valid image can be a goal image~\cite{rig,skew}) but maintain separate notations for clarity. $f_\psi(\cdot)$ denotes the encoder of the $\beta-VAE$~\cite{betavae} that encodes observations $s\sim S$ to latent states $z\sim f_\psi(s)$. The goal conditioned policy given the current latent state $z_t$, and the goal $z_g$ is denoted by $\pi_\theta(\cdot | z_t,z_g)$, and $a_t\sim \pi_\theta(\cdot | z_t,z_g)$ denotes the action sampled from the policy at time $t$. The policy $\pi_\theta(\cdot | z_t,z_g)$ consists of a deterministic component $\mu_\theta(\cdot | z_t,z_g)$, and a noise term $\epsilon$, such that $\pi_\theta(\cdot | z_t,z_g) = \mu_\theta(\cdot | z_t,z_g) + \sigma_\theta\epsilon$, where $\epsilon$ is a Gaussian $\mathcal{N}(0,\mathbf{I})$ in this paper. $ReachNet(z_i,z_j;k)$ denotes the reachability network that takes as input two latent states  $z_i$, and $z_j$ and is conditioned on a reachability integer $k\in[1,..,H]$, where $H$ is the maximum time horizon of the episode. The output of $ReachNet(z_i,z_j;k)$ is either a $0$ denoting $z_j$ is currently not reachable from $z_i$  (and vice-versa) or a $1$ denoting $z_j$ is reachable from $z_i$ (and vice-versa). 

We consider the problem setting where a robot is initialized to a particular configuration, and is tasked to reach a goal, specified as an image. The test time goal distribution, from which goal images will be sampled for evaluation is not available during training, and hence the training approach is completely self-supervised. The underlying distribution of observations $\mathcal{S}$ is same as the underlying distribution of goals $\mathcal{G}$ during training, and are distributions over images from a camera.


==> arxiv_version/3-approach.tex <==
\vspace*{-0.2cm}
\section{Our Approach}
\label{sec:approach}
In this section, we discuss the specifics of the proposed approach, summarized in Algorithm~\ref{alg:mainbrief} .

%\subsection{Setup}


%either a third person view (in the real robot experiment) or from a camera mounted on the robot arm (in all the simulation experiments). 

%  \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{reachnet.png}
%     \caption{A schematic of the reachability network used to determine whether the latent state $z_i$ is reachable from the latent state $z_j$ in $k$ time-steps. The reachability vector $\mathbf{k}$ consists of a vector of the same size as $z_i$ and $z_j$ with all its elements being $k$. The output $0$ indicates that state $z_i$ is not reachable from state $z_j$.}
%     \label{fig:reachnetwork}
% \end{figure}

% \begin{figure*}[h!]
% \centering
%   \hspace*{-0.9cm}
%         \begin{subfigure}[b]{0.30\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{illustrative_figs/reach_vae1.PNG}
%     \caption{Sampling from the VAE}
%     \label{fig:vaegeneral}
%         \end{subfigure}% \\
%         \hspace*{-0.2cm}
%       %\vspace*{-2cm}
%          \begin{subfigure}[b]{0.30\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{illustrative_figs/vae_one_episode_pushreach1.PNG}
%     \caption{Traversal in the latent space}
%     \label{fig:vaeepisode}
%         \end{subfigure}   
%          \hspace*{-0.1cm}
%         \begin{subfigure}[b]{0.4\textwidth}
%               \centering
%   \includegraphics[width=\textwidth]{illustrative_figs/analysis2.PNG}
%     \caption{Analysis of ReachExplore}
%     \label{fig:analysis1}
%           \end{subfigure}   
%          \hspace*{-0.9cm}%\quad
%     \caption{(a) ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red). (b) This figure shows how sampling goals that lie on the latent VAE manifold and traversing on the latent manifold leads to latent states that decode to realistic dynamically feasible image frames.\
%     (c) The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (3) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it executes the stochastic policy for $T-k^*$ steps. (2) shows the case when the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then executes the stochastic policy for $T-k$ steps. This is similar in principle to the high level idea of Go-Explore~\cite{goexplore} (1) shows the case when the agent executes the stochastic policy for $T$ steps starting at the origin. The simplified Go-Explore and SkewFit~\cite{skew} models are described in Section~\ref{sec:analysis}}
%     \label{fig:vae}
%     \vspace*{-0.5cm}
% \end{figure*}


\subsection{Our Method's Key Insight}
\label{sec:reachidea}
Consider the goal conditioned policy $\pi(\cdot | z_t,z_g)$ with an initial latent state $z_0$, and a goal latent state $z_g$. The key idea of our method is to do committed exploration, by directly going to the frontier of reachable states for $z_0$ by executing the deterministic policy $\mu_\theta(\cdot | z_t,z_{k^*})$ and then execute the exploration policy $\pi_\theta(\cdot | z_t,z_g)$ from the frontier to perform goal directed exploration for the actual goal $z_g$. The frontier defined by $p_{k^*}$ is the empirical distribution of states that can be reliably reached from the initial state, and are the farthest away from the initial state, in terms of the minimum number of timesteps needed to visit them. The timestep index $k^*$ that defines how far away the current frontier is, can be computed as follows:
$$k^*=\argmax_k(IsReachable(z_0;k)) $$
The binary predicate  $IsReachable(z_0;k)$ keeps track of whether the fraction of states in the empirical distribution of $k-$reachable states $p_k$ is above a threshold $1-\delta$. The value of $IsReachable(z_0;k)$ $\forall k\in[1,..,H]$ before the start of the episode from $z_0$ is computed as:
%IsReachable(k)==True \text{iff}
\begin{equation}
       =\begin{cases}
      True, & \text{if}\ \mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)\geq 1 - \delta \\
      False, & \text{otherwise}
    \end{cases}
  \end{equation}
Here  $p_\phi(z)$ is the current probability distribution of latent states as learned by the $\beta-VAE$~\cite{betavae} with encoder $f_\psi(\cdot)$. $\delta$ is set to 0.2. For computing $\mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)$ above, we randomly sample states $z\sim p_\phi(z)$ from the latent manifold of the VAE, the intuition of which is illustrated in Fig.~\ref{fig:vae}. After calculating all the predicates $IsReachable(z_0;k)$ $\forall k\in[1,...,H]$ and determining the value of $k^*$, we sample a state $z_{k^*}$ from the empirical distribution of $k^*-$reachable states, $p_{k^*}$, ensuring that it does not belong to any $p_{k}$ $ \forall k< k^*$. Here, the empirical distribution $p_k$ denotes the set of states $z$ in the computation of $\mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)$ for which $ReachNet(z_0,z;k)$ returns a $1$, and  $ReachNet(z_0,z;k')$ returns a $0$, $\forall k'<k$.

In order to ensure that the sampled state $z_{k^*}$ is the closest possible state to the goal $z_g$ among all states in the frontier $p_{k^*}$, we perform the following additional optimization
\begin{equation}
    z_{k^*} = \argmin_{z\sim p_{k^*}}||z-z_g||_2
\end{equation}
Here, $||\cdot||_2$ denotes the $L_2$ norm. The above optimization encourages choosing the state in the frontier that is closest to the latent goal state $z_g$.
\begin{algorithm}[t!]
	\begin{algorithmic}[1]
		\Procedure{Overall}{GCP $\mu_\theta$, $\pi_\theta$, Prior $p(z)$, $S$, $f_\psi(\cdot)$, $IsReachable(\cdot)$, $H_0$, $N$, $\epsilon$, $\delta$, ReplayBuffer $\mathcal{B}$}
		\State $p_\phi = p(z)$
		\State Init $ReachNet(\cdot,\cdot; k)$, Def ReachData $\mathcal{D}$, $K=H_0N$
% 			\State Initialize $ReachNet(\cdot,\cdot; k)$ where $k=\{K,...,1\}$ 
% 			\State Def $K=H_0*N$ lists for $p_k$.
% 			\State Def Global ReachDataset = $\{ \}$ //to train $ReachNet$
		\For{episodes = 1 to $N$}
		\State $s_0\sim S_0$, encode $z_0=f_\psi(s_0)$, $z_{g}\sim p_\phi,\hat{z}^*=z_0$
% 		\State Sample initial state $s_0\sim S_0$, encode $z_0=f_\psi(s_0)$
% 		\State Sample latent goal $z_{g}$ from $p_\phi=p_{skewed}$
    %\State $\hat{z}^*=z_0$
    % \State //\texttt{Apply ReachExplore idea after some training}
	\If{episodes $\geq$ $N/4$} 
	 \For{$k=K-1,...,1$}
	\State Set the value of $IsReachable(z_0;k)$
	 \EndFor
% 			 \State Sample $M$ latent states $\{z\}_M\sim p_{\phi}$
% 	 \For{$k=K_{max},...,1$, $\forall z\in\{z\}_M$}
% 	 \State Initialize list $p_k\longleftarrow\{\}$
	
% 	  \If{$\frac{1}{k-1}\sum_{i=1}^{k-1}	 ReachNet(z,z_0;i)\geq 1-\epsilon$} 
% 	  \State Append $z$ to $p_k$
% 	  \EndIf
% 	  \For{counter = 1 to $C$}
% 	  \State Sample a latent state $z\sim p_k$
% 	   \If{$ReachNet(z,z_0;k)$}
% 	  \State c = c+1
% 	  \EndIf
% 	  \EndFor
% 	  \If{$\frac{c}{C}\geq 1-\epsilon$} 
% 	  \State Set $IsReachable(k)==True$
% 	  \EndIf
% 	  \EndFor
	  \State  $k^*=\argmax_k(IsReachable(z_0;k))$ 
	  \State Choose $ z_{k^*} = \argmin_{z\sim p_{k^*}}||z-z_g||_2$
	  	% 	\State //Set initial latent state to be $z^*$
	  	\State Exec $\pi_\theta(z_0;z_{k^*})$, reach $\hat{z}^*$ s.t. $||\hat{z}^*-z_{k^*}||\approx 0$
	  	\EndIf
		\State Set $H=H_0*episodes$ // \texttt{Curriculum} 
		\For{$t=0,...,H-1$}
		\If{$t==0$}
		\State Select $a_t\sim\mu_\theta(\hat{z}^*;z_{g})$ and execute it
		\EndIf
		\If{$t>0$ and $t<k^*$}
		\State Select $a_t\sim\mu_\theta(f_\psi(s_t);z_{g})$ and execute it
		\EndIf 
			\If{$t>0$ and $t\geq k^*$}
		\State Select $a_t\sim\pi_\theta(f_\psi(s_t);z_{g})$ and execute it
		\EndIf 
		\State // \texttt{Store tuple and Train policy}
		\State \textsc{StoreandTrain()}
		\EndFor 
%\State //Append to the dataset for training the ReachNet
%\State //Append observations and labels to $\mathcal{D}$
\State \textsc{AppendtoDataset($\mathcal{D}$)}
% \For{$t_1 = 0,...,H-1$}
% \For{$t_2 = 0,...,H-1$}
% \If{$t_1\neq t_2$}
% \State ReachDataset.add($(z_{t_1},z_{t_2},|t_1-t_2|)$)
% \EndIf
% \EndFor
% \EndFor

		

% 	\EndFor
%\State // Samples states to add in replay buffer $\mathcal{R}$
% \State //\texttt{Replay with goals as previously seen states}
\State \textsc{SampleFutureStates($\mathcal{B}$)}
% 	\For{$t=0,...,H-1$}
% 	\For{$i=0,...,k-1$}
%     \State Sample future states $s_{h_i}, t\leq h_i-1 \leq H-2$
%     \State Store $(s_t,a_t,s_{t+1},f_\psi(s_{h_i}),h_i+1)$ in $\mathcal{R}$
%     	\EndFor
%     		\EndFor
    \State Construct skewed dist.  $p_{skewed}$ from $\mathcal{B}$ (Skew-Fit) 
    \State Train the encoder using $p_\phi = p_{skewed}$
    \State Train $ReachNet(\cdot,\cdot; k)$ using ReachDataset $\mathcal{D}$
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\caption{Overview of the proposed Algorithm (Subroutines and the complete Algorithm are in the Appendix)}
	\label{alg:mainbrief}
\end{algorithm}
  
%  remove space after algo float  
% \setlength{\textfloatsep}{5pt}% Remove \textfloatsep


Our method encourages \textit{committed} exploration because the set of states until the frontier $p_{k^*}$ have already been sufficiently explored, and hence the major thrust of exploration should be beyond that, so that new states are rapidly discovered. The SkewFit~\cite{skew} approach showed that if the distribution over states is skewed to highly weigh rare states, and goals are sampled from this skewed distribution, the entropy over states $\mathcal{H}(\mathcal{S})$ will eventually approach the entropy of a uniform distribution $U_{\mathcal{S}}$ over the states. However, this is guaranteed in the infinite time limit. Applying our method with the SkewFit trick for sampling goals will still maintain the guarantee of maximum entropy, but improve sample efficiency of policy learning. Algorithm~\ref{alg:mainbrief} shows an overview algorithm for our method. In our specific implementation, we use SAC~\cite{sac} as the base off-policy model-free RL algorithm for minimizing the Bellman Error in the overall algorithm that is described in the Appendix.


\begin{figure*}[t!]
\centering
   \hspace*{-1cm}
       \adjustbox{valign=t}{ \begin{subfigure}[t]{0.60\textwidth}
               \centering
    \includegraphics[width=\textwidth]{arxiv_version/figures/vae_manifold_updated.png}
    \caption{\begin{footnotesize}(1) Our method samples latent goals from the the probability density manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold (i.e. sampling $z$ with low probability density under $p_\phi(z)$) is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the sphere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red). (2) The second figure shows how sampling goals that lie on the latent VAE manifold and traversing on the latent manifold leads to latent states that decode to realistic dynamically feasible image frames.\end{footnotesize}}
    \label{fig:vaegeneral}
        \end{subfigure}}% \\
    %     \hspace*{-0.1cm}
    %   %\vspace*{-2cm}
    %      \adjustbox{valign=t}{\begin{subfigure}[t]{0.30\textwidth}
    %           \centering
    % \includegraphics[width=\textwidth]{illustrative_figs/vae_one_episode_pushreach1.PNG}
    % \caption{\textcolor{red}{This figure shows how sampling goals that lie on the latent VAE manifold and traversing on the latent manifold leads to latent states that decode to realistic dynamically feasible image frames.}}
    % \label{fig:vaeepisode}
    %     \end{subfigure}}   
        % \hspace*{-0.1cm}
        \hspace{0.2cm}
        \adjustbox{valign=t}{\begin{subfigure}[t]{0.38\textwidth}
               \centering
   \includegraphics[width=\textwidth]{arxiv_version/figures/ReachExplore_analysis_updated.png}
    \caption{\begin{footnotesize}\textcolor{black}{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (3) shows the case when  the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it executes the stochastic policy for $T-k^*$ steps. (2) shows the case when the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then executes the stochastic policy for $T-k$ steps. (1) shows the case when the agent executes the stochastic policy for $T$ steps starting at the origin. The simplified Go-Explore~\cite{goexplore} and SkewFit~\cite{skew} models are described in Section~\ref{sec:analysis}}\end{footnotesize}}
    \label{fig:analysis1}
          \end{subfigure}}   
         \hspace*{-0.9cm}%\quad
    \caption{(a) Sampling from the VAE probability density manifold and traversal in the VAE latent space. (b) Simplified analysis of Our method.}
    \label{fig:vae}
    \vspace*{-0.5cm}
\end{figure*}




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{reach_vae.PNG}
%     \caption{ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red).}
%     \label{fig:vae}
% \end{figure}


% \begin{figure}[t]
%     \centering
%      \begin{subfigure}[b]{0.6\columwidth}
%               \centering
%     \includegraphics[width=0.9\columwidth]{illustrative_figs/reach_vae.PNG}
%     \caption{Forward pass of the ReachExplore approach}
%     \label{fig:reachidea}
%         \end{subfigure}% \\
%          \begin{subfigure}[b]{0.4\columwidth}
%               \centering
%      \includegraphics[width=\columnwidth]{illustrative_figs/vae_one_episode.PNG}
%     \caption{Simulation of one episode}
%     \label{fig:reachidea}
%         \end{subfigure}% \\
%     \caption{ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red).}
%     \label{fig:vae}
% \end{figure}



\subsection{Training the Reachability Network}
\label{sec:trainreachnet}
\vspace*{-0.2cm}
The reachability network $ReachNet(z_i,z_j;k)$ is a feedforward neural network with fully connected layers and ReLU non-linearities, the architecture of which is shown in Fig.~\ref{fig:mainfig}, with details in the Appendix. The architecture has three basic components, two encoders ($encoder_{\mathbf{state}}$, $encoder_{\mathbf{reach}}$), one decoder, and one concatenation layer. The latent states $z_i,z_j$ are encoded by the same encoder $encoder_{\mathbf{state}}$ (i.e. two encoders with tied weights, as in a Siamese Network~\cite{siamese}) and the reachability value $k$ is encoded by another encoder $encoder_{\mathbf{reach}}$. In order to ensure effective conditioning of the network $ReachNet$ on the variable $k$, we input a vector of the same dimension as $z_i$ and $z_j$, with all of its values being $k$, $\mathbf{k}=[k,k,...,k]$.

It is important to note that such neural networks conditioned on certain vectors have been previously explored in literature, e.g. for dynamics conditioned policies~\cite{mangapfn}. The three encoder outputs, corresponding to $z_i, z_j,$ and $k$ are concatenated and fed into a series of shared fully connected layers, which we denote as the decoder. The output of  $ReachNet(z_i,z_j;k)$ is a $1$ or a $0$ corresponding to whether $z_j$ is reachable from $z_i$ in $k$ steps or not, respectively.

To obtain training data for $ReachNet$, while executing rollouts in each episode, starting from the start state $z_0$, we keep track of  the number of time-steps needed to visit every latent state $z_i$ during the episode. We store tuples of the form $(z_i,z_j,k_{ij})$ $\forall i<j$ in memory, where $k_{ij} = j-i$, corresponding to the entire episode. Now, to obtain labels $\{0,1\}$ corresponding to the input tuple $(z_i,z_j,k)$, we use the following heuristic:
\begin{equation}
       label(z_i,z_j,k) =\begin{cases}
      1, & \text{if}\ |k_{ij} > \alpha k|\\
      0, & \text{if}  |k_{ij} < k|
    \end{cases}
  \end{equation}
Here $\alpha\in[1.2,1.5)$ is a threshold to ensure sufficient separation between positive and negative examples. 

%may include the bi about symmetric inputs bein fed to ensure the learned notion of symmetry 
\subsection{Implicit Curriculum for Increasing the Frontier}
\label{sec:curricula}
% In Sections~\ref{sec:reachidea} and~\ref{sec:trainreachnet}, we described the ReachExplore approach and demonstrated the computation of the current frontier. 
% Central to ReachExplore is the idea of repeatedly increasing the frontier of reachable states during training. It is crucial to note that for the ReachExplore approach of gradually increasing the frontier of exploration to succeed, it must be ensured that in-distribution nearby goals are sampled before goals far away.
The idea of growing the set of reachable states during training is vital to ReaxhExplore. Hence, we leverage curriculum to ensure that in-distribution nearby goals are sampled before goals further away.
This naturally relates to the idea of a curriculum~\cite{curriculum}, and can be ensured by gradually increasing the maximum horizon $H$ of the episodes. So, we start with a horizon length of $H=H_0$ and gradually increase it to $H=NH_0$ during training, where $N$ is the total number of episodes.

In addition to this, while sampling goals we also ensure that the chosen goal before the start of every episode does not lie in any of the $p_k$ distributions, where $k\leq k^*$ corresponding to the calculated $k^*$. This implies that the chosen goal is beyond the current frontier, and hence would require exploration beyond what has been already visited.

%\subsection{Overall Algorithm}
    
%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{illustrative_figs/reachexplore_analysis_all.PNG}
%     \caption{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (c) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it randomly explores for $T-k^*$ steps. (b) shows the case when ReachExplore is not employed, and the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then randomly explores for $T-k$ steps. This is similar in principle to the high level idea of Go-Explore~\cite{goexplore} (a) shows the case when ReachExplore is not employed, and the agent starts doing random exploration for $T$ steps starting at the origin. This is similar in principle to SkewFit~\cite{skew}.}
%     \label{fig:analysis1}
% \end{figure}





%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{analysis.png}
%     \caption{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (a) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it randomly explores for $T-k^*$ steps. (b) shows the case when with probability $1-\chi$, the goal-reaching policy fails to take the agent to the frontier, and ends up somewhere within the already explored blue region. After that the  agent randomly explores for $T-k^*$ steps. Note that for computing the lower bound $L_1$, we consider the worst case when the circle of radius $\sqrt{T-k^*}$ is contained within the circle of radius $k^*$. (c) shows the case when ReachExplore is not employed, and the agent starts doing random exploration for $T$ steps starting at the origin.}
%     \label{fig:analysis}
% \end{figure}


==> arxiv_version/4-analysis.tex <==

\section{Analysis of ReachExplore: Intuition of deep exploration through average case analysis}
\label{sec:analysis}
In this section, we provide formal analysis of ReachExplore in a simplified, idealized, setting. Consider a 2D world with a single start location $\mathbf{z}_0$ and and let the goal be denoted by $\mathbf{z}_g$. Let $p_{k^*}$ denote the current frontier. Let $T$ denote the total time-steps in the current episode. 

We aim to show that using this time-step budget, the odds of exploring previously unvisited states farther away from the start state are higher when using ReachExplore, as compared to without using it. 
% Let $\chi$ denote the probability of the deterministic goal-conditioned policy reaching a goal state in $p_{k^*}$ in $k^*$. 
For simplicity, we assume the stochastic goal-reaching policy to be the policy of a random walker, and the deterministic goal-reaching policy to be near-optimal in the sense that given a target goal in $p_{k^*}$, and an initial state in the already explored region, it can precisely reach the  target location at the frontier with a high probability($\gg0$). 

For analysis, we define SkewFit~\cite{skew}, GoExplore~\cite{goexplore}, and our method in the above setting to be the following simplified schemes, and illustrate the same in Fig.~\ref{fig:analysis1}:
\begin{enumerate}

%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]

    \item \textbf{SkewFit-variant:} The model that executes the stochastic policy for the entire length $T$ of the episode to reach goal $z_g$, and sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
    \item \textbf{GoExplore-variant:} The model that first chooses a random previously visited intermediate latent goal state from the archive (not necessarily from the frontier $p_{k^*}$), executes a deterministic goal directed policy for say $k$ steps to reach the intermediate goal, and then executes the stochastic policy exploring for the next $T-k$ steps. For analysis, $0<k<k^*$. This is similar in principle to the idea of Go-Explore~\cite{goexplore}\footnote{Here, we refer to the intuition of Phase 1 of Go-Explore, where the idea is to ``select a state from the archive, go to that state, start exploring from that state, and update the archive." For illustration and analysis, we do not consider the exact approach of Go-Explore. In order to ``go to that state" Go-Explore directly resets the environment to that state, which is not allowed in our problem setting. Hence, in Fig.~\ref{fig:analysis1}, we perform the analysis with a goal-directed policy to reach the state. Also, since Go-Explore does not keep track of reachability, we cannot know whether the intermediate goal chosen can be reached in $k$ timesteps. But for analysis, we assume the intermediate goal is chosen from some $p_k$ distribution as described in Section~\ref{sec:reachidea}}. It also sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
    \item \textbf{Our method:} The model that first chooses a state from the frontier $p_{k^*}$, executes a deterministic goal directed policy for say $k^*$ steps to reach the frontier, and then executes the stochastic policy exploring for the next $T-k^*$ steps.  It also sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
\end{enumerate}

%From the theory of hitting times in 2D random walks, we have the following result.
\begin{lemma}
For a random walk with unit step size in 2D (in a plane), the average distance away from a point (say, the origin) traversed in $t$ time-steps is $\sqrt{t}$.
\label{lemma:main}
\end{lemma}
\begin{proof}
The proof of is provided in the Appendix.
% In a plane, consider the sum of $t$ 2D vectors with random orientations. For convenience, we use the phasor notation, and so assume the phase of each vector to be random. Starting at some point (let's call it the origin $z_0$), we assume $t$ steps are taken in an arbitrary direction, which is equivalent to assuming that the angle $\theta$ of the phasors is uniformly distributed in $[0,2\pi)$. The position $z_t$ in the complex plane after $t$ steps is:
% $$ z_t = \sum_{k=1}^te^{i\theta_k}$$
% The square of the absolute value of $z_t$is:
% $$ |z_t|^2 = \sum_{k=1}^te^{i\theta_k}\sum_{m=1}^te^{-i\theta_m}
% = t + \underset{k=1,m=1,k\neq m}{\sum\sum^t}e^{i(\theta_k-\theta_m)}$$
% Now, we calculate the expected value of the $|z_t|^2$ variable by noting that since $\theta_k$ and $\theta_m$ are randomly sampled in $[0,2\pi)$ with uniform probability, the displacements $e^{i\theta_k}$ and $e^{i\theta_m}$ are random variables, so their difference corresponding to $\theta_k-\theta_m$ is also a random variable and has an expected value (mean) of $0$. Hence,
% $$<|z_t|^2> = t \implies |z_t|_{rms} = \sqrt{t}$$

% So, the average (root-mean-square) distance traversed after $t$ steps starting at some $z_0$ in the 2D plane is $\sqrt{t}$
\end{proof}
\noindent The subsequent results are all based on the above stated lemma and assumptions. 
\begin{lemma}
Starting at $z_0$ and assuming the stochastic goal-reaching policy to be a random walk, on average the SkewFit scheme will reach as far as $R_1 =\sqrt{T}$ at the most in one episode.
\end{lemma}
\begin{proof}
This follows directly from Lemma~\ref{lemma:main} by setting $t=T$, where $T$ is the max. number of timesteps in the episode.
\end{proof}
\vspace{-0.3cm}
% The lemma is illustrated in the first figure (1) of Fig.~\ref{fig:analysis1}, and is similar in principle to the basic SkewFit~\cite{skew} approach because at the start of each episode a stochastic goal-directed policy is rolled out from the initial state.

% In the second figure (2) of Fig.~\ref{fig:analysis1}, we consider a situation where a random previously visited intermediate latent goal state from the archive is chosen (not necessarily from the frontier $p_{k^*}$). Then the agent executes a deterministic goal directed policy for say $k$ steps to reach the intermediate goal, and then executes the stochastic policy exploring for the next $\sqrt{T-k}$ steps. For analysis, $0<k<k^*$. This is similar in principle to the idea of Go-Explore~\cite{goexplore}\footnote{Here, we refer to the intuition of Phase 1 of Go-Explore, where the idea is to ``select a state from the archive, go to that state, start exploring from that state, and update the archive." For illustration and analysis, we do not consider the exact approach of Go-Explore. In order to ``go to that state" Go-Explore directly resets the environment to that state, which is not allowed in our problem setting. Hence, in Fig.~\ref{fig:analysis1}(b), we perform the analysis with a goal-directed policy to reach the state. Also, since Go-Explore does not keep track of reachability, we cannot know whether the intermediate goal chosen can be reached in $k$ timesteps. But for analysis, we assume the intermediate goal is chosen from some $p_k$ distribution as described in Section~\ref{sec:reachidea}}. 

%In this case, the maximum average distance away from the origin traversed by the agent is atmost $r=\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$.
\begin{lemma}
Starting at $z_0$ and assuming the deterministic goal-deterministic policy to be near optimal (succeeds with a very high probability$>>0$), and the stochastic goal-reaching policy to be a random walk, on average GoExplore scheme will be bounded by $R_2 =\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$ in one episode.
\label{lemma:goexplore}
\end{lemma}
\begin{proof}
Since GoExplore first goes to a random previously visited state using the deterministic goal conditioned policy, from Fig~\ref{fig:analysis1} it is evident that the distance of such a state from the start state could be in the range $(0,k^*)$. Let this distance be $k$. Then, from Lemma~\ref{lemma:main}, the max distance on average traversed by the agent from $z_0$, if the intermediate state is at a distance $k$, can be given as:
$$ r_k = k + \sqrt{T-k}$$
Averaging over all the distance of all possible intermediate positions $k\in(0,k^*)$, we obtain the final averaged maximum distance reached by the agent in one episode as:
$$R_2 = \frac{1}{k^*}\sum_{k=0}^{k^*}(k+\sqrt{T-k})$$
%\vspace{-0.2cm}
\end{proof}
\vspace{-0.3cm}

% From the theory of hitting times in 2D random walks where at each timestep, the agent can move by 1 unit in any direction~\cite{hitting}, the average distance away from the origin traversed in $t$ steps is $\sqrt{t}$ \HB{Not a grid graph. This is for moving in free space, starting at a fixed point, where at each timestep the agent moves by 1 unit - so the agent can take discrete steps. We had discussed this on the whiteboard}. Hence, considering the stochastic policy (which for simplicity of analysis we considered to be a random walk), the maximum distance on average from $\mathbf{s}_0$ traversed in $T$ time-steps is $\sqrt{T}$. 



% While, if we employ ReachExplore, the maximum distance on average is atmost $k^* + \sqrt{T-k^*}$, as described in the following lemma:
\begin{lemma}
Starting at $z_0$ and assuming the deterministic  goal-conditioned policy to be near optimal (succeeds with a very high probability $>>0$), and the stochastic goal-reaching policy to be a random walk, on average our method will be bounded by $R_3 = k^* + \sqrt{T-k^*}$
\end{lemma}
\begin{proof}
In the proof for lemma~\ref{lemma:goexplore}, setting $k=k^*$ in the formula, for $r_k$ gives us the maximum average distance for our method as:
$$R_3 =  k^* + \sqrt{T-k^*}$$
%\vspace{-0.2cm}
\end{proof}
\vspace{-0.3cm}
\begin{theorem}
$R_3>R_2$ $\forall k^*\in[1,T)$ and $R_3>R_1$ $\forall k^*\in[1,T)$. i.e. After the frontier $k^*$ is sufficiently large, the maximum distance from the origin reached by our method is more than both GoExplore and SkewFit.
\label{lemma:final}
\end{theorem}
\begin{proof}
We provide the proof of this in the Appendix.
\end{proof}

% In the Appendix we show that for values of $k^*>T/4$, $k^* + \sqrt{T-k^*}$ is always greater than  $r=\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$.
\noindent Theorem~\ref{lemma:final} is the main result of our analysis and it intuitively suggests the effectiveness of deep exploration guaranteed by our method. This is shown through a visualization in Fig.~\ref{fig:analysis1}. 

In Fig.~\ref{fig:analysis1}\,(2) and (3), we assume the deterministic policy succeeds with high probability($\gg0$), which is usually the case after sufficient training iterations in off-policy Q-learning. It can be easily seen that if $k^*$ increases during training (i.e. the reachable frontier expands), then after a finite number of interactions with the environment, we will have $k^*>\sqrt{T}$. We ensure that this happens because of the implicit curriculum on horizon length, and the sampling of goals beyond the current reachable frontier at the start of every episode.




% \subsection{Fast(er) coverage guarantees through average case analysis (Sec to be commented)}
% In this section, we provide theoretical justifications for why applying the ReachExplore trick ensures faster coverage. Consider a 2D world with a single start location $\mathbf{s}_0$ and and let the goal be denoted by $\mathbf{s}_g$. Let $k^*$ denote the current frontier. Let $T$ denote the total number of time-steps in the current episode. We sim to show that using this time-step budget, the odds of exploring previously unvisited states are higher when using ReachExplore, as compared to without using it. Let $\chi$ denote the probability of the deterministic goal-conditioned policy reaching a goal state in $p_{k^*}$ in $k^*$. For simplicity, we assume the stochastic goal-reaching policy to be the policy of a random walker. 

% From the theory of hitting times in 2D random walks~\cite{hitting}, the average distance away from the origin traversed in $t$ steps is $\sqrt{t}$. We consider two cases:
% \begin{itemize}
%     \item The agent employs ReachExplore to go to the frontier at a radius of $k^*$, using the deterministic goal-conditioned policy and then perform a random walk with the remaining $T-k^*$ steps. During this random walk the agent will go upto a distance of $\sqrt{T-k^*}$ in any direction. Let the total area traversed on average be $A_1$.
%     \item The agent does not employ ReachExplore and executes the default stochastic goal conditioned policy (which we assumed for simplicity to be the policy of a random walk) from the start state $\mathbf{s}_g$ and continues for  $T$ time-steps, thus ending up on an average somewhere in a circle of radius $\sqrt{T}$ centered at $\mathbf{s}_{k^*}\sim p_{k^*}$. Let the total area traversed on average be denoted by $A_2$, and we have $A_2=\pi T$.
% \end{itemize}
% We have the following lower bound on $A_1$ (Fig.~\ref{fig:analysis})
% $$A_1 \geq \chi\left(\pi (k^*)^2 + \frac{1}{2}\pi (T - k^*)\right) + (1-\chi)\pi (k^*)^2 $$
% Let us denote the above lower bound by $L_1$. To show $A_1>A_2$ it is enough to show that $L_1-A_2>0$. Let us consider the difference $L_1-A_2$:
% $$L_1-A_2 = \pi(k^*)^2 -\frac{1}{2}\pi\chi k^* + \frac{1}{2}\pi (\chi-2)T$$
% Treating the above as a quadratic expression in the variable $x=k^*$, we note that the value of $Ax^2+Bx+C>0$ $\forall x$ when $B^2-4AC < 0$. For our problem, $$B^2-4AC = \frac{1}{4}\pi^2\chi^2 - 2\pi^2T(\chi-2)=2\pi^2(\frac{1}{8}\chi^2-T\chi+2T)$$
% Since $\chi\in(0,1)$ and $T>1$, the value of $B^2-4AC$ is always greater than $0$. So, by analyzing the roots of the equation, 
% $$\pi(k^*)^2 -\frac{1}{2}\pi\chi k^* + \frac{1}{2}\pi (\chi-2)T = 0$$
% we have 
% $$\forall k^* >\frac{1}{4}\chi + \frac{1}{2}\sqrt{\frac{1}{4}\chi^2 -2T\chi + 4T}$$
% $L_1-A_2>0$ and so $A_1>A_2$. This result tells us that there is a certain value of frontier $k^*<T$ such that when we have achieved this frontier, it is beneficial to perform committed exploration via the ReachExplore approach. Now, in each iteration of training, since we sample goals beyond the currently reachable frontier $k^*$ (Section~\ref{sec:approach}C), so the value of $k^*$ will always increase during training. Hence, the above value will be reached at some point during training. 


==> arxiv_version/5-experiments.tex <==

\section{Experiments}
Our experiments aim to understand the following questions: (1) How does our method compare to existing state-of-the-art exploration baselines, in terms of faster convergence and higher cumulative success? 
%(2) How does keeping track of reachability ensure faster convergence and deep exploration required to solve long-horizon robotic tasks directly from images?
(2) How does our method scale as task complexity increases?
(3) Can our method scale to tasks on a real robotic arm?

\subsection{Environments}
We consider the image-based and state-based environments illustrated in Fig.~\ref{fig:sim_envs}. In case of image-based environments, the initial state and the goal are both specified as images. In case of state-based environments, the initial state and the goal consists of the coordinates of the object(s), the position and velocity of different components of the robotic arm, and other details as appropriate for the environment (Refer to the Appendix for details). In both these cases, during training, the agent does not have access to any oracle goal-sampling distribution. In Fig.~\ref{fig:sim_envs}, (b), and (c) are configured to be \textit{sparse-reward} settings, where the reward is $1$ only when the agent $solves$ the goal and is $0$ otherwise. To define when a goal is $solved$, for each environment there is a certain threshold distance between the agent's final state and the goal state, the details of which are mentioned in the appendix. All the other environments in Fig.~\ref{fig:sim_envs} use \textit{only} a latent distance based reward during training (reward $r=-||z_t-z_g||_2$; $z_t$ is the agent's current latent state and $z_g$ is the goal latent state), and have no access to ground-truth simulator states. 

% \begin{figure}[t]
% \centering
%         \begin{subfigure}[b]{0.5\columnwidth}
%               \centering             \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/one.png}
%     %\caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%          \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/five.png}
%   % \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%     % \includegraphics[width=0.7\columnwidth]{illustrative_figs/one.png}
%     \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%           \begin{subfigure}[b]{0.5\columnwidth}
%               \centering             \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/fetch_one.png}
%     %\caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%          \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/fetch_final.png}
%   % \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%     % \includegraphics[width=0.7\columnwidth]{illustrative_figs/one.png}
%     \caption{Fetch Slide}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
        
       
%      \caption{Illustrations of all the simulation environments evaluated in this paper, with example initial and goal images.}  
%  \label{fig:sim_results}
% \end{figure}
 \begin{figure}
     \centering
     \includegraphics[width=0.99\columnwidth]{arxiv_version/figures/reachexplore_allenvs.png}
     \caption{Illustrations of all the environments evaluated in this paper, with example initial (left) and goal (right) images.  Each environment we consider is meant to demonstrate scaling of the proposed approach to different settings: image-based goals, state-based goals, continuous action spaces, discrete action spaces, different dynamics (point mass, Fetch robot, Sawyer robot, Franka Panda robot), increasing task complexity (Push to Push and Reach), and applicability to a real robot. Details are in the Appendix. }
     \label{fig:sim_envs}
     \vspace*{-0.4cm}
 \end{figure} 
 
 
\begin{figure*}[h!]
\centering
 \begin{subfigure}[b]{0.60\textwidth}
               \centering
    \includegraphics[width=\textwidth]{arxiv_version/figures/reachexplore_results.png}
    \caption{Comparative results on simulation environments}
    \label{fig:quantitative}
        \end{subfigure}\hspace*{-0.1cm}
                 \begin{subfigure}[b]{0.40\textwidth}
               \centering
    \includegraphics[width=\textwidth]{arxiv_version/figures/qualitative.png}
    \caption{Qualitative results showing the goal image on the left, and rendered images of the final states reached by SkewFit and our method for two evaluation runs in two different environments.}
    \label{fig:qualitative}
        \end{subfigure}

            %\quad
     \caption{Comparison of our method and SkewFit on an ensemble of vision-based and state-based simulation environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are with respect to three random seeds. It is important to emphasize that the training proceeds in a completely self-supervised manner, without assuming any access to the oracle goal sampling distribution. The results reported are for evaluations on test suites (initial and goal images are sampled from a test distribution unknown to the agent) as training progresses. Although the ground-truth simulator states are not accessed during training (for (a), (c), (d), (e), and (f)), for the evaluation reported in these figures, we measure the ground truth $L_2$ norm of the final distance of the object/end-effector (as appropriate for the environment) from the goal location.  In (f), we evaluate the final distance between the (puck+end-effector)'s location and the goal location. In (c), success is measured as +1 if the agent reaches the final green goal square in the grid, and 0 otherwise. In (b), success is measured as +1 if the puck reaches within 2cm of the goal location. In (a), (d), (e), and (f), lower is better. In (b) and (c), higher is better.}  
 \label{fig:sim_results}
 \vspace*{-0.6cm}
\end{figure*}

 
%  Each environment we consider is meant to demonstrate scaling of the proposed approach to different settings: image-based goals, state-based goals (Fetch slide), continuous action spaces, discrete action spaces (Locked door navigation), different dynamics (point mass, Fetch robot, Sawyer robot, Franka Panda robot), and applicability to a real robot (Franka Panda).
\begin{enumerate}

%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]
  
  \item \textbf{Pointmass Navigation} (\textit{Image-based}): A pointmass object must be navigated from an initial location to a goal location in the presence of obstacles. The agent must plan a temporally extended path that would occassionally involve moving away from the goal. This is a 2D environment with a continuous action space, and the agent has access to images from a top-down view. 
   \item \textbf{Fetch Slide} (\textit{State-based}): A Fetch robot arm must be controlled to push and slide a puck on the table such that it reaches a certain goal location. It is ensured that sliding must happen (and not just pushing) because the goal location is beyond the reach of the arm's end-effector. We make this environment significantly difficult by reducing the default friction coefficient by a factor of 2. The agent has access to state information - the position $(x,y,z)$ and velocity $(v_x,v_y,v_z)$ of its end-effector. 
   \item \textbf{Gridworld Locked Door Navigation} (\textit{Image-based}): A point agent navigates a maze to pick up a key, open a locked door, and navigate to a goal location on the other side of the door. This is a 2D environment, and the agent has access to a top-down view. At each time-step, the agent has the option to choose from six actions (so discrete action space).
   \item \textbf{Sawyer Pick} (\textit{Image-based}): A Sawyer robot arm must be controlled to pick a puck from a certain location and lift it to a target location above the table. The agent has access to images from a camera mounted on the arm.
        \item \textbf{Sawyer Push} (\textit{Image-based}): A Sawyer robot must push a puck to a certain location with the help of its end-effector. The agent has access to images from a camera mounted on the arm.
    \item \textbf{Sawyer Push and Reach} (\textit{Image-based}): A Sawyer robot arm is controlled to push a puck to a target location, and move its end-effector to a (different) target location. The agent has access to images from a camera mounted on the arm.
    \item \textbf{Franka Panda Peg in a Hole} (\textit{State-based; Real robot}); A real Franka Panda arm must be controlled to place a peg in a hole. The agent is velocity controlled and has access to state information - the position $(x,y,z)$ and velocity $(v_x,v_y,v_z)$ of its end-effector. 
\end{enumerate}
\subsection{Setup}
We use the Pytorch library~\cite{pytorch1,pytorch2} in Python for implementing our algorithm, and ADAM~\cite{adam} for optimization.  We consider two recent state-of-the-art exploration algorithms, namely Skew-Fit~\cite{skew}, and Go-Explore~\cite{goexplore} as our primary baselines for comparison. For both these baselines, for consistency, we use SAC for policy-learning.  Based on the original implementation of Go-Explore~\cite{goexplore}, we create a version using SAC~\cite{sac} as the base policy and employing the Go-Explore trick which we use as our baseline.

For training, we train our method and the baselines in a completely unsupervised manner, without access to any oracle goal-sampling distribution. In addition, in the image-based environments, during training the agent does not have access to any prior information about the state-space. In order to 
\textit{evaluate} the performance of the algorithms, we sample goal images from a uniform distribution over valid images and report the final distance of the agent to the corresponding states in simulator. This method of evaluation, although applicable only in simulation, is a reliable metric for RL with vision-based goals, as described in prior works~\cite{rig,skew}. It is important to note that we access the simulator states only for \textit{evaluation} - not for training (except for (b), and (h) in Fig.~\ref{fig:sim_envs}). 

%During training, to measure reward, we compute the $L_1$ norm of the difference between the agent's latent state $z_t$ and the goal latent state $z_g$.
% \begin{figure*}[h!]
% \centering
%  \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pointmassfinal.png}
%     \caption{Pointmass Navigation (Image)}
%     \label{fig:pointmass}
%         \end{subfigure}\hspace*{-0.2cm}
%                  \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pickplacefinal.png}
%     \caption{Sawyer Pick and Place (Image)}
%     \label{fig:pickplace}
%         \end{subfigure}
        
        
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/push_easy_final.png}
%     \caption{Sawyer Push (Image)}
%     \label{fig:pusheasy}
%         \end{subfigure}% \\
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pushreachfinal.png}
%     \caption{Sawyer Push and Reach (Image)}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%         %\hspace*{-0.5cm}
        
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/gridlocked_doorfinal.png}
%     \caption{Gym Locked Door Navigation (Image)}
%     \label{fig:fetchslide}
%         \end{subfigure}\hspace*{-0.2cm}
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/fetchslide_final.png}
%     \caption{Fetch robot - Slide (State)}
%     \label{fig:fetchslide}
%         \end{subfigure}
%             %\quad
%      \caption{Comparison of our method and SkewFit on an ensemble of vision-based and state-based simulation environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are with respect to three random seeds. It is important to emphasize that the training proceeds in a completely self-supervised manner (for both our method and SkewFit), without assuming any access to the oracle goal sampling distribution. The results reported are for evaluations on test suites (initial and goal images are sampled from a test distribution unknown to the agent) as training progresses. Although the ground-truth simulator states are not accessed during training (for (a), (b), (c), (d), and (e)), for the evaluation reported in these figures, we measure the ground truth L2 norm of the final distance of the oject/end-effector (as appropriate for the environment) from the goal location. In (e), success is measured as +1 if the agent reaches the final green goal square in the grid, and 0 otherwise. In (f), success is measured as +1 if the puck reaches the goal location with a tolerance threshold of $0.1\%$. In (a), (b), (c), and (d), lower is better. In (e) and (f), higher is better.}  
%  \label{fig:sim_results}
% \end{figure*}




\subsection{Results}
\noindent\textbf{Our method achieves higher success during evaluation in reaching closer to the goals compared to the baselines}
Fig.~\ref{fig:sim_results} shows comparisons of our method against the baseline algorithms on all the robotic simulation environments. It is evident that our method performs significantly better than all the baselines. The image based Sawyer Push and Reach environment is challenging because there are two components to the overall task. The significant performance improvement of our method over the baselines can be can be clearly seen in Fig.~\ref{fig:sim_results}.

 The pointmass navigation environment is challenging because during evaluation, we choose the initial position to be inside the U-shaped area, and the goal location to be outside it, and the agent does not know this apriori. So, during training the agent must learn to set difficult goals outside the black arena and must try to solve them. This requires deep committed exploration, and as shown in Fig.~\ref{fig:quantitative}, our method succeeds in achieving this.

In addition to the image based goal environments, we consider a challenging state-based goal environment as proof-of-concept to demonstrate the effectiveness of our method. In Fig.~\ref{fig:quantitative} we see that for the slide task on a Fetch robot, our method achieves much higher success rate compared to the baselines in pushing the puck with the right amount of force in the right direction such that it stops exactly at the goal location. In order to succeed in this task, the agent must acquire an implicit estimate of the friction coefficient between the puck and the table top, and hence must learn to set goals close and solve them before setting goals farther away. 


\noindent\textbf{Our method scales to tasks of increasing complexity}
From Fig.~\ref{fig:quantitative}, we see that our method performs comparably to its baselines. The improvement of our method over SkewFit is not statistically significant. However, in the task of Push and Reach (Fig.~\ref{fig:quantitative}) we observe significant improvement of our method over SkewFit. The baselines succeed either in the push part of the task or the reach part of the task but not both, suggesting overly greedy policies without long term consideration (Refer qualitative results in Fig.~\ref{fig:qualitative}).This suggests the effectiveness of our method in scaling to a difficult task that requires more temporal abstraction. This benefit is probably because our method performs two staged exploration, which enables it to quickly discover regions that are farther away from the initial state given at the start of the episode. 
%Since the agent receives a +1 reward only when it pushes the puck to the desired location and brings the end-effector to its desired location (i.e. sparse reward), focusing the thrust of exploration on previously unexplored states is crucial to discover trajectories that successfully solve the task. 

We observe similar behaviors of scaling to more complicated tasks by looking at the results of the Pointmass Navigation in Fig.~\ref{fig:quantitative}. While the task can be solved even by simple strategies when the goal location is within the U-shaped ring, the agent must actually discover temporally abstracted trajectories when the goal location is outside the U-shaped ring. Discovering such successful trajectories in the face of only latent rewards, and no ground-truth reward signals further demonstrates the need for committed exploration. 
  

% \begin{figure*}[t]
% \centering
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pushreach_eval1.png}
%     \caption{Sawyer Push and Reach (Image)}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pickplace_final.png}
%     \caption{Sawyer Pick and Place (Image)}
%     \label{fig:pickplace}
%         \end{subfigure}
        
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pointmass.png}
%     \caption{Pointmass Navigation (Image)}
%     \label{fig:pointmass}
%         \end{subfigure}
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{anglediff_compare.png}
%     \caption{Sawyer Door opening (I)[rev. legend]}
%     \label{fig:avg_r_lf}
%         \end{subfigure}
        
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{fetchslideresult.png}
%     \caption{Fetch robot - Slide (State)}
%     \label{fig:fetchslide}
%         \end{subfigure}
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{fetchesults.png}
%     \caption{Fetch robot - Reach (State)}
%     \label{fig:results}
%         \end{subfigure}
%     %\quad
%      \caption{Comparison of our method and SkewFit on an ensemble of vision-based and state-based environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are wrt 3 seeds in (a), (d), and (e), and wrt 2 seeds in (b), (c), and (f). It is important to emphasize that the training proceeds in a completely unsupervised manner (for both our method and SkewFit), without assuming any access to the oracle goal sampling distribution.}  
%  \label{fig:sim_results}
% \end{figure*}
  

  
\noindent\textbf{Our method scales to tasks on a Real Franka Panda robotic arm} Fig.~\ref{fig:panda} shows results for our method on a peg-in-a-hole evaluated on the Franka Panda arm. Here the objective is to insert a peg into a hole, an illustration of which is shown in Fig.~\ref{fig:sim_envs}.  The reward function is defined to be the negative of the distance from the center of bottom of the peg to the center of the bottom of the hole. There is an additional heavy reward penalty for `collision' and a mild penalty for `contact.' The home position of the panda arm (to which it is initialized) is such that the distance from the center of the bottom of the peg to the center of the bottom of the hole is 0.35 meters. The heavy penalty for collision is -10 and the mild penalty for contact is -1. We can observe from Fig.~\ref{fig:panda} that our method successfully solves the task while the baseline GoExplore does not converge to the solution. This demonstrates the applicability of our method on a real robotic arm.

% \begin{figure}
%   \centering
%  \begin{subfigure}[b]{0.7\columnwidth}
%               \centering
%     \includegraphics[width=\columnwidth]{results_figs/franka_real_arm.png}
%     \caption{Reaching task (State-based)}
%     \label{fig:pointmass}
%         \end{subfigure}%\hspace*{-0.2cm}
%                  \begin{subfigure}[b]{0.2\columnwidth}
%               \centering
%     \includegraphics[width=\columnwidth]{illustrative_figs/pandaarm.png}
%     \caption{Panda arm}
%     \label{fig:pickplace}
%         \end{subfigure}
%       \caption{Results of a Reaching task on the real Franka Emika Panda arm. The goal is specified as a tuple of coordinates (x,y,z) to be reached. The state consists of the position and velocities of the end-effector. Higher is better.}
%     \label{fig:panda}
%     \vspace*{-0.2cm}
% \end{figure}


\begin{figure}
   \centering
    \includegraphics[width=0.85\columnwidth]{arxiv_version/figures/real.png}    
    \caption{Results of a Peg-in-a hole task on the real Franka Emika Panda arm. The evaluation metric on the y-axis is the distance ($L_2$ norm) of the center of the bottom of the hole from the center of the bottom of the peg. The state consists of the position and velocities of the end-effector. Lower is better}
    \label{fig:panda}
     \vspace*{-0.5cm}
  \end{figure}
   

==> arxiv_version/6-related_works.tex <==
\vspace*{-0.35cm}
\section{Related Works}


\noindent \textbf{Vision-based RL for Robotics.} Recent works have investigated vision-based learning of RL policies for specific robotic tasks like grasping~\cite{grasping1,grasping2}, pushing~\cite{pushing2,pushing1}, and navigation~\cite{navigation2,navigation1}, however relatively few prior works have considered the problem of learning policies in a completely self-supervised manner~\cite{rig,skew}. A recent paper~\cite{avi} considers RL directly from images, for general tasks without engineering a reward function, but involves a human in the loop. Some other prior works learn latent representations for RL in an unsupervised manner which can used as input to the policy, but they either require expert demonstration data~\cite{upn,sim2realmanga}, or assume access to ground-truth states and reward functions during training~\cite{worldmodels,ground2,ground3}. RIG~\cite{rig} proposes a general approach of first learning a latent abstraction from images, and then planning in the latent space, but requires data collected from a randomly initialized policy to design parametric goal distributions.  In addition, niether approaches do not guarantee any notion of exploration or coverage that is required for solving difficult temporally-extended tasks from minimal supervision - in particular with goals specified as raw images.



\noindent \textbf{Goal-conditioned Policy Learning.}
While traditional model-free RL algorithms are trained to succeed in single tasks~\cite{td3,sac,ppo,trpo}, goal-conditioned policy learning holds the promise of learning general-purpose policies that can be used for different tasks specified as different goals~\cite{kaelbling1993learning,her,rig,arc}. However, most goal-conditioned policy learning algorithms make the stronger assumption of having access to an oracle goal sampling distribution during training~\cite{kaelbling1993learning,her,universal,leap}. A recent paper~\cite{arc} proposes an algorithm to create dynamics-aware embeddings of states, for goal-conditioned RL, but it is not scalable to images as goals (instead of ground-truth states).  

Some other prior works do not assume access to an oracle goal-sampling distribution, but sample goals based on some ad-hoc heuristics like learning progress~\cite{learnprogress1,learnprogress2}, how off-policy the goal is~\cite{offpolicy} or sample goals randomly from the learn latent distribution over image observations~\cite{rig}. Skew-Fit~\cite{skew} adds structure to the goal-sampling process by sampling goals in the latent space such that the entropy over the learned distribution over states is maximized, but provides no guarantee of coverage/exploration in finite time. 





\noindent \textbf{Exploration for RL.} Skew-fit~\cite{skew} proposes a novel entropy maximizing objective that ensures gradual coverage in the infinite time limit. In addition, it does not incorporate any notion of commitment during exploration, which is needed to discover complex skills for solving temporally extended tasks in finite time. Go-Explore~\cite{goexplore} addresses this issue to some extent by keeping track of previously visited states in the replay buffer, and at the start of each episode, re-setting the environment to a previously visited state chosen on the basis of domain-specific heuristics, and continuing exploration from there. However, this approach is fundamentally limited because it assumes the environment is re-settable, which is not always feasible on a real robot. In addition, the domain-specific heuristics for Montezuma's revenge in the original paper do not readily apply to latent spaces for robotic tasks.

On the contrary, novelty/surprise based criteria have been used in many RL applications like games, and mazes~\cite{curiosity,count,rupam}. In~\cite{curiosity}, a curiosity based intrinsic reward signal is used in addition to the external reward in order to encourage the RL agent to visit previously unvisited states. In~\cite{count}, the authors explicitly keep track of the state visitation frequencies and reward the agent for visiting states with less visitation frequency. VIME \cite{vime} considers information gathering behaviors to reduce epistemic uncertainty on the dynamics model. 

%Although these methods are general in that novelty bonuses are not %task-specific, there is no mechanism to distill the learned %knowledge from visiting novel states into adaptive policies that can %adapt to diverse goals at test-time. The policies learned are %reactive because the knowledge gained by visiting $novel$ states is %quickly forgotten when other states become more novel.

\noindent \textbf{Reachability and Curriculum Learning.} Our method is related to curriculum learning approaches in reinforcement learning \cite{approximate_hjb, curriculum_held, ELMAN199371, openai2019solving, curriculum_bengio, racaniere2019automated} whereby learning easier tasks is prioritized over hard tasks, as long as measures are taken to avoid forgetting behaviors on old tasks.   

\noindent \textbf{Frontier-based Exploration for Robot Mapping.} Finally, our method is intuitively similar to a large body of classic work on robot mapping, particularly frontier-based exploration approaches \cite{frontier_based_exploration, frontier_based_exploration_multirobot, frontier_based_exploration_holz}.


==> arxiv_version/7-conclusion.tex <==
 \vspace*{-0.2cm}
\section{Conclusion} 
 \vspace*{-0.2cm}
\label{sec:conclusion}
In this paper we proposed an algorithm for committed exploration, by keeping track of the frontier of reachable states, and during the start of every episode, executing a deterministic goal-conditioned policy to reach the current frontier, followed by executing a stochastic goal-conditioned exploration policy to reach the goal. The proposed approach can work directly over image-based observations and goal specifications, does not require any reward signal from the environment during training, and is completely self-supervised in that it does not assume access to the oracle goal-sampling distribution for evaluation. Through experiments on eight environments with varying characteristics, task complexities, and temporal abstractions, we demonstrate the efficacy of the proposed approach over state of the art exploration baselines.


==> neurips/1-introduction.tex <==
\vspace*{-0.3cm}
\section{Introduction}
\label{sec:intro}  
\vspace*{-0.3cm}
%Reinforcement Learning (RL) enables agents to learn complex skills by interacting with the environment, alleviating the need for manual engineering of behavioral skills.
Efficient exploration is one of the central open challenges in Reinforcement Learning (RL), and a key requirement for learning optimal policies, particularly in sparse-reward and long-horizon settings, where the optimization problem is difficult to solve, but easy to specify. We show that discovering policies for  these settings benefits significantly from autonomous goal-setting and exploration, which requires keeping track of what regions of the state-space have been sufficiently explored and can be reached via planning, and what regions remain unknown. In this paper we present an exploration method that keeps track of reachable regions of state space and naturally handles the exploration-exploitation dilemma in sequential decision-making for unknown environments~\cite{varibad,goexplore}, while being practical in real robotics settings. In addition to experimental evaluation, we also show proofs for simplified exploration settings based on expected reaching time analysis. \HB{General introduction}


%One of the central challenges in Reinforcement Learning (RL) is to learn large general purpose repertoires of behaviors that can be used for solving  complex tasks, without undertaking the time-consuming and potentially intractable job of learning each behavior separately. Such self-supervised discovery of composable behaviors for solving temporally extended tasks requires agents to autonomously explore the environment, keep track of what regions of the state-space have been sufficiently explored and can be reached, and hence naturally relates to the exploration-exploitation dilemma in sequential decision-making in unknown environments~\cite{varibad,goexplore}. \HB{General introduction}



For learning to plan in \textit{unknown} environments, appropriately trading off exploration i.e. learning about the environment, and exploitation i.e. executing promising actions is the key to successful policy learning. The necessity for this trade-off is more pertinent when we want to train agents to learn autonomously in a self-supervised manner such that it is able to solve goals sampled from an unknown distribution during evaluation. In this setting, during training, the agent must practice reaching self-specified random goals~\cite{rig}. However, trying to specify goals through exact states of objects in the environment will require a combinatorially large representation, for explicitly randomizing different variables of the states~\cite{avi,rig}. On the contrary, raw sensory signals, such as images can be used to specify goals, as has been done in recent goal-conditioned policy learning algorithms~\cite{rig,upn,skew}\HB{In the previous two lines I am trying to motivate the need for learning from images even in simulation. In the real environment it is clear why we want to use images as input - we cannot describe the environment state exactly.}. This paper tackles the question of how should an autonomous agent balance exploration and exploitation for goal-directed robotic tasks while learning directly from images, with no access to the ground-truth parameters of the environment during training. 
%Specifically, we focus our attention to the problem of keeping track of the frontier of reachable states, and using latent space reachability measures to devise efficient exploration algorithms in the above setting. \HB{The problem being considered. It is slightly vague because I intended this to be a description of the problem, not the solution. I would appreciate help to make it more crisp though.}

\begin{figure}
    \centering
  \begin{minipage}[c]{0.63\textwidth}
   \includegraphics[width=\columnwidth]{neurips/firstfigbetter.png}
  \end{minipage}
   \begin{minipage}[c]{0.35\textwidth}
    \caption{LEAF prioritizes reaching the current frontier of reachable states with a deterministic policy, and performing goal-directed exploration beyond it with a stochastic policy. Here, the yellow region corresponds to puck positions for the currently reachable frontier corresponding to the shown initial state.} \label{fig:firstfig}
\end{minipage}    
    \vspace*{-0.8cm}
\end{figure}
% In this paper, we attempt to mitigate the exploration-exploitation tradeoff in self-supervised learning of goal-conditioned policies directly from images by keeping track of the frontier of reachable states, and performing committed exploration. 



The main idea of our approach is to maintain and gradually expand the frontier of reachable states by trying to reach the current frontier directly without exploring and exploring from beyond the current frontier in order to reach the goal (Fig.~\ref{fig:firstfig}). In order to achieve this, we encourage the agent to sample goals closer to the start state(s) before sampling goals that are farther away, by appropriately querying the reachability network. 
% Planning directly in the pixel-space is not meaningful. For example, computing rewards as the pixel-wise distance between two images does not necessarily correspond to a semantically meaningful correlation with respect to how close the two ground-truth states actually are~\cite{upn,rig}. 
Since planning directly in the pixel-space is not meaningful~\cite{upn,rig}, we learn a latent representation from images, and plan in the latent space. We train a reachability network that learns whether a latent state is currently reachable from another latent state in $k$ time-steps ($k$ varies from $1$ to the maximum length of the horizon), and use this network to compute the current frontier of reachable states given a random initial start state during training. While training the goal-conditioned policy to reach a goal latent state (corresponding to a goal image), we first execute the deterministic policy trained so far to reach a latent state at the frontier (\textit{commitment}), and then execute the stochastic policy from beyond the frontier to reach the goal (\textit{exploration}). We refer to this procedure of commitment to reach the frontier and exploring beyond it as \textit{committed exploration} required for solving temporally abstracted tasks. \HB{The proposed approach. Every episode in training has two phases - execute deterministic policy to reach frontier. Explore beyond frontier while trying to reach goal. I don't mean to say the second phase here is "deep exploration". The overall scheme of having this two stage approach is enforcing deep exploration - to discover temporally abstracted winning sequences of actions that solve the task - this process happens completely at the end of training, when the reachable frontier = real frontier.}

%In order to impose this curriculum over the self-supervised sampling of goals during training, we gradually increase the max. horizon length of episodes during successive epochs of training. 

This paper makes the following contributions:
\begin{enumerate}
%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]
 \item We propose a dynamics-aware latent space reachability network.
 \item We devise a policy learning scheme using the reachability network that combines deterministic and stochastic policies for committed exploration. 
 \item We empirically evaluate the proposed approach  in a range of both image-based, and state-based simulation environments, and in a real robot environment. We demonstrate an improvement of $20\%$ on average compared to state-of-the-art exploration baselines. 
\end{enumerate}


%Since the proposed approach explicitly keeps track of reachability for committed exploration, we call our approach ReachExplore. 
% Through detailed experimentation across image-based simulation environments, a state-based simulation environment, and a real-world robotic environment, we show that ReachExplore successfully solves difficult temporally-extended tasks by achieving much higher rewards and converging with much less interactions with the environment as compared to state-of-the art image-based exploration methods. \HB{image based methods.} \HB{A brief highlight of the results. To put in specifics if needed later.}

==> neurips/2-preliminaries.tex <==
\vspace*{-0.2cm}
\section{Problem Setup and Background}
\vspace*{-0.4cm}
% In this section, we elaborate on the key concepts and paradigms that relate to the proposed approach, and lay out the mathematical notations for the rest of the paper.
\label{sec:prelim}

% \subsection{Problem Setup}
% In standard model-free RL, the objective is to learn a policy $\pi(\cdot)$ as a function of the current state of the world $s_t$ (this could be a latent abstraction state as well) that outputs an action $a_t=\pi(s_t)$ to be executed in the environment, such that the expected sum of discounted returns from the environment $R_t=\mathbb{E}_{\pi(a|s),p(s'|s,a)} [\sum_{i=t}^T\gamma^{(i-t)}r(s_i,a_i,s_{i+1})]$ is maximized. Here, $a\in\mathcal{A}$, $s\in\mathcal{S}$, $\gamma$, and $r(\cdot)$ respectively denote an action in the set of actions, a state in the set of states, the discount factor, and the reward function.

% \noindent \textbf{ Goal-conditioned policies} This formulation is insufficient when we want to optimize expected returns with respect to different goals that can be specified at test-time. Hence, explicitly conditioning the policy on the goal $s_g$ that must be achieved in the current episode, $a_t=\pi(s_t;s_g)$, and optimizing the expected sum of discounted rewards over different goals $s_g$ sampled from the set of goals $s_g\sim\mathcal{G}$, $R_t=\mathbb{E}_{\pi(a|s;s_g),p(s'|s,a)} [\sum_{i=t}^T\gamma^{(i-t)}r(s_i,a_i,s_{i+1};s_g)]$  is a common method of learning policies that can be adapted to different goals at test time~\cite{her}.

% \noindent \textbf{Self-supervised learning to solve goals} We consider the setting of learning directly from images, such that the the goals are specified as images to the policy. Also, the setting is self-supervised in the sense that during training, we do not have access to any oracle goal-sampling distribution from which goals will be sampled at test-time. Hence, the agent must learn to autonomously set goals and solve them during training, in order to learn necessary re-usable skills for solving new goals sampled from an unknown distribution at test-time. 

% % This is the setting considered in a number of recent approaches for policy learning~\cite{skew,rig}, and is challenging because it assumes very less information about the ground-truth environment and goal-specifications. One of the desiderata as pointed out in Skew-Fit~\cite{skew} is to sample sufficiently diverse goals and learn to solve them, i.e. optimize $\mathcal{H}(\mathcal{G}) - \mathcal{H}(\mathcal{G}|\mathcal{S})$, where $\mathcal{H}(\cdot)$ denotes entropy. Although this guarantees uniform coverage in the infinite limit (assuming a perfectly learned goal-reaching policy), it does not ensure deep exploration in the finite horizon case.  \HB{Agreed that uniform coverage is not guaranteed for SkewFit in the general case. For showing this, SkewFit assumes a perfect oracle goal-reaching policy. But even if the goal-reaching policy is learned (not given by an oracle), then if we assume that it can be perfectly learned, the SkewFit analysis will still hold, and they can claim uniform coverage in the infinite limit. } In this paper, we emphasize the need to keep track of reachable states so to enable deep exploration via commitment, and set goals in a curriculum fashion, so that the agent learns to solve easier goals before trying to solve more difficult goals. 


  
% \subsection{Notation}

We denote the set of observations (images) as $\mathcal{S}$ and the set of goals (images) as $\mathcal{G}$. In this paper we assume the underlying sets for $\mathcal{S}$ and $\mathcal{G}$ to be the same (any valid image can be a goal image~\cite{rig,skew}) but maintain separate notations for clarity. $f_\psi(\cdot)$ denotes the encoder of the $\beta-VAE$~\cite{betavae} that encodes observations $s\sim S$ to latent states $z\sim f_\psi(s)$. The goal conditioned policy given the current latent state $z_t$, and the goal $z_g$ is denoted by $\pi_\theta(\cdot | z_t,z_g)$, and $a_t\sim \pi_\theta(\cdot | z_t,z_g)$ denotes the action sampled from the policy at time $t$. The policy $\pi_\theta(\cdot | z_t,z_g)$ consists of a deterministic component $\mu_\theta(\cdot | z_t,z_g)$, and a noise term $\epsilon$, such that $\pi_\theta(\cdot | z_t,z_g) = \mu_\theta(\cdot | z_t,z_g) + \sigma_\theta\epsilon$, where $\epsilon$ is a Gaussian $\mathcal{N}(0,\mathbf{I})$ in this paper. $ReachNet(z_i,z_j;k)$ denotes the reachability network that takes as input two latent states  $z_i$, and $z_j$ and is conditioned on a reachability integer $k\in[1,..,H]$, where $H$ is the maximum time horizon of the episode. The output of $ReachNet(z_i,z_j;k)$ is either a $0$ denoting $z_j$ is currently not reachable from $z_i$ or a $1$ denoting $z_j$ is reachable from $z_i$. 

We consider the problem setting where a robot is initialized to a particular configuration, and is tasked to reach a goal, specified as an image. The test time goal distribution, from which goal images will be sampled for evaluation is not available during training, and hence the training approach is completely self-supervised. The underlying distribution of observations $\mathcal{S}$ is same as the underlying distribution of goals $\mathcal{G}$ during training, and both are distributions over images from a camera.


==> neurips/3-approach.tex <==
\vspace*{-0.2cm}
\section{Our Approach}
\label{sec:approach}
In this section, we discuss the specifics of the proposed approach, summarized in Algorithm~\ref{alg:mainbrief} .
\begin{figure*}[t]
\centering
   \hspace*{-0.9cm}
        \begin{subfigure}[b]{0.7\textwidth}
               \centering
    \includegraphics[width=0.9\textwidth]{arxiv_version/figures/ReachExploreMainfig_updated.png}
    \caption{Schematic of the proposed approach}
    \label{fig:reachidea}
        \end{subfigure}% \\
        \hspace*{-0.4cm}
         \begin{subfigure}[b]{0.37\textwidth}
               \centering
    \includegraphics[width=\textwidth]{reachnet.png}
    \caption{Reachability Network}
    \label{fig:reachnet}
        \end{subfigure}                 %\quad
     \caption{(a) An overview of our method on the Sawyer Push and Reach task. The initial and goal images are encoded by the encoder of the VAE into latents $z_0$ and $z_g$ respectively. Random states are sampled from the currently learned manifold of the VAE latent states, and are used to infer the current frontier $p_{k^*}$ as described in Section~\ref{sec:reachidea}. The currently learned deterministic policy is used to reach a state in the frontier $z^*$ from the initial latent state $z_0$. After that, the currently learned stochastic policy is used to reach the latent goal state $z_g$. A reconstruction of what the latent state in the frontier $z^*$ decodes to is shown. For clarity, a rendered view of the actual state $\hat{z}^*$ reached by the agent is shown alongside the reconstruction. (b) A schematic of the reachability network used to determine whether the latent state $z_j$ ($state_j$) is reachable from the latent state $z_i$ ($state_i$) in $k$ time-steps. The reachability vector $\mathbf{k}$ consists of a vector of the same size as $z_i$ and $z_j$ with all its elements being $k$. The output $0$ indicates that state $z_i$ is not reachable from state $z_j$.} 
 \label{fig:mainfig}
 \vspace*{-0.2cm}
\end{figure*}
%\subsection{Setup}


%either a third person view (in the real robot experiment) or from a camera mounted on the robot arm (in all the simulation experiments). 

%  \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{reachnet.png}
%     \caption{A schematic of the reachability network used to determine whether the latent state $z_i$ is reachable from the latent state $z_j$ in $k$ time-steps. The reachability vector $\mathbf{k}$ consists of a vector of the same size as $z_i$ and $z_j$ with all its elements being $k$. The output $0$ indicates that state $z_i$ is not reachable from state $z_j$.}
%     \label{fig:reachnetwork}
% \end{figure}

% \begin{figure*}[h!]
% \centering
%   \hspace*{-0.9cm}
%         \begin{subfigure}[b]{0.30\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{illustrative_figs/reach_vae1.PNG}
%     \caption{Sampling from the VAE}
%     \label{fig:vaegeneral}
%         \end{subfigure}% \\
%         \hspace*{-0.2cm}
%       %\vspace*{-2cm}
%          \begin{subfigure}[b]{0.30\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{illustrative_figs/vae_one_episode_pushreach1.PNG}
%     \caption{Traversal in the latent space}
%     \label{fig:vaeepisode}
%         \end{subfigure}   
%          \hspace*{-0.1cm}
%         \begin{subfigure}[b]{0.4\textwidth}
%               \centering
%   \includegraphics[width=\textwidth]{illustrative_figs/analysis2.PNG}
%     \caption{Analysis of ReachExplore}
%     \label{fig:analysis1}
%           \end{subfigure}   
%          \hspace*{-0.9cm}%\quad
%     \caption{(a) ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red). (b) This figure shows how sampling goals that lie on the latent VAE manifold and traversing on the latent manifold leads to latent states that decode to realistic dynamically feasible image frames.\
%     (c) The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (3) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it executes the stochastic policy for $T-k^*$ steps. (2) shows the case when the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then executes the stochastic policy for $T-k$ steps. This is similar in principle to the high level idea of Go-Explore~\cite{goexplore} (1) shows the case when the agent executes the stochastic policy for $T$ steps starting at the origin. The simplified Go-Explore and SkewFit~\cite{skew} models are described in Section~\ref{sec:analysis}}
%     \label{fig:vae}
%     \vspace*{-0.5cm}
% \end{figure*}

%  remove space after algo float  
% \setlength{\textfloatsep}{5pt}% Remove \textfloatsep


\subsection{The Key Insight of LEAF}
\label{sec:reachidea}
Consider the goal conditioned policy $\pi(\cdot | z_t,z_g)$ with an initial latent state $z_0$, and a goal latent state $z_g$. The key idea of our method is to do committed exploration, by directly going to the frontier of reachable states for $z_0$ by executing the deterministic policy $\mu_\theta(\cdot | z_t,z_{k^*})$ and then executing the exploration policy $\pi_\theta(\cdot | z_t,z_g)$ from the frontier to perform goal directed exploration for the actual goal $z_g$. The frontier defined by $p_{k^*}$ is the empirical distribution of states that can be reliably reached from the initial state, and are the farthest away from the initial state, in terms of the minimum number of timesteps needed to visit them. The timestep index $k^*$ that defines how far away the current frontier is, can be computed as follows:
$$\argmax_k(IsReachable(z_0;k)) $$
The binary predicate  $IsReachable(z_0;k)$ keeps track of whether the fraction of states in the empirical distribution of $k-$reachable states $p_k$ is above a threshold $1-\delta$. The value of $IsReachable(z_0;k)$ $\forall k\in[1,..,H]$ before the start of the episode from $z_0$ is computed as:
%IsReachable(k)==True \text{iff}
\begin{equation}
       =\begin{cases}
      True, & \text{if}\ \mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)\geq 1 - \delta \\
      False, & \text{otherwise}
    \end{cases}
  \end{equation}
Here  $p_\phi(z)$ is the current probability distribution of latent states as learned by the $\beta-VAE$~\cite{betavae} with encoder $f_\psi(\cdot)$. $\delta$ is set to 0.2. For computing $\mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)$ above, we randomly sample states $z\sim p_\phi(z)$ from the latent manifold of the VAE, the intuition of which is illustrated in Fig.~\ref{fig:vae}. After calculating all the predicates $IsReachable(z_0;k)$ $\forall k\in[1,...,H]$ and determining the value of $k^*$, we sample a state $z_{k^*}$ from the empirical distribution of $k^*-$reachable states, $p_{k^*}$, ensuring that it does not belong to any $p_{k}$ $ \forall k< k^*$. Here, the empirical distribution $p_k$ denotes the set of states $z$ in the computation of $\mathbb{E}_{z\sim p_\phi(z)}ReachNet(z_0,z;k)$ for which $ReachNet(z_0,z;k)$ returns a $1$, and  $ReachNet(z_0,z;k')$ returns a $0$, $\forall k'<k$.

In order to ensure that the sampled state $z_{k^*}$ is the closest possible state to the goal $z_g$ among all states in the frontier $p_{k^*}$, we perform the following additional optimization
\begin{equation}
    z_{k^*} = \argmin_{z\in p_{k^*}}||z-z_g||_2
\end{equation}
Here, $||\cdot||_2$ denotes the $L_2$ norm. The above optimization encourages choosing the state in the frontier that is closest in terms of Euclidean distance to the latent goal state $z_g$.


Our method encourages \textit{committed} exploration because the set of states until the frontier $p_{k^*}$ have already been sufficiently explored, and hence the major thrust of exploration should be beyond that, so that new states are rapidly discovered.  Algorithm~\ref{alg:mainbrief} shows an overview algorithm for our method. In our specific implementation, we use SAC~\cite{sac} as the base off-policy model-free RL algorithm for minimizing the Bellman Error in the overall algorithm that is described in the Appendix.

% The SkewFit~\cite{skew} approach showed that if the distribution over states is skewed to highly weigh rare states, and goals are sampled from this skewed distribution, the entropy over states $\mathcal{H}(\mathcal{S})$ will eventually approach the entropy of a uniform distribution $U_{\mathcal{S}}$ over the states. However, this is guaranteed in the infinite time limit. Applying our method with the SkewFit trick for sampling goals will still maintain the guarantee of maximum entropy, but improve sample efficiency of policy learning. Algorithm~\ref{alg:mainbrief} shows an overview algorithm for our method. In our specific implementation, we use SAC~\cite{sac} as the base off-policy model-free RL algorithm for minimizing the Bellman Error in the overall algorithm that is described in the Appendix.




% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{reach_vae.PNG}
%     \caption{ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red).}
%     \label{fig:vae}
% \end{figure}


% \begin{figure}[t]
%     \centering
%      \begin{subfigure}[b]{0.6\columwidth}
%               \centering
%     \includegraphics[width=0.9\columwidth]{illustrative_figs/reach_vae.PNG}
%     \caption{Forward pass of the ReachExplore approach}
%     \label{fig:reachidea}
%         \end{subfigure}% \\
%          \begin{subfigure}[b]{0.4\columwidth}
%               \centering
%      \includegraphics[width=\columnwidth]{illustrative_figs/vae_one_episode.PNG}
%     \caption{Simulation of one episode}
%     \label{fig:reachidea}
%         \end{subfigure}% \\
%     \caption{ReachExplore samples latent goals from the manifold of the learned VAE latent space $p_\phi(z)$. Sampling states from outside the manifold is likely to correspond to images (upon decoding) that do not correspond to a dynamically feasible image of a simulator state. For example, in this figure, given some latent state in the manifold (shown by the center of the spehere), states outside the manifold correspond to regions of the sphere (outlined in pink) that do not intersect the manifold (the intersection is outlined in red).}
%     \label{fig:vae}
% \end{figure}


\begin{algorithm}[H]
	\begin{algorithmic}[1]
		\Procedure{Overall}{GCP $\mu_\theta$, $\pi_\theta$, Prior $p(z)$, $S$, $f_\psi(\cdot)$, $IsReachable(\cdot)$, $H_0$, $N$, $\epsilon$, $\delta$, ReplayBuffer $\mathcal{B}$}
		\State $p_\phi = p(z)$
		\State Init $ReachNet(\cdot,\cdot; k)$, Def ReachData $\mathcal{D}$, $K=H_0N$
% 			\State Initialize $ReachNet(\cdot,\cdot; k)$ where $k=\{K,...,1\}$ 
% 			\State Def $K=H_0*N$ lists for $p_k$.
% 			\State Def Global ReachDataset = $\{ \}$ //to train $ReachNet$
		\For{episodes = 1 to $N$}
		\State $s_0\sim S_0$, encode $z_0=f_\psi(s_0)$, $z_{g}\sim p_\phi,\hat{z}^*=z_0$
% 		\State Sample initial state $s_0\sim S_0$, encode $z_0=f_\psi(s_0)$
% 		\State Sample latent goal $z_{g}$ from $p_\phi=p_{skewed}$
    %\State $\hat{z}^*=z_0$
    % \State //\texttt{Apply ReachExplore idea after some training}
	\If{episodes $\geq$ $N/4$} 
	 \For{$k=K-1,...,1$}
	\State Set the value of $IsReachable(z_0;k)$
	 \EndFor
% 			 \State Sample $M$ latent states $\{z\}_M\sim p_{\phi}$
% 	 \For{$k=K_{max},...,1$, $\forall z\in\{z\}_M$}
% 	 \State Initialize list $p_k\longleftarrow\{\}$
	
% 	  \If{$\frac{1}{k-1}\sum_{i=1}^{k-1}	 ReachNet(z,z_0;i)\geq 1-\epsilon$} 
% 	  \State Append $z$ to $p_k$
% 	  \EndIf
% 	  \For{counter = 1 to $C$}
% 	  \State Sample a latent state $z\sim p_k$
% 	   \If{$ReachNet(z,z_0;k)$}
% 	  \State c = c+1
% 	  \EndIf
% 	  \EndFor
% 	  \If{$\frac{c}{C}\geq 1-\epsilon$} 
% 	  \State Set $IsReachable(k)==True$
% 	  \EndIf
% 	  \EndFor
	  \State  $k^*=\argmax_k(IsReachable(z_0;k))$ 
	  \State Choose $ z_{k^*} = \argmin_{z\sim p_{k^*}}||z-z_g||_2$
	  	% 	\State //Set initial latent state to be $z^*$
	  	\State Exec $\pi_\theta(z_0;z_{k^*})$, reach $\hat{z}^*$ s.t. $||\hat{z}^*-z_{k^*}||\approx 0$
	  	\EndIf
		\State Set $H=H_0*episodes$ // \texttt{Curriculum} 
		\For{$t=0,...,H-1$}
		\If{$t==0$}
		\State Select $a_t\sim\mu_\theta(\hat{z}^*;z_{g})$ and execute it
		\EndIf
		\If{$t>0$ and $t<k^*$}
		\State Select $a_t\sim\mu_\theta(f_\psi(s_t);z_{g})$ and execute it
		\EndIf 
			\If{$t>0$ and $t\geq k^*$}
		\State Select $a_t\sim\pi_\theta(f_\psi(s_t);z_{g})$ and execute it
		\EndIf 
		\State // \texttt{Store tuple and Train policy}
		\State \textsc{StoreandTrain()}
		\EndFor 
%\State //Append to the dataset for training the ReachNet
%\State //Append observations and labels to $\mathcal{D}$
\State \textsc{AppendtoDataset($\mathcal{D}$)}
% \For{$t_1 = 0,...,H-1$}
% \For{$t_2 = 0,...,H-1$}
% \If{$t_1\neq t_2$}
% \State ReachDataset.add($(z_{t_1},z_{t_2},|t_1-t_2|)$)
% \EndIf
% \EndFor
% \EndFor

		

% 	\EndFor
%\State // Samples states to add in replay buffer $\mathcal{R}$
% \State //\texttt{Replay with goals as previously seen states}
\State \textsc{SampleFutureStates($\mathcal{B}$)}
% 	\For{$t=0,...,H-1$}
% 	\For{$i=0,...,k-1$}
%     \State Sample future states $s_{h_i}, t\leq h_i-1 \leq H-2$
%     \State Store $(s_t,a_t,s_{t+1},f_\psi(s_{h_i}),h_i+1)$ in $\mathcal{R}$
%     	\EndFor
%     		\EndFor
    \State Construct skewed dist.  $p_{skewed}$ from $\mathcal{B}$ (Skew-Fit) 
    \State Train the encoder using $p_\phi = p_{skewed}$
    \State Train $ReachNet(\cdot,\cdot; k)$ using ReachDataset $\mathcal{D}$
		\EndFor
		\EndProcedure
	\end{algorithmic}
	\caption{Overview of the proposed Algorithm (Subroutines are in the Appendix)}
	\label{alg:mainbrief}
\end{algorithm}
% \end{minipage}
%   \end{wrapfigure}

\subsection{Training the Reachability Network}
\label{sec:trainreachnet}
\vspace*{-0.2cm}
The reachability network $ReachNet(z_i,z_j;k)$ is a feedforward neural network with fully connected layers and ReLU non-linearities, the architecture of which is shown in Fig.~\ref{fig:mainfig}, with details in the Appendix. The architecture has three basic components, two encoders ($encoder_{\mathbf{state}}$, $encoder_{\mathbf{reach}}$), one decoder, and one concatenation layer. The latent states $z_i,z_j$ are encoded by the same encoder $encoder_{\mathbf{state}}$ (i.e. two encoders with tied weights, as in a Siamese Network~\cite{siamese}) and the reachability value $k$ is encoded by another encoder $encoder_{\mathbf{reach}}$. In order to ensure effective conditioning of the network $ReachNet$ on the variable $k$, we input a vector of the same dimension as $z_i$ and $z_j$, with all of its values being $k$, $\mathbf{k}=[k,k,...,k]$.

It is important to note that such neural networks conditioned on certain vectors have been previously explored in literature, e.g. for dynamics conditioned policies~\cite{mangapfn}. The three encoder outputs, corresponding to $z_i, z_j,$ and $k$ are concatenated and fed into a series of shared fully connected layers, which we denote as the decoder. The output of  $ReachNet(z_i,z_j;k)$ is a $1$ or a $0$ corresponding to whether $z_j$ is reachable from $z_i$ in $k$ steps or not, respectively.

To obtain training data for $ReachNet$, while executing rollouts in each episode, starting from the start state $z_0$, we keep track of  the number of time-steps needed to visit every latent state $z_i$ during the episode. We store tuples of the form $(z_i,z_j,k_{ij})$ $\forall i<j$ in memory, where $k_{ij} = j-i$, corresponding to the entire episode. Now, to obtain labels $\{0,1\}$ corresponding to the input tuple $(z_i,z_j,k)$, we use the following heuristic:
\begin{equation}
       label(z_i,z_j,k) =\begin{cases}
      1, & \text{if}\ |k_{ij} > \alpha k|\\
      0, & \text{if}\  |k_{ij} < k|
    \end{cases}
  \end{equation}
Here $\alpha$ is a threshold to ensure sufficient separation between positive and negative examples. We set $\alpha=1.3$ in the experiments, and do not tune its value.

%may include the bi about symmetric inputs bein fed to ensure the learned notion of symmetry 
\subsection{Implicit Curriculum for Increasing the Frontier}
\label{sec:curricula}
% In Sections~\ref{sec:reachidea} and~\ref{sec:trainreachnet}, we described the ReachExplore approach and demonstrated the computation of the current frontier. 
% Central to ReachExplore is the idea of repeatedly increasing the frontier of reachable states during training. It is crucial to note that for the ReachExplore approach of gradually increasing the frontier of exploration to succeed, it must be ensured that in-distribution nearby goals are sampled before goals far away.
The idea of growing the set of reachable states during training is vital to LEAF. Hence, we leverage curriculum to ensure that in-distribution nearby goals are sampled before goals further away.
This naturally relates to the idea of a curriculum~\cite{curriculum}, and can be ensured by gradually increasing the maximum horizon $H$ of the episodes. So, we start with a horizon length of $H=H_0$ and gradually increase it to $H=NH_0$ during training, where $N$ is the total number of episodes.

In addition to this, while sampling goals we also ensure that the chosen goal before the start of every episode does not lie in any of the $p_k$ distributions, where $k\leq k^*$ corresponding to the calculated $k^*$. This implies that the chosen goal is beyond the current frontier, and hence would require exploration beyond what has been already visited.

%\subsection{Overall Algorithm}
    
%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{illustrative_figs/reachexplore_analysis_all.PNG}
%     \caption{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (c) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it randomly explores for $T-k^*$ steps. (b) shows the case when ReachExplore is not employed, and the agent first goes to a random previously visited state, by executing a deterministic goal reaching policy (say, for $k$ steps), and then randomly explores for $T-k$ steps. This is similar in principle to the high level idea of Go-Explore~\cite{goexplore} (a) shows the case when ReachExplore is not employed, and the agent starts doing random exploration for $T$ steps starting at the origin. This is similar in principle to SkewFit~\cite{skew}.}
%     \label{fig:analysis1}
% \end{figure}





%   \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{analysis.png}
%     \caption{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode. (a) shows the case when with probability $\chi$, the deterministic goal reaching policy takes the agent to a state at the frontier in $k^*$ steps, and after that it randomly explores for $T-k^*$ steps. (b) shows the case when with probability $1-\chi$, the goal-reaching policy fails to take the agent to the frontier, and ends up somewhere within the already explored blue region. After that the  agent randomly explores for $T-k^*$ steps. Note that for computing the lower bound $L_1$, we consider the worst case when the circle of radius $\sqrt{T-k^*}$ is contained within the circle of radius $k^*$. (c) shows the case when ReachExplore is not employed, and the agent starts doing random exploration for $T$ steps starting at the origin.}
%     \label{fig:analysis}
% \end{figure}


==> neurips/4-analysis.tex <==
\vspace*{-0.5cm}
\section{Analysis: Intuition of deep exploration through average case analysis}
\label{sec:analysis}
\vspace*{-0.3cm}
In this section, we provide formal analysis of our method in a simplified, idealized, setting. Consider a 2D world with a single start location $\mathbf{z}_0$ and and let the goal be denoted by $\mathbf{z}_g$. Let $p_{k^*}$ denote the current frontier. Let $T$ denote the total time-steps in the current episode. 
% We aim to show that using this time-step budget, the odds of exploring previously unvisited states farther away from the start state are higher when using LEAF, as compared to without using it. 
% Let $\chi$ denote the probability of the deterministic goal-conditioned policy reaching a goal state in $p_{k^*}$ in $k^*$. 
For simplicity, we assume the stochastic goal-reaching policy to be the policy of a random walker, and the deterministic goal-reaching policy to be near-optimal in the sense that given a target goal in $p_{k^*}$, and an initial state in the already explored region, it can precisely reach the  target location at the frontier with a high probability($\gg0$). For analysis, we define SkewFit~\cite{skew}, GoExplore~\cite{goexplore}, and our method in the above setting to be the following simplified schemes, and illustrate the same in Fig.~\ref{fig:simpleanalysis}. To clarify, this is a simplified setup for analysis, and is not our experimental setup in section~\ref{sec:exp}.
\begin{enumerate}

%[
%    topsep=0pt,
%    noitemsep,
%    leftmargin=*,
%    itemindent=12pt]

    \item \textbf{SkewFit-variant:} The model that executes the stochastic policy for the entire length $T$ of the episode to reach goal $z_g$, and sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
    \item \textbf{GoExplore-variant:} The model that first chooses a random previously visited intermediate latent goal state from the archive (not necessarily from the frontier $p_{k^*}$), executes a deterministic goal directed policy for say $k$ steps to reach the intermediate goal, and then executes the stochastic policy exploring for the next $T-k$ steps. For analysis, $0<k<k^*$. This is similar in principle to the idea of Go-Explore~\cite{goexplore}\footnote{Here, we refer to the intuition of Phase 1 of Go-Explore, where the idea is to ``select a state from the archive, go to that state, start exploring from that state, and update the archive." For illustration and analysis, we do not consider the exact approach of Go-Explore. In order to ``go to that state" Go-Explore directly resets the environment to that state, which is not allowed in our problem setting. Hence, in Fig.~\ref{fig:simpleanalysis}, we perform the analysis with a goal-directed policy to reach the state. Also, since Go-Explore does not keep track of reachability, we cannot know whether the intermediate goal chosen can be reached in $k$ timesteps. But for analysis, we assume the intermediate goal is chosen from some $p_k$ distribution as described in Section~\ref{sec:reachidea}}. It also sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
    \item \textbf{Our method:} The model that first chooses a state from the frontier $p_{k^*}$, executes a deterministic goal directed policy for say $k^*$ steps to reach the frontier, and then executes the stochastic policy exploring for the next $T-k^*$ steps.  It also sets diverse goals at the start of every episode, as per the SkewFit objective~\cite{skew}.
\end{enumerate}


\begin{figure}[t]
\begin{minipage}[c]{0.49\textwidth}
               \centering
   \includegraphics[width=\textwidth]{neurips/analysis_simplified.png}
  \end{minipage} 
  \begin{minipage}[c]{0.45\textwidth}
    \caption{The blue area of radius $k^*$ denotes the already sufficiently explored region such that $k^*$ is the current frontier. $T$ is the max. number of timesteps of the episode.  The simplified models and results are described in Section~\ref{sec:analysis}}
    \label{fig:simpleanalysis}
\end{minipage}    
\vspace*{-0.5cm}
          \end{figure}


%From the theory of hitting times in 2D random walks, we have the following result.
\begin{lemma}
For a random walk with unit step size in 2D (in a plane), the average distance away from a point (say, the origin) traversed in $t$ time-steps is $\sqrt{t}$.
\label{lemma:main}
\end{lemma}
% \begin{proof}
% The proof of is provided in the Appendix.
% % In a plane, consider the sum of $t$ 2D vectors with random orientations. For convenience, we use the phasor notation, and so assume the phase of each vector to be random. Starting at some point (let's call it the origin $z_0$), we assume $t$ steps are taken in an arbitrary direction, which is equivalent to assuming that the angle $\theta$ of the phasors is uniformly distributed in $[0,2\pi)$. The position $z_t$ in the complex plane after $t$ steps is:
% % $$ z_t = \sum_{k=1}^te^{i\theta_k}$$
% % The square of the absolute value of $z_t$is:
% % $$ |z_t|^2 = \sum_{k=1}^te^{i\theta_k}\sum_{m=1}^te^{-i\theta_m}
% % = t + \underset{k=1,m=1,k\neq m}{\sum\sum^t}e^{i(\theta_k-\theta_m)}$$
% % Now, we calculate the expected value of the $|z_t|^2$ variable by noting that since $\theta_k$ and $\theta_m$ are randomly sampled in $[0,2\pi)$ with uniform probability, the displacements $e^{i\theta_k}$ and $e^{i\theta_m}$ are random variables, so their difference corresponding to $\theta_k-\theta_m$ is also a random variable and has an expected value (mean) of $0$. Hence,
% % $$<|z_t|^2> = t \implies |z_t|_{rms} = \sqrt{t}$$

% % So, the average (root-mean-square) distance traversed after $t$ steps starting at some $z_0$ in the 2D plane is $\sqrt{t}$
% \end{proof}
\noindent The subsequent results are all based on the above stated lemma and assumptions. All the proofs are present in the Appendix.
\begin{lemma}
Starting at $z_0$ and assuming the stochastic goal-reaching policy to be a random walk, on average the SkewFit scheme will reach as far as $R_1 =\sqrt{T}$ at the most in one episode.
\end{lemma}
% \begin{proof}
% This follows directly from Lemma~\ref{lemma:main} by setting $t=T$, where $T$ is the max. number of timesteps in the episode.
% \end{proof}
% \vspace{-0.3cm}
% The lemma is illustrated in the first figure (1) of Fig.~\ref{fig:analysis1}, and is similar in principle to the basic SkewFit~\cite{skew} approach because at the start of each episode a stochastic goal-directed policy is rolled out from the initial state.

% In the second figure (2) of Fig.~\ref{fig:analysis1}, we consider a situation where a random previously visited intermediate latent goal state from the archive is chosen (not necessarily from the frontier $p_{k^*}$). Then the agent executes a deterministic goal directed policy for say $k$ steps to reach the intermediate goal, and then executes the stochastic policy exploring for the next $\sqrt{T-k}$ steps. For analysis, $0<k<k^*$. This is similar in principle to the idea of Go-Explore~\cite{goexplore}\footnote{Here, we refer to the intuition of Phase 1 of Go-Explore, where the idea is to ``select a state from the archive, go to that state, start exploring from that state, and update the archive." For illustration and analysis, we do not consider the exact approach of Go-Explore. In order to ``go to that state" Go-Explore directly resets the environment to that state, which is not allowed in our problem setting. Hence, in Fig.~\ref{fig:analysis1}(b), we perform the analysis with a goal-directed policy to reach the state. Also, since Go-Explore does not keep track of reachability, we cannot know whether the intermediate goal chosen can be reached in $k$ timesteps. But for analysis, we assume the intermediate goal is chosen from some $p_k$ distribution as described in Section~\ref{sec:reachidea}}. 

%In this case, the maximum average distance away from the origin traversed by the agent is atmost $r=\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$.
\begin{lemma}
Starting at $z_0$ and assuming the deterministic goal-deterministic policy to be near optimal (succeeds with a very high probability$>>0$), and the stochastic goal-reaching policy to be a random walk, on average GoExplore scheme will be bounded by $R_2 =\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$ in one episode.
\label{lemma:goexplore}
\end{lemma}
% \begin{proof}
% Since GoExplore first goes to a random previously visited state using the deterministic goal conditioned policy, from Fig~\ref{fig:analysis1} it is evident that the distance of such a state from the start state could be in the range $(0,k^*)$. Let this distance be $k$. Then, from Lemma~\ref{lemma:main}, the max distance on average traversed by the agent from $z_0$, if the intermediate state is at a distance $k$, can be given as:
% $$ r_k = k + \sqrt{T-k}$$
% Averaging over all the distance of all possible intermediate positions $k\in(0,k^*)$, we obtain the final averaged maximum distance reached by the agent in one episode as:
% $$R_2 = \frac{1}{k^*}\sum_{k=0}^{k^*}(k+\sqrt{T-k})$$
% %\vspace{-0.2cm}
% \end{proof}
% \vspace{-0.3cm}

% From the theory of hitting times in 2D random walks where at each timestep, the agent can move by 1 unit in any direction~\cite{hitting}, the average distance away from the origin traversed in $t$ steps is $\sqrt{t}$ \HB{Not a grid graph. This is for moving in free space, starting at a fixed point, where at each timestep the agent moves by 1 unit - so the agent can take discrete steps. We had discussed this on the whiteboard}. Hence, considering the stochastic policy (which for simplicity of analysis we considered to be a random walk), the maximum distance on average from $\mathbf{s}_0$ traversed in $T$ time-steps is $\sqrt{T}$. 



% While, if we employ ReachExplore, the maximum distance on average is atmost $k^* + \sqrt{T-k^*}$, as described in the following lemma:
\begin{lemma}
Starting at $z_0$ and assuming the deterministic  goal-conditioned policy to be near optimal (succeeds with a very high probability $>>0$), and the stochastic goal-reaching policy to be a random walk, on average our method will be bounded by $R_3 = k^* + \sqrt{T-k^*}$
\end{lemma}
% \begin{proof}
% In the proof for lemma~\ref{lemma:goexplore}, setting $k=k^*$ in the formula, for $r_k$ gives us the maximum average distance for our method as:
% $$R_3 =  k^* + \sqrt{T-k^*}$$
% %\vspace{-0.2cm}
% \end{proof}
% \vspace{-0.3cm}
\begin{theorem}
$R_3>R_2$ $\forall k^*\in[1,T)$ and $R_3>R_1$ $\forall k^*\in[1,T)$. i.e. After the frontier $k^*$ is sufficiently large, the maximum distance from the origin reached by our method is more than both GoExplore and SkewFit.
\label{lemma:final}
\end{theorem}
% \begin{proof}
% We provide the proof of this in the Appendix.
% \end{proof}

% In the Appendix we show that for values of $k^*>T/4$, $k^* + \sqrt{T-k^*}$ is always greater than  $r=\frac{1}{k^*}(\sum_{k=0}^{k^*}(k + \sqrt{T-k})$.
\noindent Theorem~\ref{lemma:final} is the main result of our analysis and it intuitively suggests the effectiveness of deep exploration guaranteed by our method. This is shown through a visualization in Fig.~\ref{fig:simpleanalysis}. 

% In Fig.~\ref{fig:simpleanalysis}\,(2) and (3), we assume the deterministic policy succeeds with high probability($\gg0$), which is usually the case after sufficient training iterations in off-policy Q-learning. It can be easily seen that if $k^*$ increases during training (i.e. the reachable frontier expands), then after a finite number of interactions with the environment, we will have $k^*>\sqrt{T}$. We ensure that this happens because of the implicit curriculum on horizon length, and the sampling of goals beyond the current reachable frontier at the start of every episode.




% \subsection{Fast(er) coverage guarantees through average case analysis (Sec to be commented)}
% In this section, we provide theoretical justifications for why applying the ReachExplore trick ensures faster coverage. Consider a 2D world with a single start location $\mathbf{s}_0$ and and let the goal be denoted by $\mathbf{s}_g$. Let $k^*$ denote the current frontier. Let $T$ denote the total number of time-steps in the current episode. We sim to show that using this time-step budget, the odds of exploring previously unvisited states are higher when using ReachExplore, as compared to without using it. Let $\chi$ denote the probability of the deterministic goal-conditioned policy reaching a goal state in $p_{k^*}$ in $k^*$. For simplicity, we assume the stochastic goal-reaching policy to be the policy of a random walker. 

% From the theory of hitting times in 2D random walks~\cite{hitting}, the average distance away from the origin traversed in $t$ steps is $\sqrt{t}$. We consider two cases:
% \begin{itemize}
%     \item The agent employs ReachExplore to go to the frontier at a radius of $k^*$, using the deterministic goal-conditioned policy and then perform a random walk with the remaining $T-k^*$ steps. During this random walk the agent will go upto a distance of $\sqrt{T-k^*}$ in any direction. Let the total area traversed on average be $A_1$.
%     \item The agent does not employ ReachExplore and executes the default stochastic goal conditioned policy (which we assumed for simplicity to be the policy of a random walk) from the start state $\mathbf{s}_g$ and continues for  $T$ time-steps, thus ending up on an average somewhere in a circle of radius $\sqrt{T}$ centered at $\mathbf{s}_{k^*}\sim p_{k^*}$. Let the total area traversed on average be denoted by $A_2$, and we have $A_2=\pi T$.
% \end{itemize}
% We have the following lower bound on $A_1$ (Fig.~\ref{fig:analysis})
% $$A_1 \geq \chi\left(\pi (k^*)^2 + \frac{1}{2}\pi (T - k^*)\right) + (1-\chi)\pi (k^*)^2 $$
% Let us denote the above lower bound by $L_1$. To show $A_1>A_2$ it is enough to show that $L_1-A_2>0$. Let us consider the difference $L_1-A_2$:
% $$L_1-A_2 = \pi(k^*)^2 -\frac{1}{2}\pi\chi k^* + \frac{1}{2}\pi (\chi-2)T$$
% Treating the above as a quadratic expression in the variable $x=k^*$, we note that the value of $Ax^2+Bx+C>0$ $\forall x$ when $B^2-4AC < 0$. For our problem, $$B^2-4AC = \frac{1}{4}\pi^2\chi^2 - 2\pi^2T(\chi-2)=2\pi^2(\frac{1}{8}\chi^2-T\chi+2T)$$
% Since $\chi\in(0,1)$ and $T>1$, the value of $B^2-4AC$ is always greater than $0$. So, by analyzing the roots of the equation, 
% $$\pi(k^*)^2 -\frac{1}{2}\pi\chi k^* + \frac{1}{2}\pi (\chi-2)T = 0$$
% we have 
% $$\forall k^* >\frac{1}{4}\chi + \frac{1}{2}\sqrt{\frac{1}{4}\chi^2 -2T\chi + 4T}$$
% $L_1-A_2>0$ and so $A_1>A_2$. This result tells us that there is a certain value of frontier $k^*<T$ such that when we have achieved this frontier, it is beneficial to perform committed exploration via the ReachExplore approach. Now, in each iteration of training, since we sample goals beyond the currently reachable frontier $k^*$ (Section~\ref{sec:approach}C), so the value of $k^*$ will always increase during training. Hence, the above value will be reached at some point during training. 


==> neurips/5-experiments.tex <==

\section{Experiments}
\label{sec:exp}
Our experiments aim to understand the following questions: (1) How does LEAF compare to existing state-of-the-art exploration baselines, in terms of faster convergence and higher cumulative success? 
%(2) How does keeping track of reachability ensure faster convergence and deep exploration required to solve long-horizon robotic tasks directly from images?
(2) How does LEAF scale as task complexity increases?
(3) Can LEAF scale to tasks on a real robotic arm?

\subsection{Environments}
We consider the image-based and state-based environments illustrated in Fig.~\ref{fig:sim_envs}. In case of image-based environments, the initial state and the goal are both specified as images. In case of state-based environments, the initial state and the goal consists of the coordinates of the object(s), the position and velocity of different components of the robotic arm, and other details as appropriate for the environment (Refer to the Appendix for details). In both these cases, during training, the agent does not have access to any oracle goal-sampling distribution. 
% In Fig.~\ref{fig:sim_envs}, (b), and (c) are configured to be \textit{sparse-reward} settings, where the reward is $1$ only when the agent $solves$ the goal and is $0$ otherwise. To define when a goal is $solved$, for each environment there is a certain threshold distance between the agent's final state and the goal state, the details of which are mentioned in the appendix. 
All image-based environments use \textit{only} a latent distance based reward during training (reward $r=-||z_t-z_g||_2$; $z_t$ is the agent's current latent state and $z_g$ is the goal latent state), and have no access to ground-truth simulator states. 

% \begin{figure}[t]
% \centering
%         \begin{subfigure}[b]{0.5\columnwidth}
%               \centering             \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/one.png}
%     %\caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%          \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/five.png}
%   % \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%     % \includegraphics[width=0.7\columnwidth]{illustrative_figs/one.png}
%     \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%           \begin{subfigure}[b]{0.5\columnwidth}
%               \centering             \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/fetch_one.png}
%     %\caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%          \begin{subfigure}[b]{\columnwidth}
%               \centering
%     \includegraphics[width=0.8\columnwidth]{illustrative_figs/fetch_final.png}
%   % \caption{Sawyer Push and Reach}
%     \label{fig:pushreach}
%         \end{subfigure}
%     % \includegraphics[width=0.7\columnwidth]{illustrative_figs/one.png}
%     \caption{Fetch Slide}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
        
       
%      \caption{Illustrations of all the simulation environments evaluated in this paper, with example initial and goal images.}  
%  \label{fig:sim_results}
% \end{figure}

 
\begin{figure*}[h!]
\centering
\hspace*{-0.2cm}
 \begin{subfigure}[b]{0.64\textwidth}
               \centering
    \includegraphics[width=\textwidth]{neurips/sim_results.png}
    \caption{Comparative results on simulation environments}
    \label{fig:quantitative}
        \end{subfigure}\hspace*{-0.05cm}
                 \begin{subfigure}[b]{0.37\textwidth}
               \centering
    \includegraphics[width=\textwidth]{neurips/qualitative_line.png}
    \caption{Qualitative results showing the goal image on the left, and rendered images of the final states reached by SkewFit and our method for two evaluation runs in two different environments.}
    \label{fig:qualitative}
        \end{subfigure}

            %\quad
     \caption{Comparison of LEAF against the baselines. The error bars are with respect to three random seeds. The results reported are for evaluations on test suites (initial and goal images are sampled from a test distribution unknown to the agent) as training progresses. Although the ground-truth simulator states are not accessed during training (for (a), (c), (d), (e), and (f)), for the evaluation reported in these figures, we measure the ground truth $L_2$ norm of the final distance of the object/end-effector (as appropriate for the environment) from the goal location.  In (f), we evaluate the final distance between the (puck+end-effector)'s location and the goal location. In (a), (c), (d), (e), and (f), lower is better. In (b), higher is better.}  
 \label{fig:sim_results}
 \vspace*{-0.2cm}
\end{figure*}

 
%  Each environment we consider is meant to demonstrate scaling of the proposed approach to different settings: image-based goals, state-based goals (Fetch slide), continuous action spaces, discrete action spaces (Locked door navigation), different dynamics (point mass, Fetch robot, Sawyer robot, Franka Panda robot), and applicability to a real robot (Franka Panda).


\textbf{Image-based environments.} In the \textit{\textbf{Pointmass Navigation}} environment, a pointmass object must be navigated from an initial location to a goal location in the presence of obstacles. The agent must plan a temporally extended path that would occassionally involve moving away from the goal. In \textbf{\textit{Sawyer Pick}}, a Sawyer robot arm must be controlled to pick a puck from a certain location and lift it to a target location above the table. In \textbf{\textit{Sawyer Push}}, a Sawyer robot must push a puck to a certain location with the help of its end-effector. In \textbf{\textit{Sawyer Push and Reach}}, a Sawyer robot arm is controlled to push a puck to a target location, and move its end-effector to a (different) target location. In \textbf{\textit{Narrow Corridor Pushing}}, a Sawyer robot arm must push a puck from one end of a narrow slab to the other without it falling off the platform. This environment is challenging because it requires \textit\textit{{committed exploration}} to keep pushing the puck unidirectionally across the slab without it falling off.

\textbf{State-based environment.} In \textbf{\textit{Fetch Slide}}, a Fetch robot arm must be controlled to push and slide a puck on the table such that it reaches a certain goal location. It is ensured that sliding must happen (and not just pushing) because the goal location is beyond the reach of the arm's end-effector. In \textbf{\textit{Franka Panda Peg in a Hole}}, a real Franka Panda arm must be controlled to place a peg in a hole. The agent is velocity controlled and has access to state information - the position $(x,y,z)$ and velocity $(v_x,v_y,v_z)$ of its end-effector. 

% \begin{enumerate}

% %[
% %    topsep=0pt,
% %    noitemsep,
% %    leftmargin=*,
% %    itemindent=12pt]
  
%   \item \textbf{Pointmass Navigation} (\textit{Image-based}): A pointmass object must be navigated from an initial location to a goal location in the presence of obstacles. The agent must plan a temporally extended path that would occassionally involve moving away from the goal. This is a 2D environment with a continuous action space, and the agent has access to images from a top-down view. 
%   \item \textbf{Fetch Slide} (\textit{State-based}): A Fetch robot arm must be controlled to push and slide a puck on the table such that it reaches a certain goal location. It is ensured that sliding must happen (and not just pushing) because the goal location is beyond the reach of the arm's end-effector. We make this environment significantly difficult by reducing the default friction coefficient by a factor of 2. The agent has access to state information - the position $(x,y,z)$ and velocity $(v_x,v_y,v_z)$ of its end-effector. 
%   \item \textbf{Gridworld Locked Door Navigation} (\textit{Image-based}): A point agent navigates a maze to pick up a key, open a locked door, and navigate to a goal location on the other side of the door. This is a 2D environment, and the agent has access to a top-down view. At each time-step, the agent has the option to choose from six actions (so discrete action space).
%   \item \textbf{Sawyer Pick} (\textit{Image-based}): A Sawyer robot arm must be controlled to pick a puck from a certain location and lift it to a target location above the table. The agent has access to images from a camera mounted on the arm.
%         \item \textbf{Sawyer Push} (\textit{Image-based}): A Sawyer robot must push a puck to a certain location with the help of its end-effector. The agent has access to images from a camera mounted on the arm.
%     \item \textbf{Sawyer Push and Reach} (\textit{Image-based}): A Sawyer robot arm is controlled to push a puck to a target location, and move its end-effector to a (different) target location. The agent has access to images from a camera mounted on the arm.
%     \item \textbf{Franka Panda Peg in a Hole} (\textit{State-based; Real robot}); A real Franka Panda arm must be controlled to place a peg in a hole. The agent is velocity controlled and has access to state information - the position $(x,y,z)$ and velocity $(v_x,v_y,v_z)$ of its end-effector. 
% \end{enumerate}


\subsection{Setup}
We use the Pytorch library~\cite{pytorch1,pytorch2} in Python for implementing our algorithm, and ADAM~\cite{adam} for optimization.  We consider two recent state-of-the-art exploration algorithms, namely Skew-Fit~\cite{skew}, and Go-Explore~\cite{goexplore} as our primary baselines for comparison. For both these baselines, for consistency, we use SAC for policy-learning.  Based on the original implementation of Go-Explore~\cite{goexplore}, we create a version using SAC~\cite{sac} as the base policy and employing the Go-Explore trick which we use as our baseline. Implementation details are in the Appendix.

% For training, we train our method and the baselines in a completely unsupervised manner, without access to any oracle goal-sampling distribution. In addition, in the image-based environments, during training the agent does not have access to any prior information about the state-space. In order to 
% \textit{evaluate} the performance of the algorithms, we sample goal images from a uniform distribution over valid images and report the final distance of the agent to the corresponding states in simulator. This method of evaluation, although applicable only in simulation, is a reliable metric for RL with vision-based goals, as described in prior works~\cite{rig,skew}. It is important to note that we access the simulator states only for \textit{evaluation} - not for training (except for (b), and (h) in Fig.~\ref{fig:sim_envs}). 

%During training, to measure reward, we compute the $L_1$ norm of the difference between the agent's latent state $z_t$ and the goal latent state $z_g$.
% \begin{figure*}[h!]
% \centering
%  \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pointmassfinal.png}
%     \caption{Pointmass Navigation (Image)}
%     \label{fig:pointmass}
%         \end{subfigure}\hspace*{-0.2cm}
%                  \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pickplacefinal.png}
%     \caption{Sawyer Pick and Place (Image)}
%     \label{fig:pickplace}
%         \end{subfigure}
        
        
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/push_easy_final.png}
%     \caption{Sawyer Push (Image)}
%     \label{fig:pusheasy}
%         \end{subfigure}% \\
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/pushreachfinal.png}
%     \caption{Sawyer Push and Reach (Image)}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%         %\hspace*{-0.5cm}
        
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/gridlocked_doorfinal.png}
%     \caption{Gym Locked Door Navigation (Image)}
%     \label{fig:fetchslide}
%         \end{subfigure}\hspace*{-0.2cm}
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{results_figs/fetchslide_final.png}
%     \caption{Fetch robot - Slide (State)}
%     \label{fig:fetchslide}
%         \end{subfigure}
%             %\quad
%      \caption{Comparison of our method and SkewFit on an ensemble of vision-based and state-based simulation environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are with respect to three random seeds. It is important to emphasize that the training proceeds in a completely self-supervised manner (for both our method and SkewFit), without assuming any access to the oracle goal sampling distribution. The results reported are for evaluations on test suites (initial and goal images are sampled from a test distribution unknown to the agent) as training progresses. Although the ground-truth simulator states are not accessed during training (for (a), (b), (c), (d), and (e)), for the evaluation reported in these figures, we measure the ground truth L2 norm of the final distance of the oject/end-effector (as appropriate for the environment) from the goal location. In (e), success is measured as +1 if the agent reaches the final green goal square in the grid, and 0 otherwise. In (f), success is measured as +1 if the puck reaches the goal location with a tolerance threshold of $0.1\%$. In (a), (b), (c), and (d), lower is better. In (e) and (f), higher is better.}  
%  \label{fig:sim_results}
% \end{figure*}




\subsection{Results}
\vspace*{-0.3cm}
\noindent\textbf{Our method achieves higher success during evaluation in reaching closer to the goals compared to the baselines}
Fig.~\ref{fig:sim_results} shows comparisons of our method against the baseline algorithms on all the robotic simulation environments. We observe that our method performs significantly better than the baselines on the more challenging environments. The image based Sawyer Push and Reach environment is challenging because there are two components to the overall task. The Narrow corridor pushing task requires \textit{committed exploration} so that the puck does not fall off the table. The pointmass navigation environment is also challenging because during evaluation, we choose the initial position to be inside the U-shaped arena, and the goal location to be outside it. So, during training the agent must learn to set difficult goals outside the arena and must try to solve them.

%  The pointmass navigation environment is challenging because during evaluation, we choose the initial position to be inside the U-shaped area, and the goal location to be outside it, and the agent does not know this apriori. So, during training the agent must learn to set difficult goals outside the black arena and must try to solve them. This requires deep committed exploration, and as shown in Fig.~\ref{fig:quantitative}, our method succeeds in achieving this.

In addition to the image based goal environments, we consider a challenging state-based goal environment as proof-of-concept to demonstrate the effectiveness of our method. In Fetch-Slide Fig.~\ref{fig:quantitative} in order to succeed, the agent must acquire an implicit estimate of the friction coefficient between the puck and the table top, and hence must learn to set goals close and solve them before setting goals farther away. 


\noindent\textbf{Our method scales to tasks of increasing complexity}
From Fig.~\ref{fig:quantitative} (d. Sawyer Push), we see that our method performs comparably to its baselines. The improvement of our method over SkewFit is not statistically significant. However, in the task of Push and Reach (Fig.~\ref{fig:quantitative}) we observe significant improvement of our method over SkewFit and GoExplore. The baselines succeed either in the push part of the task or the reach part of the task but not both, suggesting overly greedy policies without long term consideration (Refer qualitative results in Fig.~\ref{fig:qualitative}).This suggests the effectiveness of our method in scaling to a difficult task that requires more temporal abstraction. This benefit is probably because our method performs two staged exploration, which enables it to quickly discover regions that are farther away from the initial state given at the start of the episode. 
%Since the agent receives a +1 reward only when it pushes the puck to the desired location and brings the end-effector to its desired location (i.e. sparse reward), focusing the thrust of exploration on previously unexplored states is crucial to discover trajectories that successfully solve the task. 

We observe similar behaviors of scaling to more complicated tasks by looking at the results of the Pointmass Navigation in Fig.~\ref{fig:quantitative}. While the task can be solved even by simple strategies when the goal location is within the U-shaped ring, the agent must actually discover temporally abstracted trajectories when the goal location is outside the U-shaped ring. Discovering such successful trajectories in the face of only latent rewards, and no ground-truth reward signals further demonstrates the need for committed exploration. 
  

% \begin{figure*}[t]
% \centering
%         \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pushreach_eval1.png}
%     \caption{Sawyer Push and Reach (Image)}
%     \label{fig:pushreach}
%         \end{subfigure}% \\
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pickplace_final.png}
%     \caption{Sawyer Pick and Place (Image)}
%     \label{fig:pickplace}
%         \end{subfigure}
        
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{pointmass.png}
%     \caption{Pointmass Navigation (Image)}
%     \label{fig:pointmass}
%         \end{subfigure}
%          \begin{subfigure}[b]{0.5\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{anglediff_compare.png}
%     \caption{Sawyer Door opening (I)[rev. legend]}
%     \label{fig:avg_r_lf}
%         \end{subfigure}
        
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{fetchslideresult.png}
%     \caption{Fetch robot - Slide (State)}
%     \label{fig:fetchslide}
%         \end{subfigure}
%          \begin{subfigure}[b]{0.45\textwidth}
%               \centering
%     \includegraphics[width=\textwidth]{fetchesults.png}
%     \caption{Fetch robot - Reach (State)}
%     \label{fig:results}
%         \end{subfigure}
%     %\quad
%      \caption{Comparison of our method and SkewFit on an ensemble of vision-based and state-based environments. In the vision based environments, the goal is specified as an image and ground truth states of the simulation are not used at all during training. The error bars are wrt 3 seeds in (a), (d), and (e), and wrt 2 seeds in (b), (c), and (f). It is important to emphasize that the training proceeds in a completely unsupervised manner (for both our method and SkewFit), without assuming any access to the oracle goal sampling distribution.}  
%  \label{fig:sim_results}
% \end{figure*}
  

  
\noindent\textbf{Our method scales to tasks on a Real Franka Panda robotic arm} Fig.~\ref{fig:panda} shows results for our method on a peg-in-a-hole evaluated on the Franka Panda arm. Here the objective is to insert a peg into a hole, an illustration of which is shown in Fig.~\ref{fig:sim_envs}.  The reward function is defined to be the negative of the distance from the center of bottom of the peg to the center of the bottom of the hole. There is an additional heavy reward penalty for `collision' and a mild penalty for `contact.' The home position of the panda arm (to which it is initialized) is such that the distance from the center of the bottom of the peg to the center of the bottom of the hole is 0.35 meters. The heavy penalty for collision is -10 and the mild penalty for contact is -1. We can observe from Fig.~\ref{fig:panda} that our method successfully solves the task while the baseline GoExplore does not converge to the solution. This demonstrates the applicability of our method on a real robotic arm.

% \begin{figure}
%   \centering
%  \begin{subfigure}[b]{0.7\columnwidth}
%               \centering
%     \includegraphics[width=\columnwidth]{results_figs/franka_real_arm.png}
%     \caption{Reaching task (State-based)}
%     \label{fig:pointmass}
%         \end{subfigure}%\hspace*{-0.2cm}
%                  \begin{subfigure}[b]{0.2\columnwidth}
%               \centering
%     \includegraphics[width=\columnwidth]{illustrative_figs/pandaarm.png}
%     \caption{Panda arm}
%     \label{fig:pickplace}
%         \end{subfigure}
%       \caption{Results of a Reaching task on the real Franka Emika Panda arm. The goal is specified as a tuple of coordinates (x,y,z) to be reached. The state consists of the position and velocities of the end-effector. Higher is better.}
%     \label{fig:panda}
%     \vspace*{-0.2cm}
% \end{figure}


\begin{figure}
   \centering
       \begin{minipage}[c]{0.5\textwidth}
    \includegraphics[width=0.88\columnwidth]{neurips/real.png}    
      \end{minipage}
        \begin{minipage}[c]{0.3\textwidth}
    \caption{Results of a Peg-in-a hole task on the real Franka Emika Panda arm. The evaluation metric on the y-axis is the distance ($L_2$ norm) of the center of the bottom of the hole from the center of the bottom of the peg.}
    \label{fig:panda}
      \end{minipage}
     \vspace*{-0.8cm}
  \end{figure}
   

==> neurips/6-related_works.tex <==
\vspace*{-0.35cm}
\section{Related Works}
\vspace*{-0.35cm}

\noindent \textbf{Vision-based RL for Robotics.} 
% Reinforcement Learning from images has been very successful in recent times, for playing computer games~\cite{atari1,atari2} and performing control tasks in simulated environments~\cite{dreamer,planet,sacae}.  Planet~\cite{planet} and Dreamer~\cite{dreamer} learn world models and perform planning in a learned representation space either through online planning or through an amortized policy.
Although model-based RL approaches like Planet~\cite{planet} and Dreamer~\cite{dreamer} are sample efficient, their success in comparison to model-free RL~\cite{upn,skew,rig,leap} at solving long-horizon goal-conditioned tasks that involve complex manipulation and locomotion has been limited~\cite{fly}. CURL~\cite{curl} incorporates the idea of contrastive learning of representations that has been successful in computer vision, as an auxiliary loss for model-free RL. Two very recent papers~\cite{rad,nyu} demonstrate how model-free RL can be regularized by incorporating data augmentations (like random crops, color jitters etc.) of input image frames to the policy. Theses approaches aim to learn good representations from images, for planning and are orthogonal to our work. 

Recent works have investigated vision-based learning of RL policies for specific robotic tasks like grasping~\cite{grasping1,grasping2}, pushing~\cite{pushing2,pushing1}, and navigation~\cite{navigation2,navigation1}, however relatively few prior works have considered the problem of learning policies in a completely self-supervised manner~\cite{rig,skew}. A recent paper~\cite{avi} considers RL directly from images, for general tasks without engineering a reward function, but involves a human in the loop. Other prior works learn latent representations for RL in an unsupervised manner which can be used as input to the policy, but they either require expert demonstration data~\cite{upn,sim2realmanga}, or assume access to ground-truth states and reward functions during training~\cite{worldmodels,ground2,ground3}. RIG~\cite{rig} proposes a general approach of first learning a latent abstraction from images, and then planning in the latent space, but requires data collected from a randomly initialized policy to design parametric goal distributions.  In addition, either approaches do not guarantee any notion of exploration or coverage that is required for solving difficult temporally-extended tasks from minimal supervision - in particular with goals specified as raw images.



\noindent \textbf{Goal-conditioned Policy Learning.}
While traditional model-free RL algorithms are trained to succeed in single tasks~\cite{td3,sac,ppo,trpo}, goal-conditioned policy learning holds the promise of learning general-purpose policies that can be used for different tasks specified as different goals~\cite{kaelbling1993learning,her,rig,arc}. However, most goal-conditioned policy learning algorithms make the stronger assumption of having access to an oracle goal sampling distribution during training~\cite{kaelbling1993learning,her,universal,leap}. A recent paper~\cite{arc} proposes an algorithm to create dynamics-aware embeddings of states, for goal-conditioned RL, but it is not scalable to images as goals (instead of ground-truth states).  

% Some other prior works do not assume access to an oracle goal-sampling distribution, but sample goals based on some ad-hoc heuristics like learning progress~\cite{learnprogress1,learnprogress2}, how off-policy the goal is~\cite{offpolicy} or sample goals randomly from the learn latent distribution over image observations~\cite{rig}. Skew-Fit~\cite{skew} adds structure to the goal-sampling process by sampling goals in the latent space such that the entropy over the learned distribution over states is maximized, but provides no guarantee of coverage/exploration in finite time. 





\noindent \textbf{Exploration for RL.} Skew-fit~\cite{skew} proposes a novel entropy maximizing objective that ensures gradual coverage in the infinite time limit. In addition, it does not incorporate any notion of commitment during exploration, which is needed to discover complex skills for solving temporally extended tasks in finite time. Go-Explore~\cite{goexplore} addresses this issue to some extent by keeping track of previously visited states in the replay buffer, and at the start of each episode, re-setting the environment to a previously visited state chosen on the basis of domain-specific heuristics, and continuing exploration from there. However, this approach is fundamentally limited for robotics because it assumes the environment is re-settable, which is not always feasible especially for policy learning from images. In addition, the domain-specific heuristics for Montezuma's revenge in the paper~\cite{goexplore} do not readily apply to latent spaces for robotic tasks.

On the contrary, novelty/surprise based criteria have been used in many RL applications like games, and mazes~\cite{curiosity,count,rupam}. 
% In~\cite{curiosity}, a curiosity based intrinsic reward signal is used in addition to the external reward in order to encourage the RL agent to visit previously unvisited states. In~\cite{count}, the authors explicitly keep track of the state visitation frequencies and reward the agent for visiting states with less visitation frequency.
VIME \cite{vime} considers information gathering behaviors to reduce epistemic uncertainty on the dynamics model. 
A recent paper, Plan2Explore~\cite{plan2explore} incorporates an information gain based intrinsic reward to first learn a world model similar to Dreamer~\cite{dreamer}, without rewards and then learn a policy given some reward function. The main drawbacks of this approach are that it tries to learn a global world model which is often infeasible in complex environments, and requires reward signals from the environment for adaptation. In contrast, our approach can learn to explore using latent rewards alone.

%Although these methods are general in that novelty bonuses are not %task-specific, there is no mechanism to distill the learned %knowledge from visiting novel states into adaptive policies that can %adapt to diverse goals at test-time. The policies learned are %reactive because the knowledge gained by visiting $novel$ states is %quickly forgotten when other states become more novel.

\noindent \textbf{Reachability and Curriculum Learning.} Our method is related to curriculum learning approaches in reinforcement learning \cite{approximate_hjb, curriculum_held, ELMAN199371, openai2019solving, curriculum_bengio, racaniere2019automated} whereby learning easier tasks is prioritized over hard tasks, as long as measures are taken to avoid forgetting behaviors on old tasks. We compute reachability in the latent space and as such our work is distinct from traditional HJ-reachability~\cite{hjb} computations that involve computation of reachable sets of physical robot states by solving Partial Differential Equations (PDEs). 

\noindent \textbf{Frontier-based Exploration for Robot Mapping.} Finally, our method intuitively relates to a large body of classic work on robot mapping, particularly frontier-based exploration approaches \cite{frontier_based_exploration, frontier_based_exploration_multirobot, frontier_based_exploration_holz}.
\vspace*{-0.6cm}

==> neurips/7-conclusion.tex <==
 \vspace*{-0.2cm}
\section{Conclusion} 
 \vspace*{-0.3cm}
\label{sec:conclusion}
In this paper we proposed an algorithm for committed exploration, by keeping track of the frontier of reachable states, and during the start of every episode, executing a deterministic goal-conditioned policy to reach the current frontier, followed by executing a stochastic goal-conditioned exploration policy to reach the goal. The proposed approach can work directly over image-based observations and goal specifications, does not require any reward signal from the environment during training, and is completely self-supervised in that it does not assume access to the oracle goal-sampling distribution for evaluation. Through experiments on eight environments with varying characteristics, task complexities, and temporal abstractions, we demonstrate the efficacy of the proposed approach over state of the art exploration baselines.

